Interactive Dimensionality Reduction for Comparative Analysis

Finding the similarities and differences between groups of datasets is a fundamental analysis task. For high-dimensional data, dimensionality reduction (DR) methods are often used to find the characteristics of each group. However, existing DR methods provide limited capability and flexibility for such comparative analysis as each method is designed only for a narrow analysis target, such as identifying factors that most differentiate groups. This paper presents an interactive DR framework where we integrate our new DR method, called ULCA (unified linear comparative analysis), with an interactive visual interface. ULCA unifies two DR schemes, discriminant analysis and contrastive learning, to support various comparative analysis tasks. To provide flexibility for comparative analysis, we develop an optimization algorithm that enables analysts to interactively refine ULCA results. Additionally, the interactive visualization interface facilitates interpretation and refinement of the ULCA results. We evaluate ULCA and the optimization algorithm to show their efficiency as well as present multiple case studies using real-world datasets to demonstrate the usefulness of this framework.

==> plots/plot_adjustment.tex <==
\tikzstyle{every plot}=[mark size=1pt]


==> supp_material/tables/mnist1.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &       PCA (x) &       PCA (y) &  LDA (x) &  LDA (y) &      cPCA (x) &      cPCA (y) &      ULCA (x) &      ULCA (y) \\
\midrule
0   & -1.066943e-19 & -3.860139e-17 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.027102e-08 & -7.703082e-11 \\
1   &  1.626916e-19 &  4.847268e-17 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  9.010722e-08 & -3.901668e-09 \\
2   &  2.616794e-22 &  1.858932e-19 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  6.035688e-08 & -2.390753e-09 \\
3   &  7.254972e-22 &  1.930773e-21 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.917857e-08 &  1.367573e-09 \\
4   &  6.703058e-23 & -2.095476e-21 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.469582e-08 & -2.886394e-09 \\
5   &  2.510439e-22 & -9.866802e-21 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.652723e-08 &  4.954351e-09 \\
6   & -2.448274e-22 &  9.769129e-21 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.297794e-08 &  2.045424e-09 \\
7   &  1.540200e-23 & -8.235647e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.213687e-08 & -2.767319e-10 \\
8   & -2.594627e-23 & -8.928126e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.800730e-08 &  3.403123e-09 \\
9   & -9.498393e-25 &  3.381705e-23 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.542507e-09 & -5.397740e-10 \\
10  &  1.822856e-25 &  1.555424e-23 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  9.947645e-09 &  2.813022e-09 \\
11  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.220844e-08 & -4.557665e-09 \\
12  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.706412e-08 & -6.710318e-09 \\
13  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.314477e-09 &  1.620035e-10 \\
14  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.742116e-10 & -1.171929e-10 \\
15  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.468125e-09 &  2.111210e-09 \\
16  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.896838e-09 & -9.114433e-10 \\
17  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -6.440826e-09 &  2.791805e-09 \\
18  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.784358e-08 &  5.391066e-10 \\
19  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.900210e-08 & -4.341927e-09 \\
20  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.471530e-09 &  1.058321e-09 \\
21  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.789058e-08 & -2.818901e-09 \\
22  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  7.026077e-09 & -7.532502e-10 \\
23  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.597455e-08 & -5.703140e-10 \\
24  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.343949e-08 &  1.531389e-09 \\
25  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  7.795557e-08 & -5.016488e-09 \\
26  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.914440e-08 &  1.027761e-09 \\
27  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.459823e-07 & -8.217156e-09 \\
28  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  6.488609e-09 &  2.012782e-09 \\
29  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.198707e-08 &  2.052823e-09 \\
30  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.573259e-08 & -1.960981e-09 \\
31  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  8.137611e-08 & -1.439407e-09 \\
32  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.108930e-08 &  2.523099e-09 \\
33  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -8.088564e-08 &  1.960208e-09 \\
34  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.800779e-08 & -3.426313e-09 \\
35  &  2.141479e-05 &  1.420012e-04 &        0 &        0 &  1.583297e-03 &  2.335186e-01 &  7.037726e-04 &  2.305472e-04 \\
36  &  6.934092e-05 &  4.678008e-04 &        0 &        0 &  1.949582e-03 &  2.806236e-01 &  2.363167e-03 &  7.473891e-04 \\
37  &  9.065502e-05 &  6.198897e-04 &        0 &        0 &  2.050037e-03 &  2.923686e-01 &  3.176937e-03 &  9.780326e-04 \\
38  &  4.795026e-05 &  3.302025e-04 &        0 &        0 &  2.006537e-03 &  2.386235e-01 &  2.610536e-03 &  1.006989e-03 \\
39  & -1.469842e-04 & -3.991366e-05 &        0 &        0 &  1.027811e-03 &  3.597852e-02 &  3.785984e-03 &  1.611099e-03 \\
40  & -1.864405e-04 & -1.747394e-04 &        0 &        0 &  1.029379e-03 &  2.293562e-02 &  2.859807e-03 &  1.009014e-03 \\
41  & -3.504243e-04 & -1.612662e-04 &        0 &        0 &  8.124271e-04 &  2.308845e-03 &  3.195220e-03 &  1.637788e-03 \\
42  & -1.462095e-04 &  3.774623e-05 &        0 &        0 &  8.027485e-04 & -1.347593e-03 &  1.745865e-03 &  1.616270e-03 \\
43  & -2.795246e-04 & -1.016695e-04 &        0 &        0 &  1.099934e-03 & -2.285887e-03 &  1.863446e-03 &  1.662240e-03 \\
44  & -1.122669e-04 & -3.305153e-04 &        0 &        0 &  1.130170e-03 & -1.920199e-03 &  2.201768e-03 &  2.183190e-03 \\
45  & -1.704615e-04 & -9.559961e-05 &        0 &        0 &  9.266115e-04 & -2.979863e-03 &  3.341397e-03 &  2.400132e-03 \\
46  & -2.150866e-04 & -2.517956e-04 &        0 &        0 &  7.163069e-04 & -2.519505e-03 &  1.344074e-03 &  1.069385e-03 \\
47  & -2.070278e-04 & -4.578290e-04 &        0 &        0 &  5.698027e-04 & -2.648679e-03 & -4.654569e-04 & -4.686722e-05 \\
48  & -2.751982e-04 & -6.870292e-04 &        0 &        0 &  5.177502e-04 & -2.630828e-03 & -8.219739e-04 & -2.915758e-04 \\
49  & -1.766674e-04 & -3.502533e-04 &        0 &        0 &  5.979898e-04 & -2.736392e-03 & -2.289486e-04 & -3.423557e-05 \\
50  & -9.764449e-05 & -1.747688e-04 &        0 &        0 &  5.077856e-04 & -2.224043e-03 & -8.200302e-05 &  2.434360e-05 \\
51  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.737915e-06 &  1.334266e-05 & -9.105226e-08 &  4.166322e-09 \\
52  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.409297e-06 & -4.034532e-05 &  7.553839e-11 &  1.701089e-09 \\
53  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.424714e-06 & -2.870812e-05 & -4.088139e-08 &  3.234278e-09 \\
54  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.936585e-06 & -5.577442e-06 &  1.220254e-07 & -8.038437e-09 \\
55  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.847935e-06 &  2.021725e-05 & -2.085434e-08 & -2.339753e-09 \\
56  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -2.354756e-06 & -2.691240e-05 & -4.123377e-09 & -1.785644e-10 \\
57  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -2.872221e-06 & -4.063779e-05 &  1.109846e-07 & -1.197066e-09 \\
58  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  6.304099e-08 &  1.294663e-05 &  1.341694e-08 &  1.188789e-09 \\
59  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.616317e-06 & -5.771643e-06 & -3.707441e-08 & -5.210299e-10 \\
60  & -1.454007e-05 & -1.217338e-04 &        0 &        0 &  4.699355e-04 &  1.493275e-02 &  9.654109e-05 & -1.475374e-05 \\
61  & -3.233935e-06 & -7.997835e-06 &        0 &        0 &  1.188110e-03 &  1.798177e-01 &  8.216944e-05 &  8.356831e-06 \\
62  & -8.019935e-06 &  2.130556e-05 &        0 &        0 &  1.102102e-03 &  1.965552e-01 &  3.342575e-04 &  4.585130e-05 \\
63  &  1.521343e-05 &  1.342129e-04 &        0 &        0 &  2.299375e-03 &  3.378341e-01 &  8.185197e-04 &  2.622982e-04 \\
64  &  8.817535e-05 &  7.078319e-04 &        0 &        0 &  2.237729e-03 &  2.969654e-01 &  4.804765e-03 &  2.044379e-03 \\
65  &  1.996231e-04 &  1.101081e-03 &        0 &        0 &  2.241431e-03 &  2.541362e-01 &  7.825069e-03 &  3.379556e-03 \\
66  & -7.881813e-05 &  1.358874e-03 &        0 &        0 &  2.375113e-03 &  2.017457e-01 &  1.417397e-02 &  6.449261e-03 \\
67  & -4.682708e-04 &  1.021614e-03 &        0 &        0 &  1.935793e-03 &  6.533136e-02 &  1.567659e-02 &  8.393025e-03 \\
68  & -9.109280e-04 &  1.299544e-03 &        0 &        0 &  2.077393e-03 &  2.399036e-02 &  1.833006e-02 &  1.064592e-02 \\
69  & -2.388379e-03 &  1.444106e-03 &        0 &        0 &  2.384291e-03 &  2.680245e-03 &  2.847795e-02 &  1.611765e-02 \\
70  & -4.785381e-03 & -8.411610e-04 &        0 &        0 &  3.023460e-03 & -5.692958e-03 &  3.837617e-02 &  2.236052e-02 \\
71  & -6.699287e-03 & -6.605252e-03 &        0 &        0 &  3.575491e-03 & -8.521369e-03 &  3.794521e-02 &  2.299228e-02 \\
72  & -1.019139e-02 & -1.725007e-02 &        0 &        0 &  4.136666e-03 & -1.204051e-02 &  3.171617e-02 &  1.871964e-02 \\
73  & -1.050355e-02 & -2.418862e-02 &        0 &        0 &  4.117270e-03 & -1.149372e-02 &  2.013591e-02 &  9.255015e-03 \\
74  & -8.755442e-03 & -2.466403e-02 &        0 &        0 &  3.513699e-03 & -9.111856e-03 & -3.336599e-03 & -4.419848e-03 \\
75  & -6.277631e-03 & -1.914395e-02 &        0 &        0 &  2.649492e-03 & -7.408460e-03 & -1.388818e-02 & -7.331314e-03 \\
76  & -3.390335e-03 & -1.048850e-02 &        0 &        0 &  1.981627e-03 & -7.469066e-03 & -1.556160e-02 & -4.288025e-03 \\
77  & -1.540892e-03 & -4.769709e-03 &        0 &        0 &  1.475993e-03 & -6.115922e-03 & -7.096821e-03 & -2.156385e-03 \\
78  & -4.380928e-04 & -1.390021e-03 &        0 &        0 &  1.019801e-03 & -4.293997e-03 & -2.295444e-03 & -6.834142e-04 \\
79  & -2.505553e-05 & -9.833885e-05 &        0 &        0 &  5.692455e-04 & -2.147084e-03 & -1.953755e-04 & -1.837935e-05 \\
80  & -6.520683e-06 & -2.126383e-05 &        0 &        0 &  1.248884e-03 & -1.713421e-03 &  2.821700e-06 &  1.711490e-05 \\
81  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  4.023413e-07 &  2.100001e-05 & -5.008308e-08 &  2.343675e-09 \\
82  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.948925e-06 & -1.342980e-05 &  2.565924e-08 &  2.704572e-09 \\
83  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.084184e-06 &  7.520904e-06 & -5.709850e-08 &  3.064513e-09 \\
84  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.754817e-06 & -2.678965e-05 & -1.453021e-07 &  8.458548e-09 \\
85  &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -9.156694e-07 &  2.497910e-05 & -2.382170e-08 &  3.577268e-09 \\
86  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.994162e-06 &  2.416565e-05 &  2.506050e-08 & -1.025892e-09 \\
87  &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  5.126476e-06 &  1.230141e-05 & -2.163562e-08 &  2.593381e-09 \\
88  & -1.504145e-06 & -1.259315e-05 &        0 &        0 &  4.689365e-04 &  1.489937e-02 &  1.001788e-05 & -1.528445e-06 \\
89  & -2.745557e-05 &  7.017293e-05 &        0 &        0 &  1.100655e-03 &  1.966946e-01 &  1.135269e-03 &  1.552870e-04 \\
90  & -8.530231e-06 & -1.859686e-05 &        0 &        0 &  1.171200e-03 &  1.772907e-01 &  2.472399e-03 &  3.918443e-04 \\
91  & -2.847441e-05 &  1.613052e-04 &        0 &        0 &  1.609475e-03 &  2.367045e-01 &  1.444258e-03 &  2.937773e-04 \\
92  &  2.245414e-04 &  1.232844e-03 &        0 &        0 &  2.146825e-03 &  2.600684e-01 &  6.384866e-03 &  2.974617e-03 \\
93  &  1.814069e-04 &  1.778924e-03 &        0 &        0 & -2.074319e-03 &  2.903133e-02 &  1.064907e-02 &  5.515632e-03 \\
94  & -1.128338e-04 &  2.853915e-03 &        0 &        0 &  1.904411e-04 & -2.357457e-02 &  2.012018e-02 &  1.111538e-02 \\
95  & -4.200656e-04 &  3.848927e-03 &        0 &        0 &  2.284668e-03 & -1.783358e-03 &  2.612415e-02 &  1.525719e-02 \\
96  & -1.188916e-03 &  4.396881e-03 &        0 &        0 & -1.635598e-03 &  2.536130e-03 &  3.961123e-02 &  2.100437e-02 \\
97  & -3.756395e-03 &  2.019969e-03 &        0 &        0 & -3.585004e-04 & -5.895626e-04 &  5.553539e-02 &  3.002615e-02 \\
98  & -1.005784e-02 & -6.120490e-03 &        0 &        0 &  2.404350e-04 & -2.779238e-05 &  6.863230e-02 &  3.814769e-02 \\
99  & -1.605898e-02 & -2.511135e-02 &        0 &        0 & -6.997421e-04 & -8.768929e-04 &  6.019384e-02 &  3.403422e-02 \\
100 & -2.054124e-02 & -4.378048e-02 &        0 &        0 &  1.058115e-03 & -2.300214e-04 &  2.362416e-02 &  1.412719e-02 \\
101 & -2.231438e-02 & -5.559643e-02 &        0 &        0 & -1.482627e-03 &  8.686634e-04 & -2.761769e-02 & -1.623399e-02 \\
102 & -1.835703e-02 & -5.298796e-02 &        0 &        0 &  6.196251e-04 & -3.101986e-03 & -5.942865e-02 & -3.183916e-02 \\
103 & -1.288975e-02 & -4.037896e-02 &        0 &        0 & -1.607644e-03 &  5.638135e-03 & -5.973510e-02 & -2.918068e-02 \\
104 & -6.496134e-03 & -2.143974e-02 &        0 &        0 & -1.834041e-05 & -7.295467e-03 & -4.071466e-02 & -1.620991e-02 \\
105 & -2.715744e-03 & -8.899740e-03 &        0 &        0 &  9.557631e-04 &  2.247964e-03 & -1.801951e-02 & -7.929090e-03 \\
106 & -7.492111e-04 & -2.922975e-03 &        0 &        0 &  1.693799e-03 & -4.614625e-03 & -8.672141e-03 & -3.493879e-03 \\
107 & -9.175876e-05 & -5.763813e-04 &        0 &        0 &  1.377909e-03 & -2.851387e-03 & -2.031714e-03 & -6.705101e-04 \\
108 & -3.369020e-05 & -1.098631e-04 &        0 &        0 &  1.254801e-03 & -1.749443e-03 &  1.479475e-05 &  8.842345e-05 \\
109 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.159026e-06 &  5.797796e-06 &  8.902674e-09 & -1.264789e-10 \\
110 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.982250e-08 &  3.884795e-07 &  4.288563e-08 & -9.508111e-09 \\
111 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.504604e-06 & -7.331128e-06 &  1.263440e-08 & -3.782927e-09 \\
112 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.021971e-07 &  1.388899e-05 & -1.203590e-08 &  5.481508e-11 \\
113 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -2.587492e-06 &  1.364018e-06 &  2.592038e-08 & -6.315803e-10 \\
114 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.692745e-06 & -8.251351e-06 &  3.174198e-08 & -3.243887e-09 \\
115 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.464686e-06 & -4.861578e-06 &  6.833971e-08 & -3.358997e-09 \\
116 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  6.496020e-07 &  3.976188e-06 & -1.726289e-08 &  3.300776e-09 \\
117 & -7.138287e-05 &  9.401457e-05 &        0 &        0 &  1.152383e-03 &  1.944178e-01 &  2.123546e-03 &  6.217268e-04 \\
118 & -1.156889e-04 &  3.392050e-04 &        0 &        0 &  1.137495e-03 &  1.805482e-01 &  2.310219e-03 &  7.140420e-04 \\
119 & -6.257918e-05 &  4.124084e-04 &        0 &        0 &  8.223259e-04 &  2.021767e-02 &  2.008065e-03 &  6.439136e-04 \\
120 &  2.634020e-04 &  1.524654e-03 &        0 &        0 & -6.608202e-04 &  1.079938e-02 &  7.793364e-03 &  4.473203e-03 \\
121 &  1.331130e-03 &  4.056586e-03 &        0 &        0 &  2.068892e-03 & -1.286384e-02 &  1.258435e-02 &  8.164550e-03 \\
122 &  2.899639e-03 &  8.369686e-03 &        0 &        0 & -7.255810e-04 &  5.682551e-03 &  1.820079e-02 &  1.015864e-02 \\
123 &  6.657351e-03 &  1.378415e-02 &        0 &        0 &  7.774867e-04 & -3.215047e-03 &  2.810473e-02 &  1.311050e-02 \\
124 &  1.286944e-02 &  1.637358e-02 &        0 &        0 & -1.565622e-03 &  7.909028e-04 &  2.768897e-02 &  7.805286e-03 \\
125 &  1.569124e-02 &  9.267593e-03 &        0 &        0 &  3.116873e-03 &  5.333401e-04 &  3.959490e-02 &  1.442328e-02 \\
126 &  1.311932e-02 & -1.400890e-02 &        0 &        0 & -7.771826e-04 & -3.592217e-04 &  4.215259e-02 &  1.773594e-02 \\
127 &  9.264380e-03 & -4.952580e-02 &        0 &        0 & -5.012668e-05 & -5.966737e-04 &  2.260526e-02 &  1.097497e-02 \\
128 &  7.338180e-03 & -8.039223e-02 &        0 &        0 & -3.331033e-04 &  3.646417e-05 & -2.147644e-02 & -1.294755e-02 \\
129 &  6.813228e-03 & -9.717650e-02 &        0 &        0 &  3.045173e-03 & -1.917153e-04 & -5.711175e-02 & -2.373833e-02 \\
130 &  9.757080e-03 & -8.696905e-02 &        0 &        0 &  2.904477e-04 & -8.690626e-04 & -5.630690e-02 & -1.999605e-02 \\
131 &  8.858076e-03 & -6.424214e-02 &        0 &        0 &  4.388131e-04 &  1.583222e-03 & -5.145080e-02 & -1.225400e-02 \\
132 &  7.963181e-03 & -3.948800e-02 &        0 &        0 &  4.227089e-04 & -1.902014e-03 & -2.926695e-02 & -4.385695e-03 \\
133 &  5.787917e-03 & -1.854834e-02 &        0 &        0 & -1.794323e-03 &  2.104809e-03 & -4.728196e-03 &  3.251155e-03 \\
134 &  3.387146e-03 & -7.747194e-03 &        0 &        0 &  1.076445e-03 & -1.861993e-03 & -4.247772e-03 & -3.494357e-04 \\
135 &  9.322442e-04 & -2.584241e-03 &        0 &        0 &  3.452901e-03 &  3.878325e-04 & -1.537214e-03 & -2.535334e-04 \\
136 &  6.996322e-05 & -3.698170e-04 &        0 &        0 &  5.654847e-03 & -1.552297e-03 &  1.933156e-03 &  1.318860e-03 \\
137 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.797633e-06 & -8.723434e-07 & -2.592411e-08 &  1.587503e-09 \\
138 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -4.067987e-06 &  1.063641e-07 & -3.637824e-08 &  2.374917e-09 \\
139 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -2.016470e-06 &  9.634008e-07 & -3.320553e-08 &  3.968548e-09 \\
140 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  3.907960e-06 &  3.475411e-06 & -8.485827e-08 &  4.858036e-09 \\
141 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.458799e-06 & -4.367545e-06 & -1.608428e-09 & -6.774078e-10 \\
142 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.378693e-06 &  1.072799e-06 &  5.662927e-08 & -5.150011e-10 \\
143 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  4.749959e-07 &  6.604598e-07 &  6.709692e-08 & -5.082877e-09 \\
144 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.223055e-07 & -2.548626e-06 & -1.530362e-08 & -4.780718e-09 \\
145 & -1.251045e-04 &  2.363771e-04 &        0 &        0 &  8.052741e-04 &  1.269303e-01 &  1.685727e-03 &  7.257591e-04 \\
146 & -1.210471e-04 &  6.101555e-04 &        0 &        0 & -4.115893e-04 & -4.759189e-03 &  2.531402e-03 &  1.129259e-03 \\
147 &  3.820411e-04 &  1.253652e-03 &        0 &        0 &  1.393960e-03 &  3.688546e-02 &  4.381814e-03 &  3.671352e-03 \\
148 &  1.734804e-03 &  3.378952e-03 &        0 &        0 & -2.019147e-03 & -6.562839e-03 &  6.660184e-03 &  6.106254e-03 \\
149 &  6.008441e-03 &  1.060866e-02 &        0 &        0 & -5.665504e-04 &  3.144285e-05 &  9.062167e-03 &  2.035206e-03 \\
150 &  1.365205e-02 &  2.181864e-02 &        0 &        0 & -1.299037e-04 &  1.288466e-03 &  1.699815e-02 & -1.188465e-03 \\
151 &  2.472075e-02 &  3.232028e-02 &        0 &        0 &  1.254177e-04 & -1.364909e-03 &  1.928434e-02 & -7.557436e-03 \\
152 &  3.595335e-02 &  3.184120e-02 &        0 &        0 &  1.609113e-03 & -6.058883e-03 &  2.486180e-02 & -1.504301e-02 \\
153 &  4.277292e-02 &  1.333674e-02 &        0 &        0 & -1.495348e-03 &  2.285457e-03 &  2.711689e-02 & -1.254119e-02 \\
154 &  4.743285e-02 & -2.678377e-02 &        0 &        0 &  2.233092e-03 &  2.515694e-04 &  5.274220e-03 & -1.290431e-02 \\
155 &  5.222111e-02 & -6.701449e-02 &        0 &        0 & -1.434879e-03 & -2.383377e-04 & -3.373129e-02 & -2.011495e-02 \\
156 &  5.514287e-02 & -9.991766e-02 &        0 &        0 &  9.048169e-04 & -8.125299e-04 & -7.137286e-02 & -2.796359e-02 \\
157 &  5.569360e-02 & -1.019238e-01 &        0 &        0 & -3.019834e-03 &  2.291138e-03 & -8.174233e-02 & -1.548957e-02 \\
158 &  5.290066e-02 & -8.799980e-02 &        0 &        0 & -6.284229e-05 & -2.143120e-03 & -6.327744e-02 &  1.509880e-03 \\
159 &  4.380542e-02 & -6.304551e-02 &        0 &        0 & -4.615493e-04 & -8.740335e-04 & -3.018415e-02 &  1.198466e-02 \\
160 &  3.177715e-02 & -4.135114e-02 &        0 &        0 & -2.771838e-04 & -8.376385e-04 &  2.058886e-03 &  1.006220e-02 \\
161 &  1.973962e-02 & -2.548976e-02 &        0 &        0 &  1.396615e-03 & -6.428923e-04 &  4.350026e-03 &  7.268486e-03 \\
162 &  1.008593e-02 & -1.208031e-02 &        0 &        0 &  1.078053e-04 &  1.175869e-03 &  3.428054e-04 &  2.313055e-03 \\
163 &  3.861963e-03 & -4.649756e-03 &        0 &        0 &  2.024584e-03 & -1.647458e-03 & -8.415595e-04 & -1.573232e-03 \\
164 &  2.897579e-04 & -7.528207e-04 &        0 &        0 & -1.346726e-02 &  3.940025e-03 &  3.300694e-03 &  1.484869e-03 \\
165 & -8.066816e-05 & -3.339106e-05 &        0 &        0 & -3.330325e-01 &  2.075505e-03 & -7.646283e-05 & -4.948331e-04 \\
166 & -3.007965e-05 & -1.245091e-05 &        0 &        0 & -3.330428e-01 &  2.074308e-03 & -2.844735e-05 & -1.845202e-04 \\
167 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -4.824262e-07 &  1.054770e-07 & -8.883138e-09 & -2.832829e-09 \\
168 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  6.410822e-07 &  2.492222e-07 & -3.668293e-08 &  2.419690e-10 \\
169 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.354939e-06 &  1.159788e-06 &  1.045172e-07 & -7.523917e-09 \\
170 & -5.627283e-05 & -1.383398e-04 &        0 &        0 &  2.893956e-04 & -1.027259e-03 &  5.366919e-05 & -1.825515e-05 \\
171 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  7.804176e-07 & -8.571932e-07 & -3.399142e-08 & -6.063729e-10 \\
172 &  6.522522e-05 & -2.401243e-06 &        0 &        0 &  9.282806e-04 & -7.218847e-03 & -1.727317e-05 &  4.060813e-04 \\
173 &  1.316882e-04 &  3.378436e-04 &        0 &        0 & -4.951055e-05 &  4.176402e-02 &  7.525964e-04 &  1.593508e-03 \\
174 &  2.291244e-05 &  1.185044e-03 &        0 &        0 & -7.532118e-04 & -3.798422e-02 &  1.692194e-03 &  2.740834e-03 \\
175 &  1.024071e-03 &  2.934609e-03 &        0 &        0 &  1.046341e-03 &  1.185261e-03 &  4.341587e-03 &  6.796760e-03 \\
176 &  5.954498e-03 &  1.026359e-02 &        0 &        0 &  1.158441e-03 &  3.378737e-03 &  5.480978e-03 &  3.065917e-03 \\
177 &  1.597677e-02 &  2.823196e-02 &        0 &        0 & -8.026006e-04 &  2.056054e-03 &  1.297050e-02 &  1.958243e-03 \\
178 &  2.954823e-02 &  4.785385e-02 &        0 &        0 & -1.952957e-03 &  2.062859e-03 &  7.253653e-03 & -4.351613e-03 \\
179 &  4.136372e-02 &  5.956445e-02 &        0 &        0 &  3.852578e-04 &  2.282116e-03 &  5.918319e-03 & -2.536634e-03 \\
180 &  4.497906e-02 &  5.729656e-02 &        0 &        0 & -3.811882e-04 &  1.073826e-03 &  4.023813e-03 &  1.730406e-02 \\
181 &  4.402591e-02 &  2.582410e-02 &        0 &        0 & -4.751830e-04 &  1.679792e-05 & -1.792017e-02 &  2.379920e-02 \\
182 &  3.998317e-02 & -1.535830e-02 &        0 &        0 & -7.009333e-04 &  1.693941e-03 & -3.119607e-02 &  6.046549e-03 \\
183 &  4.400987e-02 & -4.638144e-02 &        0 &        0 &  7.711938e-04 & -1.718202e-03 & -6.462783e-02 & -3.253711e-02 \\
184 &  5.277107e-02 & -5.871938e-02 &        0 &        0 & -8.181267e-04 &  5.408773e-05 & -7.078879e-02 & -5.781560e-02 \\
185 &  6.290146e-02 & -5.552335e-02 &        0 &        0 &  2.157449e-04 & -8.345176e-04 & -3.608721e-02 & -5.454916e-02 \\
186 &  7.117507e-02 & -5.207775e-02 &        0 &        0 &  1.857116e-04 &  1.128190e-03 & -3.973703e-03 & -3.586730e-02 \\
187 &  6.912736e-02 & -4.528825e-02 &        0 &        0 &  3.166423e-03 &  9.361180e-04 &  1.997296e-02 & -8.272251e-03 \\
188 &  5.536405e-02 & -3.595712e-02 &        0 &        0 &  1.335039e-04 & -1.096838e-03 &  1.867963e-02 &  4.029696e-03 \\
189 &  3.548228e-02 & -2.809117e-02 &        0 &        0 &  2.483543e-03 & -3.362994e-04 &  5.946322e-03 &  2.472171e-03 \\
190 &  1.911255e-02 & -1.681021e-02 &        0 &        0 &  3.583623e-04 & -3.646510e-04 &  2.445867e-03 & -3.896826e-04 \\
191 &  7.089838e-03 & -6.747206e-03 &        0 &        0 & -4.558504e-03 &  3.197279e-03 & -3.835447e-03 & -2.809574e-03 \\
192 &  9.676955e-04 & -1.084003e-03 &        0 &        0 &  3.304332e-03 & -2.308276e-03 &  1.009405e-03 & -2.924452e-05 \\
193 & -1.729580e-04 & -7.159271e-05 &        0 &        0 & -3.330285e-01 &  2.074625e-03 & -1.638582e-04 & -1.060954e-03 \\
194 & -1.647545e-04 & -6.819700e-05 &        0 &        0 & -3.330340e-01 &  2.074949e-03 & -1.562115e-04 & -1.010626e-03 \\
195 & -1.086969e-04 & -4.499304e-05 &        0 &        0 & -3.330342e-01 &  2.074270e-03 & -1.029567e-04 & -6.667668e-04 \\
196 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.540650e-06 & -8.877397e-08 & -1.211229e-07 &  1.323542e-08 \\
197 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -8.572121e-07 &  1.740215e-07 & -1.174523e-07 &  5.194669e-09 \\
198 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -8.933034e-07 &  1.023552e-07 &  1.298978e-08 & -3.744787e-09 \\
199 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.915184e-06 & -1.181459e-07 &  2.083433e-08 &  8.751443e-10 \\
200 &  1.633480e-04 &  1.098213e-04 &        0 &        0 & -9.470826e-05 & -2.830022e-03 & -1.423845e-04 &  7.907456e-04 \\
201 &  1.999829e-04 &  8.654845e-04 &        0 &        0 & -4.325034e-04 & -3.932451e-03 &  8.251949e-04 &  3.604597e-03 \\
202 &  2.062677e-04 &  2.838421e-03 &        0 &        0 & -1.816102e-04 & -7.430159e-03 &  2.268357e-03 &  7.610702e-03 \\
203 &  3.560550e-03 &  9.608643e-03 &        0 &        0 &  2.700015e-04 & -9.119778e-04 &  2.423499e-03 &  1.117979e-02 \\
204 &  1.367321e-02 &  2.788301e-02 &        0 &        0 &  1.374533e-04 & -1.002077e-03 &  7.251113e-03 &  1.755039e-02 \\
205 &  2.762204e-02 &  5.814557e-02 &        0 &        0 &  2.859023e-03 & -3.498501e-03 &  4.287824e-03 &  1.826161e-02 \\
206 &  3.864827e-02 &  8.256654e-02 &        0 &        0 & -1.049506e-03 & -3.451814e-04 & -6.795007e-03 &  3.026143e-02 \\
207 &  4.098186e-02 &  8.831630e-02 &        0 &        0 & -1.364629e-03 &  2.077215e-03 & -8.744647e-04 &  4.233880e-02 \\
208 &  3.480176e-02 &  6.551698e-02 &        0 &        0 &  1.847322e-03 & -2.991173e-03 & -3.952097e-03 &  4.342063e-02 \\
209 &  2.037823e-02 &  1.900853e-02 &        0 &        0 &  1.841113e-03 &  5.646355e-04 & -1.543435e-02 &  2.358329e-02 \\
210 &  1.382713e-02 & -1.780675e-02 &        0 &        0 & -1.555063e-03 &  1.461838e-03 & -4.686448e-02 & -2.001654e-02 \\
211 &  1.707932e-02 & -1.965568e-02 &        0 &        0 &  6.995866e-04 & -2.339385e-03 & -7.601619e-02 & -5.397042e-02 \\
212 &  2.773375e-02 & -1.499188e-03 &        0 &        0 & -6.616742e-04 &  9.388266e-04 & -5.500162e-02 & -5.993809e-02 \\
213 &  4.674119e-02 &  6.835313e-03 &        0 &        0 & -5.003101e-04 &  2.709551e-03 & -1.836281e-02 & -6.378187e-02 \\
214 &  6.547373e-02 &  4.576920e-04 &        0 &        0 &  9.038635e-04 & -1.682997e-03 &  3.445337e-02 & -4.568111e-02 \\
215 &  7.586307e-02 & -1.363796e-02 &        0 &        0 &  3.125358e-06 & -3.915097e-04 &  4.652636e-02 & -3.527774e-02 \\
216 &  7.234087e-02 & -2.209389e-02 &        0 &        0 & -2.584703e-03 &  2.830038e-03 &  3.919039e-02 & -1.121984e-02 \\
217 &  5.214218e-02 & -2.577104e-02 &        0 &        0 & -1.228526e-03 & -1.432320e-04 &  1.756778e-02 & -2.572298e-03 \\
218 &  2.927749e-02 & -1.850384e-02 &        0 &        0 & -5.112419e-03 & -1.873545e-04 &  7.544727e-03 & -3.049529e-03 \\
219 &  1.247424e-02 & -9.588668e-03 &        0 &        0 & -1.762360e-03 & -3.194369e-04 & -2.929522e-03 & -4.236961e-03 \\
220 &  2.515076e-03 & -2.292835e-03 &        0 &        0 & -1.252722e-03 &  1.675879e-03 & -1.764617e-03 & -4.701378e-04 \\
221 & -1.210022e-04 & -5.008660e-05 &        0 &        0 & -3.330351e-01 &  2.074161e-03 & -1.147376e-04 & -7.422456e-04 \\
222 & -1.497146e-04 & -6.197155e-05 &        0 &        0 & -3.330335e-01 &  2.074483e-03 & -1.418786e-04 & -9.183763e-04 \\
223 & -7.041373e-05 & -2.914644e-05 &        0 &        0 & -3.330366e-01 &  2.074667e-03 & -6.686384e-05 & -4.319261e-04 \\
224 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.394096e-06 &  1.229652e-07 &  8.625467e-09 & -8.524542e-11 \\
225 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.920370e-06 & -2.301995e-07 &  8.339582e-08 & -1.916029e-09 \\
226 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  3.833874e-07 &  6.895831e-09 & -1.296194e-07 &  7.554364e-09 \\
227 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.111779e-06 &  7.951871e-08 &  1.237015e-07 & -9.715264e-09 \\
228 &  3.110846e-05 &  3.627976e-04 &        0 &        0 & -3.296726e-05 & -3.122695e-03 &  5.746248e-04 &  1.692136e-03 \\
229 &  1.445993e-04 &  1.693849e-03 &        0 &        0 & -7.148435e-04 & -1.606920e-02 &  1.671311e-03 &  6.061115e-03 \\
230 &  1.581891e-03 &  7.520170e-03 &        0 &        0 & -4.059942e-04 &  7.058869e-03 &  1.768937e-03 &  1.528954e-02 \\
231 &  7.911462e-03 &  2.289063e-02 &        0 &        0 & -7.283118e-04 & -3.962751e-03 &  4.073594e-03 &  3.016097e-02 \\
232 &  2.375448e-02 &  5.589778e-02 &        0 &        0 &  2.939372e-04 &  9.910753e-04 &  8.501890e-04 &  3.432909e-02 \\
233 &  3.624391e-02 &  8.943530e-02 &        0 &        0 & -2.320082e-03 & -3.709033e-04 & -5.756453e-03 &  4.191432e-02 \\
234 &  4.280926e-02 &  1.062183e-01 &        0 &        0 & -1.433816e-06 & -1.389634e-03 & -2.487819e-02 &  3.205752e-02 \\
235 &  3.463758e-02 &  8.197383e-02 &        0 &        0 & -1.694896e-03 &  2.292871e-04 &  1.696186e-03 &  3.193365e-02 \\
236 &  1.841313e-02 &  2.013263e-02 &        0 &        0 & -4.466901e-03 & -1.259755e-04 &  1.565678e-02 &  4.541982e-03 \\
237 &  6.693173e-03 & -3.963560e-02 &        0 &        0 &  4.022034e-04 &  8.353032e-06 &  1.482049e-02 & -1.210389e-02 \\
238 &  6.309805e-03 & -5.636794e-02 &        0 &        0 & -4.097260e-04 &  4.131823e-04 & -5.108924e-02 & -3.023626e-02 \\
239 &  1.298399e-02 & -2.717078e-02 &        0 &        0 & -2.231179e-04 &  2.846380e-03 & -8.251674e-02 & -2.540407e-02 \\
240 &  1.834058e-02 &  1.331564e-02 &        0 &        0 &  4.642507e-04 & -3.076323e-03 & -5.974852e-02 & -6.451325e-03 \\
241 &  3.058347e-02 &  4.834010e-02 &        0 &        0 &  5.151253e-04 & -2.074180e-03 & -2.527254e-02 & -3.801698e-03 \\
242 &  4.952563e-02 &  4.569428e-02 &        0 &        0 & -1.314564e-03 & -6.543904e-04 &  1.833765e-02 & -2.269959e-02 \\
243 &  6.894904e-02 &  2.004893e-02 &        0 &        0 &  7.682583e-04 &  6.829166e-04 &  3.773534e-02 & -3.428463e-02 \\
244 &  8.144461e-02 & -1.943053e-03 &        0 &        0 & -5.329954e-04 & -2.867216e-03 &  4.190002e-02 & -1.703732e-02 \\
245 &  7.162280e-02 & -1.473838e-02 &        0 &        0 &  9.356454e-04 &  1.118364e-04 &  2.686175e-02 & -1.236046e-03 \\
246 &  4.548716e-02 & -1.646191e-02 &        0 &        0 &  6.917212e-04 &  1.340380e-03 &  1.654110e-02 & -1.142534e-03 \\
247 &  1.903851e-02 & -1.050544e-02 &        0 &        0 &  2.963209e-03 & -2.496292e-03 &  9.480309e-03 &  8.323608e-04 \\
248 &  4.887873e-03 & -3.474225e-03 &        0 &        0 & -1.240918e-04 & -3.019563e-03 & -2.951663e-03 & -2.252512e-03 \\
249 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.058169e-07 & -4.048667e-08 &  5.340847e-08 &  2.271822e-10 \\
250 & -2.255974e-05 & -9.338179e-06 &        0 &        0 & -3.330354e-01 &  2.074517e-03 & -2.133475e-05 & -1.383845e-04 \\
251 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  5.572289e-08 & -1.196328e-08 &  3.552475e-08 & -1.823892e-09 \\
252 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  6.218983e-08 & -7.617817e-09 & -5.132060e-08 &  1.878583e-09 \\
253 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.689455e-08 & -4.044146e-09 &  6.079932e-08 & -2.734316e-09 \\
254 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  7.905541e-08 & -2.158799e-08 & -4.490359e-08 &  8.560429e-09 \\
255 & -1.806227e-06 &  1.250097e-07 &        0 &        0 &  3.448362e-04 & -1.430228e-03 &  7.861483e-06 & -6.943262e-06 \\
256 & -4.261459e-05 &  4.237074e-04 &        0 &        0 &  5.447074e-05 & -3.223159e-03 &  1.064149e-03 &  1.718070e-03 \\
257 &  5.310753e-04 &  3.541684e-03 &        0 &        0 &  1.417715e-06 & -1.832521e-03 &  3.126766e-03 &  9.924595e-03 \\
258 &  5.954837e-03 &  1.749091e-02 &        0 &        0 &  1.088029e-03 & -2.196035e-04 &  3.869661e-03 &  2.858149e-02 \\
259 &  1.969940e-02 &  4.716677e-02 &        0 &        0 & -8.265622e-04 &  4.213155e-04 &  2.322419e-03 &  4.401073e-02 \\
260 &  3.445040e-02 &  8.439321e-02 &        0 &        0 &  2.682532e-03 &  8.597559e-04 & -6.537696e-03 &  4.525327e-02 \\
261 &  4.431605e-02 &  1.116138e-01 &        0 &        0 &  7.913464e-04 &  3.438147e-04 & -1.864804e-02 &  3.903097e-02 \\
262 &  4.190729e-02 &  9.422578e-02 &        0 &        0 &  1.079719e-04 &  7.329797e-04 &  3.650583e-03 &  1.187366e-02 \\
263 &  2.555445e-02 &  1.930650e-02 &        0 &        0 &  4.086408e-03 & -1.560559e-04 &  3.589655e-02 & -2.480209e-02 \\
264 &  9.662933e-03 & -6.476892e-02 &        0 &        0 & -5.979764e-05 & -8.371228e-04 &  4.845319e-02 & -3.650834e-02 \\
265 &  4.807615e-03 & -1.050871e-01 &        0 &        0 &  2.225947e-03 &  5.285093e-04 &  1.138881e-02 & -2.717272e-02 \\
266 &  9.841996e-03 & -8.677612e-02 &        0 &        0 &  8.223395e-04 & -3.641181e-03 & -5.840644e-02 & -1.727557e-02 \\
267 &  1.527816e-02 & -3.561874e-02 &        0 &        0 & -5.824441e-04 &  9.451511e-04 & -7.829180e-02 &  1.043160e-02 \\
268 &  1.611879e-02 &  1.910154e-02 &        0 &        0 & -1.161708e-03 &  2.148744e-03 & -7.198904e-02 &  2.317531e-02 \\
269 &  1.678727e-02 &  5.992321e-02 &        0 &        0 &  1.410073e-03 &  7.736559e-04 & -5.285788e-02 &  2.368499e-02 \\
270 &  2.486721e-02 &  6.122333e-02 &        0 &        0 &  2.862544e-03 &  5.007300e-04 & -1.685695e-02 & -8.778927e-03 \\
271 &  5.465794e-02 &  3.667302e-02 &        0 &        0 & -8.683327e-04 & -9.223246e-04 &  1.497725e-02 & -3.623649e-02 \\
272 &  8.324814e-02 &  1.037149e-02 &        0 &        0 & -5.243819e-04 & -4.244095e-04 &  2.495981e-02 & -1.991851e-02 \\
273 &  8.541441e-02 & -4.104093e-03 &        0 &        0 & -1.699577e-03 &  2.692053e-03 &  2.215441e-02 & -1.280052e-03 \\
274 &  6.426636e-02 & -8.927386e-03 &        0 &        0 &  1.477322e-03 &  3.500031e-04 &  1.319417e-02 &  5.559724e-03 \\
275 &  2.896006e-02 & -7.891782e-03 &        0 &        0 &  1.478500e-03 &  3.314983e-03 &  1.716590e-02 &  6.341982e-03 \\
276 &  6.790206e-03 & -4.099025e-03 &        0 &        0 &  3.975620e-03 &  1.132004e-03 & -1.499912e-04 & -7.045390e-04 \\
277 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.682899e-09 &  2.578314e-09 &  4.043099e-08 & -2.110141e-09 \\
278 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -9.487827e-09 &  4.644473e-09 &  7.930078e-08 & -5.313184e-09 \\
279 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -9.137552e-09 &  5.240198e-09 & -4.696747e-08 &  2.605716e-09 \\
280 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.499655e-09 &  2.258718e-10 & -8.291338e-08 &  2.335552e-09 \\
281 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.892518e-09 &  2.602129e-09 & -9.327347e-08 &  3.006471e-09 \\
282 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  4.977411e-09 & -3.290702e-09 &  3.202756e-08 &  8.059685e-10 \\
283 & -9.934250e-06 &  6.875536e-07 &        0 &        0 &  3.447432e-04 & -1.430285e-03 &  4.316576e-05 & -3.818724e-05 \\
284 & -2.608480e-04 &  8.097028e-04 &        0 &        0 &  3.605222e-04 & -2.514887e-03 &  1.846893e-03 &  2.051712e-03 \\
285 &  2.295603e-03 &  9.214676e-03 &        0 &        0 &  9.234138e-05 &  1.716369e-03 &  1.337772e-03 &  1.521547e-02 \\
286 &  1.374171e-02 &  3.164816e-02 &        0 &        0 &  4.464097e-05 &  8.162186e-04 &  4.234420e-03 &  3.888960e-02 \\
287 &  3.201368e-02 &  6.750541e-02 &        0 &        0 & -5.008596e-04 &  8.336045e-04 & -1.383214e-04 &  4.431162e-02 \\
288 &  4.773905e-02 &  1.035205e-01 &        0 &        0 &  1.103921e-03 & -2.473493e-03 & -1.154543e-02 &  5.074606e-02 \\
289 &  5.094931e-02 &  1.007151e-01 &        0 &        0 &  2.152268e-03 &  8.008409e-04 & -8.436937e-04 &  2.031589e-02 \\
290 &  3.568082e-02 &  3.623161e-02 &        0 &        0 & -3.235697e-03 &  9.319354e-04 &  3.805236e-02 & -2.752348e-02 \\
291 &  1.314764e-02 & -6.436143e-02 &        0 &        0 &  1.108672e-03 &  6.897462e-06 &  5.328288e-02 & -4.739227e-02 \\
292 &  3.803192e-03 & -1.284903e-01 &        0 &        0 & -1.297315e-03 & -4.867592e-04 &  2.723448e-02 & -3.121240e-02 \\
293 &  5.411465e-03 & -1.244492e-01 &        0 &        0 & -2.145442e-03 &  3.530008e-03 & -3.466862e-02 & -1.163196e-02 \\
294 &  1.214839e-02 & -7.476116e-02 &        0 &        0 &  1.946677e-03 & -1.516760e-03 & -5.409799e-02 &  1.987617e-03 \\
295 &  1.152507e-02 & -1.804701e-02 &        0 &        0 & -2.299484e-03 & -2.862993e-04 & -5.435665e-02 &  9.854037e-03 \\
296 &  3.177039e-03 &  3.126977e-02 &        0 &        0 &  1.339901e-03 &  7.033501e-04 & -7.088513e-02 &  1.083221e-02 \\
297 & -7.432576e-03 &  6.221650e-02 &        0 &        0 &  5.109363e-04 & -2.116267e-03 & -6.346058e-02 & -2.553493e-03 \\
298 & -2.387503e-03 &  6.538690e-02 &        0 &        0 & -5.269717e-03 & -1.540039e-04 & -1.469851e-02 & -2.185149e-02 \\
299 &  3.158190e-02 &  4.242299e-02 &        0 &        0 & -2.725374e-04 &  1.374430e-04 &  2.307544e-02 & -2.888899e-02 \\
300 &  7.561203e-02 &  1.212145e-02 &        0 &        0 &  2.191091e-04 &  8.751421e-04 &  1.660246e-02 & -2.239538e-02 \\
301 &  9.283560e-02 & -8.825709e-05 &        0 &        0 &  5.441554e-04 & -2.775922e-03 &  1.271394e-02 & -1.605421e-02 \\
302 &  7.764164e-02 & -1.871662e-03 &        0 &        0 &  1.686300e-03 & -2.509097e-03 &  1.728742e-02 &  2.967739e-03 \\
303 &  4.160391e-02 & -1.088519e-03 &        0 &        0 & -1.445355e-03 & -4.031709e-03 &  1.673255e-02 &  7.733135e-03 \\
304 &  9.140620e-03 & -1.918529e-03 &        0 &        0 & -1.257436e-03 & -1.559388e-03 &  9.486274e-03 &  2.641149e-03 \\
305 &  3.283541e-06 &  3.082218e-06 &        0 &        0 &  4.653427e-04 & -6.377570e-03 &  9.275117e-05 &  4.543985e-05 \\
306 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  3.806314e-11 & -2.531042e-11 &  6.330920e-08 & -4.988965e-09 \\
307 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  3.101849e-10 & -4.222915e-10 &  2.970729e-10 & -2.711964e-09 \\
308 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  4.194903e-10 & -5.712142e-10 &  8.307927e-08 & -4.638575e-09 \\
309 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.893499e-10 & -3.974474e-10 & -9.468487e-08 &  2.914904e-09 \\
310 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  4.495405e-11 & -6.400969e-11 & -4.252084e-08 &  1.658738e-09 \\
311 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.427996e-10 & -2.071250e-10 &  1.003530e-07 & -5.448976e-09 \\
312 &  9.021367e-05 &  1.655042e-03 &        0 &        0 &  4.667946e-05 &  1.049365e-03 &  1.193212e-03 &  4.591296e-03 \\
313 &  7.119709e-03 &  1.688933e-02 &        0 &        0 & -1.651997e-03 & -1.818392e-03 &  2.240244e-03 &  2.440642e-02 \\
314 &  2.533149e-02 &  4.840602e-02 &        0 &        0 &  7.826887e-04 &  7.038427e-04 &  1.060340e-02 &  4.378077e-02 \\
315 &  4.699944e-02 &  8.409439e-02 &        0 &        0 &  6.804135e-04 &  3.612798e-03 & -5.408709e-03 &  3.926397e-02 \\
316 &  5.935011e-02 &  1.025058e-01 &        0 &        0 &  3.735464e-05 & -3.380494e-04 & -1.375422e-02 &  4.805288e-02 \\
317 &  4.913115e-02 &  6.148479e-02 &        0 &        0 & -6.900237e-04 &  1.006212e-03 &  1.632095e-02 & -5.835551e-03 \\
318 &  2.129208e-02 & -3.832986e-02 &        0 &        0 &  6.747025e-04 & -1.536749e-03 &  4.789248e-02 & -4.504216e-02 \\
319 &  1.928455e-03 & -1.250854e-01 &        0 &        0 & -9.311208e-04 &  1.362280e-03 &  2.960985e-02 & -5.401256e-02 \\
320 & -6.284024e-03 & -1.414838e-01 &        0 &        0 &  3.002781e-03 & -2.771766e-03 & -2.978785e-02 & -2.567314e-02 \\
321 & -2.015484e-03 & -9.860569e-02 &        0 &        0 &  3.431272e-04 &  3.071664e-03 & -6.483474e-02 & -9.680042e-03 \\
322 &  5.192634e-04 & -3.773680e-02 &        0 &        0 & -6.990366e-04 & -1.940794e-04 & -6.023206e-02 & -9.201418e-04 \\
323 & -4.972070e-03 &  9.027911e-03 &        0 &        0 &  2.350723e-03 &  1.259484e-03 & -5.598185e-02 &  6.770221e-03 \\
324 & -2.224169e-02 &  4.372038e-02 &        0 &        0 & -9.541546e-04 & -3.127708e-03 & -6.570155e-02 & -1.308270e-02 \\
325 & -4.054789e-02 &  6.720367e-02 &        0 &        0 &  5.963654e-04 &  3.330359e-03 & -1.171449e-02 & -1.825992e-02 \\
326 & -3.135463e-02 &  5.834092e-02 &        0 &        0 &  1.991482e-04 &  6.659203e-04 &  7.480490e-02 & -3.751639e-03 \\
327 &  8.852872e-03 &  3.115750e-02 &        0 &        0 &  3.811205e-03 & -1.185686e-03 &  8.887692e-02 & -9.326388e-03 \\
328 &  6.436927e-02 &  9.921235e-04 &        0 &        0 & -8.429106e-04 &  2.964328e-03 &  5.794075e-02 & -1.172861e-02 \\
329 &  9.568454e-02 & -9.292675e-04 &        0 &        0 &  2.008078e-03 &  9.461651e-04 &  2.484212e-02 & -1.363999e-02 \\
330 &  8.855565e-02 &  5.073066e-03 &        0 &        0 & -6.359969e-04 &  1.378034e-03 &  1.949232e-02 &  9.675455e-04 \\
331 &  5.220304e-02 &  1.024418e-02 &        0 &        0 & -1.647666e-03 &  1.309493e-04 &  1.947443e-02 &  1.161638e-02 \\
332 &  1.265877e-02 &  3.293763e-03 &        0 &        0 & -4.042292e-04 &  4.087180e-03 &  1.585382e-02 &  8.257121e-03 \\
333 &  8.426079e-05 & -9.065419e-05 &        0 &        0 & -1.179499e-04 & -3.339266e-02 &  8.891412e-04 & -2.332682e-05 \\
334 &  8.892566e-05 & -2.353774e-04 &        0 &        0 & -4.869199e-05 &  4.284496e-03 & -2.787551e-04 & -1.272904e-03 \\
335 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -2.876848e-13 &  8.325562e-13 & -1.643925e-08 &  1.473074e-09 \\
336 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.014514e-12 & -6.634915e-12 &  2.152238e-08 & -7.799322e-10 \\
337 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  7.976610e-13 & -2.896350e-12 &  6.920368e-09 &  8.184623e-10 \\
338 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.606350e-13 &  5.838663e-13 & -3.370117e-08 &  1.889518e-09 \\
339 &  3.394577e-05 &  5.198202e-04 &        0 &        0 &  1.001373e-03 & -1.190282e-03 &  9.389286e-04 &  1.390320e-03 \\
340 &  1.054173e-03 &  3.408999e-03 &        0 &        0 &  9.695555e-04 & -7.055715e-04 &  1.579662e-03 &  7.048157e-03 \\
341 &  1.443340e-02 &  2.491737e-02 &        0 &        0 &  6.920073e-04 &  1.904665e-03 &  6.467785e-03 &  2.740233e-02 \\
342 &  3.981670e-02 &  6.056805e-02 &        0 &        0 &  3.211769e-05 & -1.232939e-03 &  2.165803e-02 &  4.963048e-02 \\
343 &  6.405361e-02 &  8.806523e-02 &        0 &        0 & -3.005410e-03 &  1.025157e-03 &  3.559193e-03 &  5.385785e-02 \\
344 &  6.787671e-02 &  8.123593e-02 &        0 &        0 & -1.183961e-05 & -1.477526e-03 & -1.454178e-02 &  4.991546e-02 \\
345 &  4.034511e-02 &  7.867119e-03 &        0 &        0 &  1.193566e-03 &  2.138199e-03 &  2.642663e-02 &  6.349962e-03 \\
346 &  4.948801e-03 & -8.995440e-02 &        0 &        0 &  1.409046e-04 &  4.278224e-03 &  3.191431e-02 & -5.543560e-02 \\
347 & -1.628813e-02 & -1.371429e-01 &        0 &        0 & -1.320023e-04 &  1.002292e-03 & -1.237431e-02 & -6.469528e-02 \\
348 & -2.295727e-02 & -1.116326e-01 &        0 &        0 & -3.117264e-03 & -2.318138e-04 & -6.712526e-02 & -5.201311e-02 \\
349 & -1.737069e-02 & -5.099845e-02 &        0 &        0 &  2.122857e-03 &  1.600711e-05 & -7.442311e-02 & -4.692288e-02 \\
350 & -1.723184e-02 & -3.762367e-03 &        0 &        0 & -1.851415e-03 & -1.800424e-03 & -5.412831e-02 & -3.222510e-02 \\
351 & -3.186261e-02 &  2.845457e-02 &        0 &        0 & -1.357090e-03 & -9.519552e-04 & -3.581537e-02 & -3.521795e-02 \\
352 & -5.665690e-02 &  4.994358e-02 &        0 &        0 &  1.738200e-03 &  8.967334e-04 &  1.920446e-02 & -4.058017e-02 \\
353 & -7.181438e-02 &  5.847855e-02 &        0 &        0 & -8.641849e-05 & -2.999043e-03 &  1.070399e-01 & -7.759040e-03 \\
354 & -5.496553e-02 &  3.177714e-02 &        0 &        0 &  4.699491e-04 & -1.416149e-03 &  1.835225e-01 &  2.921879e-02 \\
355 & -9.629146e-03 & -3.884601e-03 &        0 &        0 & -2.536080e-03 &  7.239886e-04 &  1.622572e-01 &  3.684858e-02 \\
356 &  5.530467e-02 & -2.645575e-02 &        0 &        0 & -8.104289e-04 & -2.410777e-03 &  1.052280e-01 &  2.246355e-02 \\
357 &  9.656842e-02 & -1.237363e-02 &        0 &        0 & -2.537642e-03 & -1.466548e-04 &  3.865400e-02 &  1.141925e-02 \\
358 &  9.407973e-02 &  9.507550e-03 &        0 &        0 &  2.808311e-03 & -2.010869e-03 &  2.810838e-02 & -1.068352e-03 \\
359 &  5.905179e-02 &  1.978160e-02 &        0 &        0 &  3.513560e-04 & -1.082444e-03 &  3.265530e-02 &  1.371437e-02 \\
360 &  1.637587e-02 &  9.386041e-03 &        0 &        0 &  7.511296e-04 & -1.680709e-03 &  2.668153e-02 &  1.325933e-02 \\
361 &  2.523526e-04 &  5.284368e-04 &        0 &        0 & -1.248632e-03 & -2.738061e-05 &  5.408828e-03 &  2.463824e-03 \\
362 &  7.089465e-05 & -1.876511e-04 &        0 &        0 & -4.796517e-05 &  4.311236e-03 & -2.222614e-04 & -1.014804e-03 \\
363 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -7.018518e-14 &  1.181431e-13 &  1.917513e-08 & -2.842632e-09 \\
364 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.585711e-14 & -1.882938e-13 & -1.062697e-07 &  7.564657e-09 \\
365 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -8.673184e-15 & -4.263256e-14 &  2.008751e-08 & -6.987144e-09 \\
366 &  1.679913e-06 & -5.367614e-05 &        0 &        0 &  2.008466e-05 &  8.018260e-05 & -7.848067e-06 &  1.229018e-04 \\
367 &  5.087579e-05 &  8.739209e-04 &        0 &        0 &  1.086917e-03 & -1.511564e-03 &  1.149212e-03 &  2.240253e-03 \\
368 &  2.941337e-03 &  4.445601e-03 &        0 &        0 & -1.988949e-03 &  1.544927e-03 &  2.701417e-03 &  9.552884e-03 \\
369 &  2.410312e-02 &  3.107291e-02 &        0 &        0 & -1.328090e-03 & -2.554024e-03 &  1.258650e-02 &  2.218098e-02 \\
370 &  5.698829e-02 &  6.230891e-02 &        0 &        0 &  1.524522e-03 & -5.910147e-04 &  1.765096e-02 &  4.180083e-02 \\
371 &  7.914471e-02 &  7.534517e-02 &        0 &        0 & -4.868814e-04 &  1.084716e-03 &  7.742519e-03 &  6.165962e-02 \\
372 &  6.720995e-02 &  4.703324e-02 &        0 &        0 & -1.267435e-03 &  2.390455e-03 & -8.782291e-03 &  8.262456e-02 \\
373 &  2.516440e-02 & -3.249910e-02 &        0 &        0 &  5.933461e-04 & -2.102458e-03 &  1.245462e-02 &  2.542218e-02 \\
374 & -1.837830e-02 & -1.066063e-01 &        0 &        0 &  7.594822e-04 & -7.519429e-04 &  1.085648e-02 & -5.586860e-02 \\
375 & -4.216498e-02 & -1.138195e-01 &        0 &        0 & -1.085200e-03 &  1.785359e-03 & -2.750037e-02 & -9.118893e-02 \\
376 & -4.290858e-02 & -6.557587e-02 &        0 &        0 &  5.186741e-04 & -1.368246e-03 & -6.448846e-02 & -9.829021e-02 \\
377 & -4.096203e-02 & -8.989020e-03 &        0 &        0 & -1.138959e-03 &  2.199795e-03 & -4.789848e-02 & -8.877319e-02 \\
378 & -4.983524e-02 &  1.870393e-02 &        0 &        0 & -1.021112e-03 &  3.114696e-03 & -1.130523e-02 & -8.326012e-02 \\
379 & -6.963342e-02 &  3.178837e-02 &        0 &        0 &  1.497677e-03 &  1.272745e-03 &  5.748000e-02 & -6.601096e-02 \\
380 & -8.858358e-02 &  4.065947e-02 &        0 &        0 & -5.188105e-06 &  1.079988e-03 &  1.052318e-01 & -4.019303e-02 \\
381 & -9.166698e-02 &  3.653282e-02 &        0 &        0 & -1.364595e-03 &  8.336072e-04 &  1.579255e-01 &  2.026652e-02 \\
382 & -6.479911e-02 & -1.440544e-03 &        0 &        0 &  8.657431e-04 &  1.759997e-03 &  2.055022e-01 &  7.269326e-02 \\
383 & -1.418123e-02 & -4.303752e-02 &        0 &        0 &  2.843114e-04 &  2.938638e-04 &  1.773798e-01 &  8.227683e-02 \\
384 &  5.123211e-02 & -5.927086e-02 &        0 &        0 &  7.596206e-04 &  2.736790e-04 &  1.069700e-01 &  4.984830e-02 \\
385 &  9.362461e-02 & -2.870327e-02 &        0 &        0 &  1.668972e-03 & -1.014649e-03 &  6.099442e-02 &  2.909731e-02 \\
386 &  9.408389e-02 &  9.074626e-03 &        0 &        0 & -3.732744e-03 &  2.894457e-03 &  4.062576e-02 &  7.936327e-03 \\
387 &  6.190191e-02 &  2.736711e-02 &        0 &        0 &  6.429803e-04 &  1.186565e-03 &  3.804639e-02 &  9.027033e-03 \\
388 &  1.885906e-02 &  1.522800e-02 &        0 &        0 &  1.226231e-03 & -2.317789e-03 &  3.101236e-02 &  1.349153e-02 \\
389 &  1.770217e-04 &  1.739068e-03 &        0 &        0 &  4.110445e-05 & -3.691252e-02 &  1.309443e-02 &  5.521161e-03 \\
390 & -1.675360e-05 &  6.985465e-07 &        0 &        0 &  4.690168e-04 &  1.918514e-03 &  3.004705e-04 & -1.140415e-04 \\
391 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.082523e-15 &  3.530509e-14 &  1.308733e-09 &  6.475747e-10 \\
392 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -8.253131e-14 & -1.865175e-14 &  5.323647e-08 & -1.545930e-09 \\
393 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  4.786471e-14 &  5.573320e-14 &  2.276999e-08 & -4.046535e-09 \\
394 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.547330e-14 & -5.773160e-15 & -8.233961e-08 &  3.561520e-09 \\
395 &  7.047424e-05 &  9.620907e-04 &        0 &        0 &  1.239601e-03 & -2.252831e-03 &  1.135816e-03 &  2.671452e-03 \\
396 &  6.155614e-03 &  5.076918e-03 &        0 &        0 &  2.363839e-03 & -4.084481e-03 &  1.510468e-03 &  9.373838e-03 \\
397 &  3.754922e-02 &  3.300558e-02 &        0 &        0 &  2.559410e-04 &  4.370749e-04 &  1.141429e-02 &  2.040490e-02 \\
398 &  7.483877e-02 &  5.442253e-02 &        0 &        0 & -3.724503e-04 & -2.340446e-03 &  1.739043e-02 &  3.265059e-02 \\
399 &  9.124810e-02 &  5.169285e-02 &        0 &        0 &  9.757185e-04 & -2.854992e-03 &  2.033454e-02 &  7.407818e-02 \\
400 &  6.649142e-02 &  1.032217e-02 &        0 &        0 &  8.716695e-04 &  5.197888e-04 &  1.342835e-02 &  1.216342e-01 \\
401 &  7.966177e-03 & -5.940281e-02 &        0 &        0 &  1.141338e-03 & -3.845328e-03 &  1.349253e-02 &  7.797067e-02 \\
402 & -4.388661e-02 & -9.285210e-02 &        0 &        0 &  1.457446e-03 & -3.155484e-03 &  6.637399e-03 & -4.335700e-03 \\
403 & -6.672558e-02 & -6.563930e-02 &        0 &        0 &  9.208409e-04 & -1.348386e-03 & -2.539854e-02 & -7.303393e-02 \\
404 & -6.467824e-02 & -1.334170e-02 &        0 &        0 & -3.446620e-04 & -1.111286e-03 & -3.362788e-02 & -9.501843e-02 \\
405 & -6.434286e-02 &  1.844590e-02 &        0 &        0 &  1.199259e-04 &  5.089864e-04 &  2.365603e-02 & -6.558445e-02 \\
406 & -7.642489e-02 &  2.107651e-02 &        0 &        0 &  7.554759e-04 & -2.613478e-03 &  8.594591e-02 & -4.236576e-02 \\
407 & -9.292521e-02 &  1.698781e-02 &        0 &        0 & -2.941204e-03 & -1.849305e-03 &  1.210878e-01 & -3.000837e-02 \\
408 & -1.048330e-01 &  2.177048e-02 &        0 &        0 &  8.788072e-04 & -6.969195e-04 &  9.261796e-02 & -1.307029e-02 \\
409 & -9.697084e-02 &  1.119570e-02 &        0 &        0 &  1.437833e-03 &  8.661213e-05 &  9.078093e-02 &  5.545717e-02 \\
410 & -5.813400e-02 & -2.703690e-02 &        0 &        0 & -4.207809e-04 &  9.281782e-05 &  1.258986e-01 &  1.100682e-01 \\
411 & -4.154117e-03 & -7.154266e-02 &        0 &        0 & -8.484168e-04 &  1.349793e-03 &  1.023683e-01 &  9.404501e-02 \\
412 &  5.266117e-02 & -8.154171e-02 &        0 &        0 &  2.120215e-03 & -2.644981e-03 &  8.404663e-02 &  6.298895e-02 \\
413 &  9.126633e-02 & -3.512783e-02 &        0 &        0 & -8.521765e-04 &  1.610960e-03 &  5.896873e-02 &  3.375898e-02 \\
414 &  8.972638e-02 &  1.218361e-02 &        0 &        0 &  1.660634e-03 &  2.672932e-03 &  4.901550e-02 &  1.603128e-02 \\
415 &  6.018858e-02 &  3.326566e-02 &        0 &        0 & -7.765975e-04 &  7.531458e-04 &  4.002262e-02 &  5.962771e-03 \\
416 &  1.826655e-02 &  1.882445e-02 &        0 &        0 & -4.793815e-04 &  4.953023e-03 &  2.996142e-02 &  9.383226e-03 \\
417 &  4.253158e-04 &  2.588469e-03 &        0 &        0 &  3.021855e-04 & -6.680737e-03 &  1.542642e-02 &  6.304099e-03 \\
418 & -2.974750e-05 &  2.669853e-05 &        0 &        0 &  5.176454e-04 & -2.384990e-03 &  3.888995e-04 &  3.904995e-06 \\
419 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.521029e-15 & -3.411160e-14 & -6.633219e-10 &  1.434882e-09 \\
420 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.093551e-14 &  2.556289e-14 &  7.343070e-08 &  1.714395e-09 \\
421 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -4.576672e-14 &  4.307665e-14 &  2.513641e-09 &  1.351904e-09 \\
422 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.038056e-15 &  7.049916e-15 & -1.429997e-08 &  1.821348e-09 \\
423 &  1.552190e-05 &  3.339610e-04 &        0 &        0 &  6.428742e-04 & -4.368280e-04 &  1.252092e-03 &  1.241839e-03 \\
424 &  8.975598e-03 &  4.179106e-03 &        0 &        0 & -1.391411e-05 &  2.824727e-03 & -2.363765e-03 &  5.062837e-03 \\
425 &  4.945257e-02 &  2.888740e-02 &        0 &        0 & -1.137947e-03 & -3.228132e-03 &  6.647832e-03 &  8.240044e-03 \\
426 &  8.826920e-02 &  3.913028e-02 &        0 &        0 &  2.620996e-03 &  2.883815e-03 &  1.079858e-02 &  2.387390e-02 \\
427 &  9.945629e-02 &  1.974491e-02 &        0 &        0 &  1.705262e-03 & -1.713752e-03 &  3.393180e-02 &  7.454532e-02 \\
428 &  6.258743e-02 & -2.423454e-02 &        0 &        0 &  4.356440e-04 & -6.415647e-03 &  3.775252e-02 &  1.348746e-01 \\
429 & -5.483893e-03 & -7.016266e-02 &        0 &        0 & -2.696846e-03 &  1.437217e-03 &  2.780699e-02 &  1.306406e-01 \\
430 & -5.949497e-02 & -6.743303e-02 &        0 &        0 & -1.136007e-03 &  1.691109e-03 &  1.174251e-02 &  7.647695e-02 \\
431 & -7.522377e-02 & -2.589140e-02 &        0 &        0 &  1.368637e-03 &  5.573597e-04 & -1.131786e-02 &  2.165051e-02 \\
432 & -7.258667e-02 &  9.027635e-03 &        0 &        0 &  2.597185e-03 & -2.445974e-03 &  2.020319e-02 &  2.012077e-02 \\
433 & -7.186759e-02 &  1.529342e-02 &        0 &        0 &  2.722647e-03 &  5.252034e-04 &  8.949503e-02 &  4.728324e-02 \\
434 & -7.908519e-02 &  6.369938e-03 &        0 &        0 & -1.288251e-03 &  5.664493e-04 &  1.438367e-01 &  4.550830e-02 \\
435 & -9.227256e-02 &  4.919094e-03 &        0 &        0 &  5.411641e-04 &  1.069374e-03 &  1.092353e-01 & -2.729245e-03 \\
436 & -1.017815e-01 &  1.328809e-02 &        0 &        0 & -3.414323e-04 &  3.561837e-04 &  1.073276e-02 & -5.622070e-03 \\
437 & -8.529941e-02 & -2.592090e-03 &        0 &        0 & -5.466641e-04 & -2.613007e-03 & -2.365645e-02 &  7.780957e-02 \\
438 & -4.165669e-02 & -4.746339e-02 &        0 &        0 & -1.331552e-03 &  5.738230e-04 &  3.543055e-03 &  1.188137e-01 \\
439 &  1.314376e-02 & -9.107648e-02 &        0 &        0 &  1.381850e-04 & -2.692647e-03 &  2.889005e-02 &  8.790791e-02 \\
440 &  5.901622e-02 & -8.828631e-02 &        0 &        0 & -1.666101e-03 &  4.396004e-03 &  5.527091e-02 &  4.187095e-02 \\
441 &  8.755210e-02 & -3.237145e-02 &        0 &        0 & -7.732441e-04 & -8.965144e-04 &  4.930920e-02 &  2.263316e-02 \\
442 &  8.145104e-02 &  2.023001e-02 &        0 &        0 &  7.142622e-04 & -3.510319e-03 &  4.998257e-02 &  1.871264e-02 \\
443 &  5.234840e-02 &  3.760151e-02 &        0 &        0 & -2.691638e-03 &  4.077927e-04 &  4.369785e-02 &  1.247844e-02 \\
444 &  1.604047e-02 &  2.113886e-02 &        0 &        0 & -4.760873e-04 &  9.819434e-05 &  2.916180e-02 &  8.108988e-03 \\
445 &  2.678692e-04 &  2.366619e-03 &        0 &        0 &  3.095721e-04 &  4.843874e-03 &  1.220213e-02 &  5.238632e-03 \\
446 & -6.409453e-05 &  2.465914e-05 &        0 &        0 &  6.117222e-04 & -2.553222e-03 &  5.194436e-04 & -6.603766e-05 \\
447 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.196467e-14 &  2.423062e-14 & -6.588246e-08 &  6.966436e-09 \\
448 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.088781e-14 &  2.478573e-14 &  6.653909e-09 &  1.873139e-09 \\
449 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.379306e-14 &  1.082467e-14 &  6.211260e-08 & -3.399521e-09 \\
450 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -1.184816e-15 &  1.561251e-15 &  5.237483e-08 & -3.620861e-09 \\
451 &  1.835935e-05 &  9.192500e-05 &        0 &        0 & -1.491575e-04 &  6.831004e-04 &  1.998035e-04 &  5.103247e-04 \\
452 &  1.251791e-02 &  2.291253e-03 &        0 &        0 & -1.433576e-03 &  1.437001e-03 & -3.128047e-03 &  3.452153e-03 \\
453 &  5.871765e-02 &  1.890334e-02 &        0 &        0 &  1.790948e-03 &  1.726467e-04 &  2.667678e-03 & -3.466038e-03 \\
454 &  9.654511e-02 &  2.085875e-02 &        0 &        0 & -4.314712e-03 & -6.275796e-04 &  2.790234e-04 &  6.296103e-03 \\
455 &  1.042438e-01 & -8.126556e-03 &        0 &        0 & -1.015425e-03 &  5.391172e-04 &  2.561355e-02 &  4.955279e-02 \\
456 &  6.249088e-02 & -5.232127e-02 &        0 &        0 & -5.307908e-04 &  6.098284e-03 &  4.769351e-02 &  1.161810e-01 \\
457 & -7.622896e-03 & -7.522218e-02 &        0 &        0 &  1.524682e-03 &  1.154359e-03 &  4.267692e-02 &  1.449393e-01 \\
458 & -5.819822e-02 & -5.080258e-02 &        0 &        0 &  2.733057e-04 & -1.900949e-03 &  2.972417e-02 &  1.361820e-01 \\
459 & -7.062684e-02 & -1.260941e-02 &        0 &        0 & -2.002287e-03 &  1.222468e-03 &  1.496157e-02 &  1.101789e-01 \\
460 & -6.535696e-02 &  2.360584e-03 &        0 &        0 & -1.962480e-03 &  1.783913e-03 &  5.572710e-02 &  1.126120e-01 \\
461 & -6.417512e-02 & -6.514237e-03 &        0 &        0 & -7.367611e-04 &  1.399188e-04 &  1.082934e-01 &  1.032422e-01 \\
462 & -7.112499e-02 & -1.059700e-02 &        0 &        0 & -1.621861e-03 &  6.331979e-04 &  1.364435e-01 &  4.141692e-02 \\
463 & -8.404058e-02 &  4.523773e-03 &        0 &        0 & -5.445309e-04 & -1.708710e-04 &  7.404847e-02 & -3.143293e-02 \\
464 & -8.427049e-02 &  1.561993e-02 &        0 &        0 & -1.752419e-05 &  2.009065e-03 & -4.835180e-02 & -3.958389e-03 \\
465 & -6.015368e-02 & -1.013316e-02 &        0 &        0 &  4.833478e-04 &  4.370816e-04 & -1.060041e-01 &  9.220837e-02 \\
466 & -1.879203e-02 & -6.710143e-02 &        0 &        0 & -4.236634e-04 &  1.653237e-03 & -6.917089e-02 &  1.223003e-01 \\
467 &  3.021051e-02 & -1.049629e-01 &        0 &        0 &  1.182523e-03 &  3.782896e-03 & -5.239546e-03 &  7.089381e-02 \\
468 &  6.689114e-02 & -8.413442e-02 &        0 &        0 & -4.800647e-05 & -1.581293e-03 &  3.358972e-02 &  2.290347e-02 \\
469 &  8.356363e-02 & -1.754263e-02 &        0 &        0 & -9.169920e-04 &  1.037583e-03 &  5.244015e-02 &  2.153821e-02 \\
470 &  7.197319e-02 &  3.093720e-02 &        0 &        0 & -2.986810e-04 &  4.339747e-04 &  4.892055e-02 &  1.712547e-02 \\
471 &  4.202402e-02 &  3.778506e-02 &        0 &        0 &  3.502005e-03 & -1.758937e-05 &  4.263928e-02 &  1.426343e-02 \\
472 &  1.222199e-02 &  1.866686e-02 &        0 &        0 & -1.502453e-03 &  2.072321e-03 &  2.879004e-02 &  1.168507e-02 \\
473 &  1.698400e-04 &  1.736448e-03 &        0 &        0 &  4.990044e-04 &  5.017016e-02 &  7.960656e-03 &  3.819300e-03 \\
474 & -1.679294e-05 &  1.507175e-05 &        0 &        0 &  5.176633e-04 & -2.385132e-03 &  2.195055e-04 &  2.205759e-06 \\
475 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.596068e-15 &  3.594347e-15 & -3.758148e-08 & -1.135080e-10 \\
476 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  2.940790e-15 &  5.551115e-16 &  4.962965e-08 & -1.412920e-09 \\
477 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -5.313106e-15 &  5.551115e-17 & -2.301501e-08 &  2.902054e-09 \\
478 & -4.733328e-05 & -4.117867e-06 &        0 &        0 &  3.821563e-04 & -1.167173e-03 &  1.097574e-04 & -1.392186e-04 \\
479 &  3.655494e-05 &  1.668981e-04 &        0 &        0 &  5.911663e-04 & -1.232225e-03 &  3.312102e-04 &  6.219562e-04 \\
480 &  1.570415e-02 & -1.010323e-03 &        0 &        0 &  1.628386e-03 & -7.352694e-04 & -1.997290e-03 &  4.459661e-03 \\
481 &  6.387308e-02 &  5.977167e-03 &        0 &        0 &  2.315333e-03 & -2.760068e-03 & -6.421312e-03 & -3.118703e-03 \\
482 &  9.978635e-02 &  2.889507e-03 &        0 &        0 &  4.311686e-03 & -6.881288e-04 & -9.429502e-03 & -8.414627e-04 \\
483 &  1.055375e-01 & -2.755674e-02 &        0 &        0 & -7.002536e-05 &  1.040764e-03 &  1.182283e-02 &  1.903610e-02 \\
484 &  6.654498e-02 & -6.731434e-02 &        0 &        0 &  8.719087e-04 & -3.308632e-03 &  3.560955e-02 &  5.400069e-02 \\
485 &  3.715792e-03 & -8.228020e-02 &        0 &        0 & -9.730253e-04 & -2.469982e-03 &  3.560565e-02 &  8.700671e-02 \\
486 & -4.482330e-02 & -5.763650e-02 &        0 &        0 & -1.617515e-04 &  3.507599e-03 &  3.660234e-02 &  1.069420e-01 \\
487 & -5.595698e-02 & -3.172330e-02 &        0 &        0 & -6.041759e-04 & -5.724546e-04 &  4.564052e-02 &  1.142846e-01 \\
488 & -5.290929e-02 & -2.567270e-02 &        0 &        0 &  3.792917e-04 & -9.360762e-04 &  6.375174e-02 &  9.501294e-02 \\
489 & -5.363413e-02 & -2.541235e-02 &        0 &        0 &  3.765390e-05 & -1.871644e-04 &  1.010997e-01 &  4.540408e-02 \\
490 & -6.292798e-02 & -1.650317e-02 &        0 &        0 &  5.594425e-04 &  1.365171e-04 &  1.172910e-01 & -3.427896e-02 \\
491 & -6.985920e-02 &  2.394593e-04 &        0 &        0 &  4.657724e-03 & -1.461815e-03 &  3.760963e-02 & -6.591169e-02 \\
492 & -6.315657e-02 & -3.499765e-03 &        0 &        0 & -2.629017e-03 & -1.347953e-03 & -8.456082e-02 &  9.001401e-03 \\
493 & -3.610494e-02 & -4.286476e-02 &        0 &        0 &  7.438028e-05 &  1.481621e-03 & -1.267909e-01 &  1.028152e-01 \\
494 &  8.405211e-03 & -8.886580e-02 &        0 &        0 &  2.705404e-03 & -2.354368e-03 & -7.106006e-02 &  1.162088e-01 \\
495 &  4.663673e-02 & -9.983920e-02 &        0 &        0 & -1.354154e-03 &  8.881547e-04 & -6.162898e-03 &  5.779401e-02 \\
496 &  7.408325e-02 & -5.546932e-02 &        0 &        0 &  9.789323e-04 & -1.427635e-03 &  4.323297e-02 &  2.448165e-02 \\
497 &  7.496817e-02 &  8.368039e-03 &        0 &        0 &  8.345918e-04 & -2.396345e-04 &  5.200142e-02 &  1.928316e-02 \\
498 &  5.926795e-02 &  4.044215e-02 &        0 &        0 &  6.218130e-05 & -2.003489e-03 &  4.468480e-02 &  1.479464e-02 \\
499 &  3.018331e-02 &  3.296365e-02 &        0 &        0 & -1.248869e-03 &  1.643801e-03 &  3.527339e-02 &  1.348962e-02 \\
500 &  8.919220e-03 &  1.463303e-02 &        0 &        0 &  3.457112e-03 & -1.482336e-02 &  1.640582e-02 &  4.542906e-03 \\
501 & -6.875459e-05 &  9.420421e-04 &        0 &        0 &  1.851976e-03 &  1.668053e-01 &  3.753813e-03 &  2.122002e-03 \\
502 & -8.994523e-05 & -2.192261e-04 &        0 &        0 &  2.878012e-04 & -1.013412e-03 & -2.983517e-05 &  2.199744e-05 \\
503 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  1.140488e-17 & -1.703498e-15 &  5.994644e-08 & -4.919619e-09 \\
504 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -4.452475e-18 &  1.734723e-17 &  7.580798e-08 & -6.474655e-09 \\
505 &  0.000000e+00 &  0.000000e+00 &        0 &        0 & -3.227672e-18 & -1.077263e-15 & -9.573381e-08 &  5.013980e-09 \\
506 & -1.092968e-04 & -9.508529e-06 &        0 &        0 &  3.821723e-04 & -1.167217e-03 &  2.533614e-04 & -3.214731e-04 \\
507 &  1.167069e-04 &  2.542459e-04 &        0 &        0 &  3.769310e-04 & -3.841156e-04 &  1.036793e-03 &  7.969993e-04 \\
508 &  1.664089e-02 & -5.159323e-03 &        0 &        0 &  1.075477e-03 & -4.520919e-04 & -1.433112e-03 &  5.228739e-03 \\
509 &  6.089805e-02 & -4.493551e-03 &        0 &        0 & -5.373320e-03 &  5.007039e-04 & -2.815471e-03 &  1.032560e-02 \\
510 &  9.862495e-02 & -1.063295e-02 &        0 &        0 & -7.980557e-04 &  1.399916e-03 & -1.592140e-02 &  1.737102e-03 \\
511 &  1.067131e-01 & -3.594152e-02 &        0 &        0 & -1.301948e-03 & -1.699238e-03 & -9.896808e-03 &  1.284851e-04 \\
512 &  7.437911e-02 & -6.654551e-02 &        0 &        0 & -3.804326e-04 &  2.144322e-03 &  1.840956e-02 &  8.824546e-03 \\
513 &  1.850121e-02 & -8.262182e-02 &        0 &        0 &  3.210795e-04 &  9.583763e-04 &  1.369389e-02 &  1.571241e-02 \\
514 & -2.599462e-02 & -7.138437e-02 &        0 &        0 &  8.502654e-04 & -2.658723e-03 &  1.526110e-02 &  3.614291e-02 \\
515 & -4.285949e-02 & -5.735453e-02 &        0 &        0 & -2.393164e-04 & -5.508754e-04 &  3.650518e-02 &  5.187842e-02 \\
516 & -4.314758e-02 & -5.065374e-02 &        0 &        0 &  1.156516e-03 &  5.671604e-04 &  6.425516e-02 &  3.118350e-02 \\
517 & -4.559122e-02 & -4.500940e-02 &        0 &        0 & -1.350221e-03 &  3.009991e-04 &  1.014660e-01 & -3.507495e-02 \\
518 & -5.560814e-02 & -3.327654e-02 &        0 &        0 & -1.710049e-03 &  2.115096e-03 &  1.051625e-01 & -9.739117e-02 \\
519 & -5.465414e-02 & -2.717692e-02 &        0 &        0 &  1.381755e-03 &  4.550644e-04 &  2.374860e-02 & -7.335103e-02 \\
520 & -3.873710e-02 & -4.211559e-02 &        0 &        0 &  7.477672e-04 & -2.116296e-03 & -7.403780e-02 &  4.115605e-02 \\
521 & -4.467340e-03 & -7.719328e-02 &        0 &        0 & -2.286714e-03 &  9.229425e-04 & -9.502209e-02 &  1.182323e-01 \\
522 &  3.210299e-02 & -9.052169e-02 &        0 &        0 & -2.322935e-03 &  1.712680e-03 & -3.133666e-02 &  1.147203e-01 \\
523 &  6.222136e-02 & -6.353747e-02 &        0 &        0 &  1.961316e-03 & -1.493485e-03 &  1.462016e-02 &  5.626141e-02 \\
524 &  7.369980e-02 & -8.788007e-03 &        0 &        0 & -3.527079e-03 &  3.549405e-03 &  3.423472e-02 &  1.914760e-02 \\
525 &  6.453579e-02 &  3.327574e-02 &        0 &        0 &  1.389495e-03 &  1.102241e-04 &  3.880842e-02 &  1.312999e-02 \\
526 &  4.184823e-02 &  3.873306e-02 &        0 &        0 &  1.580926e-03 & -1.179459e-03 &  3.531051e-02 &  1.515602e-02 \\
527 &  1.833588e-02 &  2.475372e-02 &        0 &        0 & -6.360094e-04 & -5.522450e-03 &  2.662821e-02 &  9.201355e-03 \\
528 &  4.689209e-03 &  8.677916e-03 &        0 &        0 & -1.762278e-03 &  1.431052e-02 &  9.060953e-03 &  4.071566e-04 \\
529 &  4.731361e-05 &  5.471998e-04 &        0 &        0 &  1.356520e-03 &  8.789641e-02 &  1.159457e-03 &  1.647418e-04 \\
530 & -2.969890e-05 & -7.238598e-05 &        0 &        0 &  2.878026e-04 & -1.013728e-03 & -9.843333e-06 &  7.256855e-06 \\
531 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 &  2.802597e-45 & -6.452252e-09 &  2.152193e-09 \\
532 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -2.802597e-45 &  1.083612e-07 & -6.778332e-09 \\
533 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -1.401298e-45 & -3.919220e-08 &  3.167593e-10 \\
534 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.526075e-08 & -8.072021e-10 \\
535 &  3.015029e-04 & -3.913412e-05 &        0 &        0 & -3.792841e-04 & -2.147494e-04 &  1.433987e-03 &  1.147170e-03 \\
536 &  1.513378e-02 & -7.389832e-03 &        0 &        0 & -1.170938e-03 &  1.493678e-03 &  2.822272e-03 &  7.575968e-03 \\
537 &  5.354056e-02 & -1.195368e-02 &        0 &        0 &  2.111004e-03 & -1.773393e-04 & -2.114698e-03 &  1.921924e-02 \\
538 &  9.206271e-02 & -1.825214e-02 &        0 &        0 & -2.461146e-03 &  7.797713e-04 & -1.564450e-02 &  1.717155e-02 \\
539 &  1.069718e-01 & -3.536912e-02 &        0 &        0 & -1.332844e-03 &  3.182423e-03 & -2.172929e-02 & -5.476470e-03 \\
540 &  8.663077e-02 & -5.651402e-02 &        0 &        0 &  7.517337e-04 & -1.541406e-03 & -6.473602e-03 & -1.293038e-02 \\
541 &  4.459374e-02 & -7.724975e-02 &        0 &        0 & -1.848963e-03 & -2.794492e-05 & -1.179940e-02 & -1.914289e-02 \\
542 &  1.743510e-05 & -8.755506e-02 &        0 &        0 & -3.402084e-04 &  1.340803e-03 & -1.600692e-02 & -1.806448e-02 \\
543 & -2.625140e-02 & -8.673329e-02 &        0 &        0 &  3.758317e-03 & -7.340623e-04 &  5.627319e-03 & -1.478347e-02 \\
544 & -3.549173e-02 & -8.053965e-02 &        0 &        0 & -4.014035e-03 & -7.284177e-05 &  4.999922e-02 & -4.377525e-02 \\
545 & -3.936584e-02 & -7.175879e-02 &        0 &        0 &  1.087721e-03 & -4.488376e-04 &  9.520855e-02 & -9.342488e-02 \\
546 & -4.216276e-02 & -6.271973e-02 &        0 &        0 & -8.057453e-04 & -1.586996e-03 &  8.843812e-02 & -1.015934e-01 \\
547 & -3.111870e-02 & -6.684348e-02 &        0 &        0 &  2.369415e-03 &  3.507957e-03 &  1.329267e-02 & -3.780579e-02 \\
548 & -6.009239e-03 & -8.061607e-02 &        0 &        0 & -1.234991e-03 &  7.863627e-04 & -5.005477e-02 &  7.106778e-02 \\
549 &  2.207684e-02 & -8.137575e-02 &        0 &        0 &  1.726303e-03 & -3.599152e-03 & -5.788976e-02 &  1.213873e-01 \\
550 &  5.226185e-02 & -5.653498e-02 &        0 &        0 &  1.416340e-03 & -2.074750e-03 & -1.451047e-02 &  9.441392e-02 \\
551 &  6.770914e-02 & -5.122440e-03 &        0 &        0 &  1.757754e-03 & -7.145692e-04 &  1.911321e-02 &  5.648038e-02 \\
552 &  6.351522e-02 &  2.960469e-02 &        0 &        0 &  1.870087e-03 & -2.028304e-06 &  3.242603e-02 &  2.569711e-02 \\
553 &  4.881008e-02 &  4.113525e-02 &        0 &        0 & -6.250195e-04 &  1.571972e-03 &  2.357210e-02 &  1.133008e-02 \\
554 &  2.484706e-02 &  3.031299e-02 &        0 &        0 &  9.434856e-04 &  4.051698e-03 &  2.356984e-02 &  9.266119e-03 \\
555 &  9.057751e-03 &  1.631278e-02 &        0 &        0 & -2.366512e-04 &  5.369901e-03 &  1.898476e-02 &  7.285004e-03 \\
556 &  1.692447e-03 &  3.996990e-03 &        0 &        0 &  1.058079e-03 &  6.988393e-03 &  2.841115e-03 & -7.218140e-04 \\
557 &  9.884901e-06 &  2.415829e-04 &        0 &        0 &  3.066746e-04 & -4.189415e-02 &  2.480092e-04 &  8.240875e-05 \\
558 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.938989e-09 &  2.514616e-09 \\
559 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  6.143833e-08 & -2.395364e-09 \\
560 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.081817e-07 & -6.037663e-09 \\
561 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -8.435053e-09 &  5.677739e-10 \\
562 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  7.014317e-08 & -3.867889e-09 \\
563 &  2.429149e-04 &  9.168965e-05 &        0 &        0 &  1.073085e-04 & -2.495466e-04 &  1.462135e-03 &  6.230116e-04 \\
564 &  1.111912e-02 & -6.530898e-03 &        0 &        0 &  1.329734e-03 &  1.765625e-05 &  6.081211e-03 &  7.168315e-03 \\
565 &  3.802970e-02 & -1.631011e-02 &        0 &        0 & -8.874123e-04 & -2.573819e-04 &  5.764994e-03 &  2.021528e-02 \\
566 &  7.792551e-02 & -2.318908e-02 &        0 &        0 & -1.049686e-03 & -8.009258e-06 & -1.494157e-02 &  3.053182e-02 \\
567 &  1.023534e-01 & -3.292897e-02 &        0 &        0 &  3.201089e-03 & -5.385852e-03 & -1.995995e-02 &  1.284824e-02 \\
568 &  1.007139e-01 & -4.649306e-02 &        0 &        0 & -4.826927e-04 &  1.443185e-03 & -2.548127e-02 & -1.659797e-02 \\
569 &  7.821464e-02 & -6.977331e-02 &        0 &        0 &  1.260943e-03 &  6.673170e-04 & -4.260272e-02 & -4.178394e-02 \\
570 &  4.158062e-02 & -9.426947e-02 &        0 &        0 & -1.937611e-03 & -8.037576e-05 & -4.867382e-02 & -4.850748e-02 \\
571 &  1.225991e-02 & -1.069838e-01 &        0 &        0 &  3.682945e-04 & -7.768826e-04 & -2.101913e-02 & -6.301476e-02 \\
572 & -7.334650e-03 & -1.047990e-01 &        0 &        0 & -2.806774e-03 &  4.908323e-04 &  3.165245e-02 & -9.809629e-02 \\
573 & -1.449466e-02 & -9.684845e-02 &        0 &        0 & -1.659917e-04 &  2.948347e-03 &  7.307974e-02 & -1.131957e-01 \\
574 & -1.111428e-02 & -9.035069e-02 &        0 &        0 & -4.268601e-04 & -1.279428e-03 &  5.349079e-02 & -8.753894e-02 \\
575 &  4.958595e-03 & -8.463861e-02 &        0 &        0 &  1.297600e-03 & -9.752343e-04 & -1.134746e-02 & -1.463634e-03 \\
576 &  2.637485e-02 & -6.911181e-02 &        0 &        0 &  2.790097e-04 &  1.392522e-03 & -5.275533e-02 &  8.524150e-02 \\
577 &  4.932604e-02 & -3.418568e-02 &        0 &        0 & -2.540660e-03 &  1.820103e-03 & -4.034333e-02 &  1.096378e-01 \\
578 &  6.338564e-02 &  9.694186e-03 &        0 &        0 & -3.644945e-03 &  5.379051e-03 & -1.309632e-02 &  7.941966e-02 \\
579 &  6.006904e-02 &  4.423509e-02 &        0 &        0 & -1.522917e-03 &  5.880949e-04 &  1.013061e-02 &  6.504710e-02 \\
580 &  4.786930e-02 &  4.703958e-02 &        0 &        0 & -7.199313e-04 &  4.311919e-03 &  1.577710e-02 &  2.765856e-02 \\
581 &  2.944711e-02 &  3.505368e-02 &        0 &        0 &  4.692244e-04 &  2.300350e-03 &  1.470285e-02 &  9.563074e-03 \\
582 &  1.238627e-02 &  2.027626e-02 &        0 &        0 & -3.120510e-03 &  6.532167e-03 &  1.648529e-02 &  7.973867e-03 \\
583 &  3.625255e-03 &  8.087915e-03 &        0 &        0 & -2.059745e-04 & -4.324569e-03 &  7.881129e-03 &  1.299201e-03 \\
584 &  3.534136e-04 &  1.723241e-03 &        0 &        0 & -2.084024e-03 & -1.666497e-02 &  3.285183e-04 & -1.842201e-04 \\
585 &  3.216547e-05 & -4.045504e-05 &        0 &        0 &  2.699661e-04 &  7.868290e-03 & -1.334599e-04 & -3.131690e-04 \\
586 &  5.901058e-05 & -1.561952e-04 &        0 &        0 & -4.849267e-05 &  4.231611e-03 & -1.850250e-04 & -8.446966e-04 \\
587 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.291913e-08 & -3.352086e-09 \\
588 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.764941e-08 & -1.309014e-10 \\
589 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.454354e-08 & -3.861128e-09 \\
590 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.895369e-08 &  5.268835e-10 \\
591 &  1.276555e-04 &  4.204514e-05 &        0 &        0 &  3.637722e-04 & -3.588747e-04 &  8.776075e-04 & -1.636766e-04 \\
592 &  6.372182e-03 & -4.323666e-03 &        0 &        0 & -4.671818e-04 & -1.661435e-03 &  2.570588e-03 &  6.368941e-03 \\
593 &  2.507423e-02 & -1.627058e-02 &        0 &        0 & -1.077033e-03 &  3.373921e-03 &  1.024873e-02 &  2.154842e-02 \\
594 &  5.439854e-02 & -2.488211e-02 &        0 &        0 &  6.907541e-04 &  9.332220e-04 & -5.464071e-03 &  3.391732e-02 \\
595 &  8.859094e-02 & -3.348172e-02 &        0 &        0 &  1.540087e-04 &  2.779735e-03 & -7.865052e-03 &  3.616595e-02 \\
596 &  1.050620e-01 & -3.868530e-02 &        0 &        0 & -1.691291e-03 &  7.690844e-04 & -2.059133e-02 &  6.876437e-03 \\
597 &  1.039182e-01 & -5.644295e-02 &        0 &        0 & -5.025968e-04 & -8.306441e-04 & -3.476007e-02 & -3.203647e-02 \\
598 &  8.618146e-02 & -8.023461e-02 &        0 &        0 &  1.956389e-03 & -4.550548e-04 & -3.581602e-02 & -6.630899e-02 \\
599 &  6.125428e-02 & -9.533455e-02 &        0 &        0 &  1.097497e-03 & -1.954060e-03 & -1.160163e-02 & -1.042968e-01 \\
600 &  3.792580e-02 & -9.987853e-02 &        0 &        0 & -5.903750e-04 &  3.515719e-05 &  1.799451e-02 & -1.408865e-01 \\
601 &  2.707400e-02 & -9.054901e-02 &        0 &        0 & -2.294029e-03 &  1.091562e-03 &  3.106419e-02 & -1.304629e-01 \\
602 &  2.870875e-02 & -7.112202e-02 &        0 &        0 &  4.298768e-03 & -3.043547e-03 & -7.747426e-03 & -7.106607e-02 \\
603 &  4.084742e-02 & -4.547401e-02 &        0 &        0 & -2.093314e-03 &  3.931113e-03 & -5.868218e-02 &  9.024543e-03 \\
604 &  5.424670e-02 & -6.992195e-03 &        0 &        0 & -4.437275e-04 & -1.983115e-03 & -7.729845e-02 &  5.162148e-02 \\
605 &  6.037220e-02 &  3.381458e-02 &        0 &        0 &  3.527609e-03 & -3.503054e-03 & -7.894175e-02 &  5.639423e-02 \\
606 &  5.478670e-02 &  5.531073e-02 &        0 &        0 & -1.918909e-03 & -3.045071e-03 & -4.577689e-02 &  5.513738e-02 \\
607 &  4.122003e-02 &  5.860695e-02 &        0 &        0 &  7.740329e-04 & -4.858990e-03 & -1.954375e-02 &  4.533900e-02 \\
608 &  2.596459e-02 &  4.131407e-02 &        0 &        0 &  8.464827e-05 & -3.083760e-03 & -5.441311e-03 &  1.952853e-02 \\
609 &  1.217398e-02 &  2.233534e-02 &        0 &        0 &  2.247428e-03 & -4.499941e-03 &  8.964877e-03 &  9.929829e-03 \\
610 &  4.212561e-03 &  9.264887e-03 &        0 &        0 &  2.138684e-03 & -7.601440e-04 &  8.077400e-03 &  1.171533e-03 \\
611 &  8.417400e-04 &  2.421735e-03 &        0 &        0 & -5.100264e-05 & -1.475279e-02 &  7.141494e-04 & -1.365208e-03 \\
612 &  1.510842e-04 &  8.917160e-04 &        0 &        0 & -6.839969e-04 & -3.156442e-02 & -1.004183e-05 & -6.618962e-04 \\
613 &  4.466773e-05 & -1.182311e-04 &        0 &        0 & -4.873530e-05 &  4.238613e-03 & -1.400527e-04 & -6.393865e-04 \\
614 &  1.028587e-04 & -2.722568e-04 &        0 &        0 & -4.885215e-05 &  4.276739e-03 & -3.224699e-04 & -1.472343e-03 \\
615 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.916180e-07 & -6.051881e-09 \\
616 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.499335e-08 &  2.754043e-09 \\
617 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.385719e-08 & -7.878126e-10 \\
618 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.843414e-08 &  1.270790e-09 \\
619 &  1.230253e-04 &  2.582003e-05 &        0 &        0 & -1.939634e-04 &  6.921972e-04 &  8.344368e-04 & -2.250277e-04 \\
620 &  2.658393e-03 & -2.263633e-03 &        0 &        0 & -1.692542e-03 &  2.043281e-03 &  2.635066e-03 &  2.726176e-03 \\
621 &  1.221136e-02 & -1.060760e-02 &        0 &        0 &  2.008374e-03 & -1.215382e-03 &  3.545158e-03 &  1.383966e-02 \\
622 &  3.075766e-02 & -2.044074e-02 &        0 &        0 &  5.059090e-04 & -3.108585e-03 &  2.345960e-04 &  2.726281e-02 \\
623 &  5.775459e-02 & -3.040092e-02 &        0 &        0 &  2.530837e-03 & -7.946021e-04 &  3.509401e-03 &  3.802746e-02 \\
624 &  8.156595e-02 & -3.536700e-02 &        0 &        0 & -3.906437e-03 & -5.689979e-04 &  9.131791e-03 &  2.721849e-02 \\
625 &  9.709215e-02 & -3.461158e-02 &        0 &        0 &  1.749079e-03 &  8.827187e-04 &  2.323570e-02 & -1.534962e-03 \\
626 &  9.786162e-02 & -3.750782e-02 &        0 &        0 &  8.799255e-04 & -8.964743e-04 &  2.789568e-02 & -5.248031e-02 \\
627 &  8.692649e-02 & -3.627467e-02 &        0 &        0 & -1.213746e-03 &  2.571889e-03 &  5.033860e-02 & -1.061493e-01 \\
628 &  7.272435e-02 & -3.220522e-02 &        0 &        0 & -2.642968e-03 &  4.359278e-04 &  4.570186e-02 & -1.410950e-01 \\
629 &  6.540714e-02 & -1.941405e-02 &        0 &        0 &  3.955272e-03 & -1.046725e-03 & -4.568722e-03 & -1.258901e-01 \\
630 &  6.183351e-02 &  1.198553e-03 &        0 &        0 & -1.946169e-03 & -1.299323e-03 & -5.109192e-02 & -7.532172e-02 \\
631 &  5.890587e-02 &  2.771602e-02 &        0 &        0 &  6.983911e-04 &  3.993406e-03 & -9.438115e-02 & -2.508364e-02 \\
632 &  5.185140e-02 &  5.343956e-02 &        0 &        0 &  2.017964e-04 & -8.064960e-04 & -1.146714e-01 &  7.734919e-03 \\
633 &  4.069575e-02 &  6.399127e-02 &        0 &        0 &  3.343243e-04 &  1.736092e-03 & -9.279127e-02 &  3.372253e-02 \\
634 &  2.832176e-02 &  5.928239e-02 &        0 &        0 &  1.225039e-03 &  1.567753e-03 & -5.052135e-02 &  4.509787e-02 \\
635 &  1.683285e-02 &  4.717895e-02 &        0 &        0 & -2.244276e-03 & -1.183912e-03 & -2.146952e-02 &  4.616446e-02 \\
636 &  8.309360e-03 &  2.743942e-02 &        0 &        0 & -2.620565e-03 & -2.551326e-03 &  1.007635e-03 &  2.771933e-02 \\
637 &  2.690998e-03 &  1.175391e-02 &        0 &        0 &  2.836800e-05 &  3.440898e-03 &  3.581211e-03 &  1.050018e-02 \\
638 &  9.310233e-04 &  3.647569e-03 &        0 &        0 & -1.026480e-03 & -1.307797e-04 &  3.060683e-03 &  2.218668e-03 \\
639 &  3.192033e-04 &  1.164714e-03 &        0 &        0 & -3.849785e-04 &  1.040071e-02 & -6.088432e-04 &  9.581604e-04 \\
640 & -7.677444e-06 &  3.484056e-04 &        0 &        0 & -6.645045e-04 & -2.399386e-02 &  7.180756e-05 &  1.286612e-04 \\
641 &  2.540733e-05 & -6.725070e-05 &        0 &        0 & -4.762684e-05 &  4.272141e-03 & -7.962898e-05 & -3.636891e-04 \\
642 &  5.819099e-05 & -1.540258e-04 &        0 &        0 & -4.807901e-05 &  4.223644e-03 & -1.824194e-04 & -8.329613e-04 \\
643 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -9.345920e-09 & -4.413198e-10 \\
644 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.471398e-08 & -8.577664e-10 \\
645 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  6.742269e-08 & -3.381179e-09 \\
646 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -7.240439e-09 &  2.064081e-09 \\
647 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.934569e-08 & -1.174169e-09 \\
648 &  2.291542e-04 & -3.020885e-04 &        0 &        0 &  1.123414e-03 &  1.313229e-03 &  2.520509e-03 &  1.581023e-03 \\
649 &  2.408616e-03 & -3.279391e-03 &        0 &        0 & -1.670524e-03 & -1.004012e-03 &  3.897694e-03 &  7.191084e-03 \\
650 &  8.526450e-03 & -8.032153e-03 &        0 &        0 & -7.951548e-05 &  4.500682e-04 &  4.653614e-03 &  9.465863e-03 \\
651 &  1.951366e-02 & -1.451156e-02 &        0 &        0 & -6.499246e-04 &  3.328614e-04 &  8.232902e-03 &  1.310465e-02 \\
652 &  3.855296e-02 & -2.310321e-02 &        0 &        0 &  1.102603e-04 &  2.455033e-03 &  2.456759e-02 &  1.547002e-02 \\
653 &  5.365519e-02 & -2.357876e-02 &        0 &        0 & -9.278198e-04 & -1.173370e-03 &  4.923108e-02 & -2.857818e-03 \\
654 &  6.145365e-02 & -1.742476e-02 &        0 &        0 &  1.302409e-03 & -1.094883e-03 &  8.186090e-02 & -3.822995e-02 \\
655 &  6.127720e-02 & -3.034283e-03 &        0 &        0 & -9.489240e-04 & -1.529546e-03 &  1.031593e-01 & -8.100813e-02 \\
656 &  5.645513e-02 &  1.528912e-02 &        0 &        0 & -3.893249e-03 &  2.093064e-03 &  8.784504e-02 & -9.665590e-02 \\
657 &  4.896479e-02 &  3.153395e-02 &        0 &        0 &  3.340570e-03 & -1.645126e-03 &  2.717736e-02 & -9.154415e-02 \\
658 &  3.973411e-02 &  4.833955e-02 &        0 &        0 &  5.239055e-04 & -7.074072e-04 & -2.954385e-02 & -6.182102e-02 \\
659 &  3.034684e-02 &  5.767274e-02 &        0 &        0 &  1.109734e-03 & -7.215829e-05 & -6.045492e-02 & -1.237585e-02 \\
660 &  1.752414e-02 &  6.063380e-02 &        0 &        0 & -5.063970e-04 &  1.083473e-03 & -8.277177e-02 &  2.501810e-02 \\
661 &  7.440881e-03 &  5.320688e-02 &        0 &        0 & -1.534009e-03 & -1.437789e-03 & -6.938432e-02 &  4.713582e-02 \\
662 &  2.638265e-03 &  4.213234e-02 &        0 &        0 &  1.411888e-04 &  4.676921e-03 & -3.936807e-02 &  6.229432e-02 \\
663 & -2.865326e-04 &  2.941351e-02 &        0 &        0 &  2.010003e-03 &  3.967871e-04 & -1.419488e-02 &  6.006889e-02 \\
664 & -1.090387e-03 &  1.694904e-02 &        0 &        0 & -2.790807e-04 & -2.663077e-03 & -1.130540e-03 &  3.773104e-02 \\
665 & -7.282639e-04 &  7.911560e-03 &        0 &        0 & -1.997747e-03 & -2.109175e-03 &  2.564245e-03 &  1.967954e-02 \\
666 & -8.854807e-05 &  3.342779e-03 &        0 &        0 &  3.259605e-04 &  6.964695e-03 &  1.212749e-03 &  6.876865e-03 \\
667 &  1.950718e-05 &  9.590930e-04 &        0 &        0 &  2.039971e-04 &  1.668076e-02 & -4.129568e-05 &  2.367911e-03 \\
668 &  1.131031e-05 &  2.181071e-04 &        0 &        0 &  7.356443e-04 &  1.684992e-03 &  2.104327e-05 &  5.581610e-04 \\
669 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -7.011279e-08 &  5.614240e-09 \\
670 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.271662e-08 &  4.443731e-09 \\
671 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.792319e-08 &  1.077979e-09 \\
672 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.851770e-08 & -5.383282e-09 \\
673 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.813872e-08 &  6.988483e-11 \\
674 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.481448e-07 &  9.464364e-09 \\
675 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -8.005828e-08 &  3.730089e-09 \\
676 &  5.752142e-05 & -1.241133e-05 &        0 &        0 &  2.979243e-04 & -1.749378e-03 &  1.275925e-03 &  1.447300e-04 \\
677 & -3.026679e-04 & -1.016689e-04 &        0 &        0 & -2.542523e-04 &  1.113277e-03 &  4.031461e-03 & -1.292289e-03 \\
678 & -5.263870e-04 & -2.437897e-04 &        0 &        0 & -1.518919e-03 &  7.894478e-04 &  6.246192e-03 & -5.407705e-03 \\
679 & -9.710172e-04 & -4.902692e-04 &        0 &        0 &  1.867188e-03 & -1.108736e-03 &  1.178190e-02 & -1.597955e-02 \\
680 & -1.539147e-03 &  7.842785e-04 &        0 &        0 & -2.536817e-05 & -2.970775e-04 &  3.126413e-02 & -2.530099e-02 \\
681 & -3.141459e-04 &  4.779212e-03 &        0 &        0 & -6.301547e-04 &  2.453712e-03 &  5.218373e-02 & -4.145847e-02 \\
682 & -2.076723e-03 &  1.210362e-02 &        0 &        0 &  1.697556e-03 & -1.673684e-03 &  7.953984e-02 & -6.735322e-02 \\
683 & -3.029087e-03 &  1.990606e-02 &        0 &        0 & -1.533078e-03 &  1.341376e-04 &  8.476480e-02 & -8.188317e-02 \\
684 & -2.437848e-03 &  2.802250e-02 &        0 &        0 &  3.812373e-03 & -1.371769e-03 &  5.312829e-02 & -7.897024e-02 \\
685 & -2.227851e-03 &  3.498497e-02 &        0 &        0 & -8.959979e-04 & -1.060860e-03 &  8.716733e-03 & -5.296670e-02 \\
686 & -4.497360e-03 &  3.873035e-02 &        0 &        0 & -1.274695e-04 &  1.874716e-03 & -3.006802e-02 & -2.330472e-02 \\
687 & -7.155401e-03 &  4.032266e-02 &        0 &        0 & -8.596012e-04 & -1.220093e-03 & -6.230182e-02 &  1.501542e-02 \\
688 & -9.749078e-03 &  4.098683e-02 &        0 &        0 &  2.403407e-03 &  1.419855e-03 & -7.449153e-02 &  5.129228e-02 \\
689 & -9.896483e-03 &  3.560769e-02 &        0 &        0 & -8.529057e-04 & -1.482973e-03 & -5.412544e-02 &  7.535663e-02 \\
690 & -8.035330e-03 &  2.877714e-02 &        0 &        0 & -7.105966e-04 &  3.497114e-04 & -3.254686e-02 &  7.775850e-02 \\
691 & -4.470358e-03 &  1.997130e-02 &        0 &        0 & -1.797304e-04 & -3.500160e-03 & -8.652290e-03 &  6.192910e-02 \\
692 & -2.639555e-03 &  1.379105e-02 &        0 &        0 &  2.369316e-03 &  8.204823e-03 &  5.853789e-04 &  4.418087e-02 \\
693 & -1.611075e-03 &  7.851654e-03 &        0 &        0 &  1.465724e-03 &  1.276916e-02 &  4.108583e-03 &  2.639095e-02 \\
694 & -6.684896e-04 &  3.760738e-03 &        0 &        0 &  1.206061e-03 &  1.379977e-02 &  3.216639e-03 &  1.246200e-02 \\
695 & -1.581033e-04 &  1.284377e-03 &        0 &        0 &  1.362796e-03 &  3.716244e-03 &  1.042224e-03 &  3.893182e-03 \\
696 &  1.569320e-05 &  1.844354e-04 &        0 &        0 &  7.211482e-04 &  3.666438e-03 &  1.460526e-05 &  5.414013e-04 \\
697 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.722419e-09 & -1.634369e-09 \\
698 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  9.706236e-08 & -5.755044e-09 \\
699 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.711599e-08 &  5.710265e-09 \\
700 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.424515e-08 & -1.384296e-09 \\
701 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.169933e-09 &  2.360221e-09 \\
702 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.418627e-08 & -1.995886e-09 \\
703 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.360271e-08 &  1.621465e-09 \\
704 & -5.656005e-05 &  7.435766e-06 &        0 &        0 &  4.801383e-04 & -3.018557e-03 &  1.387363e-04 & -2.199892e-04 \\
705 & -5.820547e-04 &  3.144467e-05 &        0 &        0 &  7.624410e-04 & -4.150980e-03 &  2.014548e-03 & -2.803669e-03 \\
706 & -1.403600e-03 &  8.507203e-05 &        0 &        0 &  1.257621e-03 & -5.703846e-03 &  5.247283e-03 & -6.400657e-03 \\
707 & -3.259427e-03 &  2.521261e-04 &        0 &        0 &  1.923377e-03 & -7.267389e-03 &  1.350295e-02 & -1.537547e-02 \\
708 & -6.386035e-03 &  1.775361e-03 &        0 &        0 & -2.589965e-04 &  6.545213e-04 &  3.119063e-02 & -3.136198e-02 \\
709 & -1.047250e-02 &  5.648513e-03 &        0 &        0 &  8.791606e-05 & -7.834184e-04 &  5.157746e-02 & -4.992626e-02 \\
710 & -1.477581e-02 &  1.069581e-02 &        0 &        0 & -3.189530e-04 & -1.029635e-03 &  6.287077e-02 & -6.829736e-02 \\
711 & -1.667399e-02 &  1.454275e-02 &        0 &        0 & -4.720623e-05 & -2.117163e-03 &  5.429904e-02 & -7.032076e-02 \\
712 & -1.667474e-02 &  1.831107e-02 &        0 &        0 & -4.390325e-04 &  1.126803e-03 &  2.199771e-02 & -5.618029e-02 \\
713 & -1.540295e-02 &  1.979780e-02 &        0 &        0 & -8.065292e-04 &  2.799086e-03 & -5.365903e-03 & -2.691882e-02 \\
714 & -1.375604e-02 &  2.066809e-02 &        0 &        0 & -1.823079e-04 & -3.435751e-04 & -2.375676e-02 &  1.015945e-03 \\
715 & -1.295598e-02 &  2.302604e-02 &        0 &        0 &  1.408122e-04 & -1.496174e-03 & -4.338184e-02 &  2.446841e-02 \\
716 & -1.224512e-02 &  2.513087e-02 &        0 &        0 &  4.389574e-03 & -1.563694e-02 & -5.215192e-02 &  4.817505e-02 \\
717 & -1.025611e-02 &  2.440068e-02 &        0 &        0 &  4.201773e-03 & -1.677160e-02 & -4.275863e-02 &  6.107725e-02 \\
718 & -7.095916e-03 &  1.922932e-02 &        0 &        0 &  3.932051e-03 & -1.672007e-02 & -2.533645e-02 &  5.504645e-02 \\
719 & -3.501526e-03 &  1.275257e-02 &        0 &        0 &  3.247515e-03 & -1.238979e-02 & -5.950198e-03 &  4.146170e-02 \\
720 & -2.074388e-03 &  9.981590e-03 &        0 &        0 &  3.168770e-03 & -1.004380e-02 &  1.689199e-03 &  3.501245e-02 \\
721 & -1.199328e-03 &  5.825879e-03 &        0 &        0 &  2.577584e-03 & -5.364812e-03 &  5.622651e-03 &  2.174719e-02 \\
722 & -4.827425e-04 &  2.289410e-03 &        0 &        0 &  2.013705e-03 & -1.976114e-03 &  1.349820e-03 &  7.845123e-03 \\
723 & -7.144247e-05 &  8.653300e-04 &        0 &        0 &  1.338511e-03 &  1.032021e-03 &  5.238904e-04 &  2.716020e-03 \\
724 &  1.799549e-05 &  1.147735e-04 &        0 &        0 &  7.134833e-04 &  1.805383e-03 &  1.000301e-04 &  3.935924e-04 \\
725 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.235483e-08 & -9.139088e-10 \\
726 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.925993e-09 &  3.572889e-09 \\
727 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.092036e-08 &  1.921699e-09 \\
728 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.300153e-08 &  2.246327e-10 \\
729 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.048373e-07 &  4.319200e-09 \\
730 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.003557e-09 &  2.752875e-10 \\
731 & -2.539976e-05 &  3.776495e-06 &        0 &        0 &  4.075603e-04 & -2.682511e-03 &  4.821405e-05 & -8.036635e-05 \\
732 & -2.294575e-04 &  4.397747e-05 &        0 &        0 &  5.070693e-04 & -3.210839e-03 &  5.536792e-04 & -7.631918e-04 \\
733 & -2.738462e-04 &  7.203463e-05 &        0 &        0 &  6.234298e-04 & -3.415640e-03 &  7.281220e-04 & -9.887295e-04 \\
734 & -6.135806e-04 &  2.877794e-04 &        0 &        0 &  1.039610e-03 & -3.942357e-03 &  2.110242e-03 & -2.229975e-03 \\
735 & -1.152899e-03 &  2.874464e-04 &        0 &        0 &  1.309093e-03 & -4.957458e-03 &  4.759306e-03 & -4.778010e-03 \\
736 & -2.504250e-03 &  1.231507e-03 &        0 &        0 &  1.452820e-03 & -5.796370e-03 &  1.087079e-02 & -1.088469e-02 \\
737 & -3.500268e-03 &  2.205908e-03 &        0 &        0 &  1.821299e-03 & -7.194959e-03 &  1.590335e-02 & -1.462129e-02 \\
738 & -4.122172e-03 &  3.315885e-03 &        0 &        0 &  2.020664e-03 & -7.528529e-03 &  1.521926e-02 & -1.718248e-02 \\
739 & -4.730412e-03 &  4.723344e-03 &        0 &        0 &  2.284612e-03 & -7.711842e-03 &  9.739503e-03 & -2.027869e-02 \\
740 & -4.602826e-03 &  5.233967e-03 &        0 &        0 &  2.596169e-03 & -7.639656e-03 & -1.028019e-03 & -1.513069e-02 \\
741 & -4.687762e-03 &  5.631345e-03 &        0 &        0 &  2.589763e-03 & -7.380886e-03 & -7.264211e-03 & -8.876318e-03 \\
742 & -4.594130e-03 &  6.861081e-03 &        0 &        0 &  2.653358e-03 & -7.986959e-03 & -1.166108e-02 &  1.229762e-04 \\
743 & -3.194886e-03 &  5.962462e-03 &        0 &        0 &  2.506563e-03 & -8.312009e-03 & -1.222668e-02 &  6.620977e-03 \\
744 & -3.138126e-03 &  5.993809e-03 &        0 &        0 &  2.759348e-03 & -1.021936e-02 & -1.547987e-02 &  7.249040e-03 \\
745 & -3.120424e-03 &  5.910728e-03 &        0 &        0 &  2.790179e-03 & -1.150426e-02 & -1.372654e-02 &  1.221546e-02 \\
746 & -1.902058e-03 &  4.865051e-03 &        0 &        0 &  2.662167e-03 & -1.154675e-02 & -7.325147e-03 &  1.309658e-02 \\
747 & -7.870360e-04 &  3.124732e-03 &        0 &        0 &  2.322850e-03 & -9.592799e-03 & -8.391601e-04 &  1.002064e-02 \\
748 & -5.203996e-04 &  2.650716e-03 &        0 &        0 &  2.270236e-03 & -8.774401e-03 &  9.304922e-04 &  9.198353e-03 \\
749 & -3.035289e-04 &  1.405776e-03 &        0 &        0 &  1.755095e-03 & -7.045795e-03 &  1.584639e-03 &  5.266404e-03 \\
750 & -1.336764e-04 &  6.661385e-04 &        0 &        0 &  1.338670e-03 & -5.880489e-03 &  1.261245e-03 &  2.672763e-03 \\
751 & -6.115193e-05 &  1.684902e-04 &        0 &        0 &  8.708382e-04 & -6.086616e-03 &  3.325734e-04 &  8.660689e-04 \\
752 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  7.705295e-08 & -2.676651e-09 \\
753 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.390799e-08 & -2.883047e-10 \\
754 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.344424e-08 &  8.579096e-10 \\
755 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  6.078791e-09 &  3.234541e-10 \\
756 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.230339e-08 & -7.020361e-12 \\
757 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.210552e-08 &  6.410986e-10 \\
758 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.292438e-08 &  4.711470e-09 \\
759 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  9.467230e-08 & -5.559619e-09 \\
760 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.572258e-08 & -7.667921e-10 \\
761 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.886974e-08 &  2.251462e-09 \\
762 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.965078e-08 &  5.368981e-09 \\
763 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.499817e-08 & -1.732327e-09 \\
764 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -8.007550e-08 &  6.338108e-09 \\
765 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.798965e-08 &  8.023539e-10 \\
766 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -9.326137e-08 &  2.212328e-10 \\
767 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.029488e-08 &  1.386750e-09 \\
768 & -1.143231e-04 &  1.686248e-04 &        0 &        0 &  8.932923e-04 & -2.657314e-03 & -4.138355e-04 & -3.060094e-04 \\
769 & -1.526303e-04 &  2.251274e-04 &        0 &        0 &  8.932279e-04 & -2.657234e-03 & -5.524800e-04 & -4.085552e-04 \\
770 & -2.166498e-04 &  2.988402e-04 &        0 &        0 &  9.664795e-04 & -2.926651e-03 & -6.856644e-04 & -1.295769e-04 \\
771 & -9.736587e-05 &  1.977600e-04 &        0 &        0 &  5.543896e-04 & -1.764739e-03 & -9.370376e-04 &  6.971455e-06 \\
772 & -2.781882e-05 &  5.650287e-05 &        0 &        0 &  5.544265e-04 & -1.764233e-03 & -2.676659e-04 &  1.983908e-06 \\
773 & -6.131117e-06 &  1.867469e-05 &        0 &        0 &  7.252392e-04 & -3.394297e-03 & -5.282481e-05 &  3.277046e-05 \\
774 & -9.765993e-05 &  2.974611e-04 &        0 &        0 &  7.252445e-04 & -3.394531e-03 & -8.417762e-04 &  5.219894e-04 \\
775 & -1.312188e-04 &  3.809571e-04 &        0 &        0 &  1.156035e-03 & -5.660519e-03 & -3.224681e-04 &  1.148338e-03 \\
776 & -7.612529e-05 &  2.147084e-04 &        0 &        0 &  9.028760e-04 & -4.529890e-03 &  8.510743e-05 &  8.166094e-04 \\
777 & -1.064689e-06 &  3.002915e-06 &        0 &        0 &  9.027813e-04 & -4.529981e-03 &  1.155864e-06 &  1.142468e-05 \\
778 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.409259e-08 & -1.911404e-09 \\
779 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.420310e-08 & -3.272405e-10 \\
780 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.292978e-08 &  5.938094e-10 \\
781 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.954772e-08 & -1.488858e-09 \\
782 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.837926e-09 &  1.586351e-09 \\
783 &  0.000000e+00 &  0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -6.581877e-08 &  3.526709e-09 \\
\bottomrule
\end{tabular}


==> supp_material/tables/mnist2.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &       PCA (x) &       PCA (y) &  LDA (x) &  LDA (y) &      cPCA (x) &      cPCA (y) &      ULCA (x) &      ULCA (y) \\
\midrule
0   & -2.021269e-18 & -6.136352e-18 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.349604e-07 &  2.350816e-06 \\
1   & -6.045554e-20 & -1.372421e-17 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.755208e-07 &  1.624157e-06 \\
2   &  6.981689e-22 &  8.098115e-20 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.861003e-07 & -2.811297e-06 \\
3   &  2.789414e-22 &  2.140790e-20 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.434684e-08 & -4.812794e-07 \\
4   &  1.156670e-23 & -5.321014e-21 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.177914e-07 & -4.484185e-07 \\
5   & -1.619016e-23 &  1.688023e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.716525e-08 &  1.248625e-06 \\
6   & -9.636597e-24 & -9.358297e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.337848e-07 &  9.465949e-07 \\
7   & -4.419780e-24 &  5.996542e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.668562e-07 & -1.317235e-06 \\
8   &  1.910267e-24 & -2.680383e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.562976e-07 &  2.110768e-06 \\
9   &  5.372229e-24 & -2.927264e-22 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.496742e-07 & -2.720439e-06 \\
10  &  1.514136e-24 & -9.541478e-23 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.846797e-07 &  4.456737e-06 \\
11  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.557839e-08 & -1.072928e-06 \\
12  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.192265e-07 & -1.996592e-06 \\
13  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.915034e-07 &  1.277693e-06 \\
14  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.618560e-07 &  1.573779e-06 \\
15  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.642560e-07 & -1.658167e-06 \\
16  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.627362e-07 &  3.778665e-06 \\
17  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -6.221928e-08 &  1.849233e-06 \\
18  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.655025e-07 &  2.290336e-06 \\
19  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.529607e-07 & -1.424193e-06 \\
20  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.461000e-07 &  3.542351e-06 \\
21  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.850674e-08 & -4.473311e-07 \\
22  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.972876e-07 &  3.018381e-06 \\
23  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.044808e-07 &  3.070936e-06 \\
24  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.687322e-07 &  2.224728e-06 \\
25  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.052841e-07 &  2.038727e-06 \\
26  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.087249e-07 & -2.725403e-06 \\
27  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.861658e-08 & -9.917002e-07 \\
28  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.279186e-07 & -2.441974e-06 \\
29  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.661001e-07 & -2.438490e-06 \\
30  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.773156e-07 &  2.798493e-06 \\
31  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.634180e-07 &  4.358274e-06 \\
32  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.776639e-07 & -2.094035e-06 \\
33  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.545947e-08 &  5.733502e-07 \\
34  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -5.344084e-07 &  4.184049e-06 \\
35  &  2.141479e-05 &  1.420014e-04 &        0 &        0 &  1.583297e-03 &  2.335186e-01 &  9.485752e-04 & -3.724359e-04 \\
36  &  6.934092e-05 &  4.678013e-04 &        0 &        0 &  1.949582e-03 &  2.806236e-01 &  3.228251e-03 & -1.263507e-03 \\
37  &  9.065502e-05 &  6.198903e-04 &        0 &        0 &  2.050037e-03 &  2.923686e-01 &  4.383788e-03 & -1.718510e-03 \\
38  &  4.795026e-05 &  3.302026e-04 &        0 &        0 &  2.006537e-03 &  2.386235e-01 &  3.696144e-03 & -8.254126e-04 \\
39  & -1.469842e-04 & -3.991414e-05 &        0 &        0 &  1.027811e-03 &  3.597852e-02 &  5.580313e-03 & -6.089708e-04 \\
40  & -1.864405e-04 & -1.747399e-04 &        0 &        0 &  1.029379e-03 &  2.293562e-02 &  4.209730e-03 & -8.277015e-04 \\
41  & -3.504243e-04 & -1.612669e-04 &        0 &        0 &  8.124271e-04 &  2.308845e-03 &  5.236871e-03 & -2.172152e-05 \\
42  & -1.462095e-04 &  3.774536e-05 &        0 &        0 &  8.027485e-04 & -1.347593e-03 &  3.453861e-03 &  1.365616e-03 \\
43  & -2.795246e-04 & -1.016709e-04 &        0 &        0 &  1.099934e-03 & -2.285887e-03 &  3.701332e-03 &  1.669677e-03 \\
44  & -1.122669e-04 & -3.305165e-04 &        0 &        0 &  1.130170e-03 & -1.920199e-03 &  3.762385e-03 &  2.969959e-03 \\
45  & -1.704615e-04 & -9.560007e-05 &        0 &        0 &  9.266115e-04 & -2.979863e-03 &  4.805749e-03 &  1.995960e-03 \\
46  & -2.150866e-04 & -2.517956e-04 &        0 &        0 &  7.163069e-04 & -2.519505e-03 &  1.678892e-03 &  1.097587e-03 \\
47  & -2.070278e-04 & -4.578286e-04 &        0 &        0 &  5.698027e-04 & -2.648679e-03 & -7.306295e-04 &  1.741495e-04 \\
48  & -2.751982e-04 & -6.870285e-04 &        0 &        0 &  5.177502e-04 & -2.630828e-03 & -1.113930e-03 & -4.250789e-04 \\
49  & -1.766674e-04 & -3.502528e-04 &        0 &        0 &  5.979898e-04 & -2.736392e-03 & -4.199411e-04 & -1.735605e-04 \\
50  & -9.764449e-05 & -1.747685e-04 &        0 &        0 &  5.077856e-04 & -2.224043e-03 & -1.927919e-04 & -1.185064e-05 \\
51  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.737915e-06 &  1.334266e-05 & -2.705409e-07 &  2.306053e-06 \\
52  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.409297e-06 & -4.034532e-05 &  2.227398e-07 & -1.497777e-06 \\
53  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.424714e-06 & -2.870812e-05 &  2.784070e-07 & -1.806052e-06 \\
54  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.936585e-06 & -5.577442e-06 & -4.956656e-07 &  4.367359e-06 \\
55  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.847935e-06 &  2.021725e-05 & -3.061612e-07 &  2.243234e-06 \\
56  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -2.354756e-06 & -2.691240e-05 & -3.421545e-07 &  2.619152e-06 \\
57  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -2.872221e-06 & -4.063779e-05 & -1.676479e-07 &  1.160977e-06 \\
58  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  6.304099e-08 &  1.294663e-05 & -2.189584e-07 &  1.761564e-06 \\
59  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.616317e-06 & -5.771643e-06 &  1.551256e-07 & -7.264984e-07 \\
60  & -1.454007e-05 & -1.217337e-04 &        0 &        0 &  4.699355e-04 &  1.493275e-02 & -2.578664e-05 & -5.719930e-05 \\
61  & -3.233935e-06 & -7.997812e-06 &        0 &        0 &  1.188110e-03 &  1.798177e-01 &  9.661507e-05 & -7.140545e-05 \\
62  & -8.019935e-06 &  2.130562e-05 &        0 &        0 &  1.102102e-03 &  1.965552e-01 &  4.588225e-04 & -2.914415e-04 \\
63  &  1.521343e-05 &  1.342130e-04 &        0 &        0 &  2.299375e-03 &  3.378341e-01 &  1.131877e-03 & -4.163587e-04 \\
64  &  8.817535e-05 &  7.078327e-04 &        0 &        0 &  2.237729e-03 &  2.969654e-01 &  6.791282e-03 & -1.284874e-03 \\
65  &  1.996231e-04 &  1.101082e-03 &        0 &        0 &  2.241431e-03 &  2.541362e-01 &  1.150336e-02 & -2.267677e-03 \\
66  & -7.881812e-05 &  1.358876e-03 &        0 &        0 &  2.375113e-03 &  2.017457e-01 &  2.179001e-02 & -3.699756e-03 \\
67  & -4.682707e-04 &  1.021615e-03 &        0 &        0 &  1.935793e-03 &  6.533136e-02 &  2.536385e-02 & -1.616870e-03 \\
68  & -9.109280e-04 &  1.299544e-03 &        0 &        0 &  2.077393e-03 &  2.399036e-02 &  3.114190e-02 &  7.038732e-04 \\
69  & -2.388379e-03 &  1.444102e-03 &        0 &        0 &  2.384291e-03 &  2.680245e-03 &  4.873953e-02 &  2.466942e-03 \\
70  & -4.785381e-03 & -8.411697e-04 &        0 &        0 &  3.023460e-03 & -5.692958e-03 &  6.738916e-02 &  8.352656e-03 \\
71  & -6.699287e-03 & -6.605261e-03 &        0 &        0 &  3.575491e-03 & -8.521369e-03 &  6.469707e-02 &  1.526196e-02 \\
72  & -1.019139e-02 & -1.725007e-02 &        0 &        0 &  4.136666e-03 & -1.204051e-02 &  5.022555e-02 &  1.729259e-02 \\
73  & -1.050355e-02 & -2.418862e-02 &        0 &        0 &  4.117270e-03 & -1.149372e-02 &  2.013285e-02 &  1.124312e-02 \\
74  & -8.755442e-03 & -2.466402e-02 &        0 &        0 &  3.513699e-03 & -9.111856e-03 & -2.238721e-02 &  1.477229e-03 \\
75  & -6.277631e-03 & -1.914394e-02 &        0 &        0 &  2.649492e-03 & -7.408460e-03 & -3.650007e-02 &  2.698358e-03 \\
76  & -3.390335e-03 & -1.048849e-02 &        0 &        0 &  1.981627e-03 & -7.469066e-03 & -2.809138e-02 &  8.414809e-03 \\
77  & -1.540892e-03 & -4.769707e-03 &        0 &        0 &  1.475993e-03 & -6.115922e-03 & -1.294620e-02 &  3.426862e-03 \\
78  & -4.380928e-04 & -1.390021e-03 &        0 &        0 &  1.019801e-03 & -4.293997e-03 & -3.963271e-03 &  1.053131e-03 \\
79  & -2.505553e-05 & -9.833883e-05 &        0 &        0 &  5.692455e-04 & -2.147084e-03 & -3.082826e-04 &  2.023856e-04 \\
80  & -6.520683e-06 & -2.126381e-05 &        0 &        0 &  1.248884e-03 & -1.713421e-03 & -1.063257e-05 &  5.965812e-05 \\
81  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  4.023413e-07 &  2.100001e-05 & -1.388798e-07 &  7.834305e-07 \\
82  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.948925e-06 & -1.342980e-05 & -9.830984e-08 &  1.469172e-06 \\
83  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.084184e-06 &  7.520904e-06 & -2.712874e-07 &  2.142976e-06 \\
84  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.754817e-06 & -2.678965e-05 & -7.260585e-08 &  6.528488e-07 \\
85  &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -9.156694e-07 &  2.497910e-05 & -3.156262e-07 &  3.392789e-06 \\
86  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.994162e-06 &  2.416565e-05 &  2.674074e-07 & -2.094430e-06 \\
87  &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  5.126476e-06 &  1.230141e-05 & -4.306334e-07 &  2.704550e-06 \\
88  & -1.504145e-06 & -1.259314e-05 &        0 &        0 &  4.689365e-04 &  1.489937e-02 & -2.879054e-06 & -4.066682e-06 \\
89  & -2.745557e-05 &  7.017314e-05 &        0 &        0 &  1.100655e-03 &  1.966946e-01 &  1.555921e-03 & -9.883835e-04 \\
90  & -8.530233e-06 & -1.859623e-05 &        0 &        0 &  1.171200e-03 &  1.772907e-01 &  3.023506e-03 & -1.914328e-03 \\
91  & -2.847441e-05 &  1.613055e-04 &        0 &        0 &  1.609475e-03 &  2.367045e-01 &  2.021217e-03 & -1.078236e-03 \\
92  &  2.245414e-04 &  1.232845e-03 &        0 &        0 &  2.146825e-03 &  2.600684e-01 &  9.518504e-03 & -1.615827e-03 \\
93  &  1.814069e-04 &  1.778926e-03 &        0 &        0 & -2.074319e-03 &  2.903133e-02 &  1.672727e-02 & -1.838344e-03 \\
94  & -1.128338e-04 &  2.853918e-03 &        0 &        0 &  1.904411e-04 & -2.357457e-02 &  3.354925e-02 & -2.645791e-03 \\
95  & -4.200655e-04 &  3.848929e-03 &        0 &        0 &  2.284668e-03 & -1.783358e-03 &  4.544084e-02 & -1.461321e-03 \\
96  & -1.188916e-03 &  4.396878e-03 &        0 &        0 & -1.635598e-03 &  2.536130e-03 &  6.589650e-02 & -1.450537e-03 \\
97  & -3.756395e-03 &  2.019959e-03 &        0 &        0 & -3.585004e-04 & -5.895626e-04 &  9.361307e-02 &  1.488743e-03 \\
98  & -1.005784e-02 & -6.120507e-03 &        0 &        0 &  2.404350e-04 & -2.779238e-05 &  1.179179e-01 &  9.042842e-03 \\
99  & -1.605898e-02 & -2.511137e-02 &        0 &        0 & -6.997421e-04 & -8.768929e-04 &  1.017796e-01 &  1.808209e-02 \\
100 & -2.054124e-02 & -4.378049e-02 &        0 &        0 &  1.058115e-03 & -2.300214e-04 &  3.487499e-02 &  1.949727e-02 \\
101 & -2.231438e-02 & -5.559641e-02 &        0 &        0 & -1.482627e-03 &  8.686634e-04 & -5.947138e-02 &  8.182386e-03 \\
102 & -1.835703e-02 & -5.298794e-02 &        0 &        0 &  6.196251e-04 & -3.101986e-03 & -1.138539e-01 &  4.965284e-04 \\
103 & -1.288975e-02 & -4.037894e-02 &        0 &        0 & -1.607644e-03 &  5.638135e-03 & -1.083618e-01 &  2.280417e-03 \\
104 & -6.496134e-03 & -2.143974e-02 &        0 &        0 & -1.834041e-05 & -7.295467e-03 & -6.732580e-02 &  8.449739e-03 \\
105 & -2.715744e-03 & -8.899739e-03 &        0 &        0 &  9.557631e-04 &  2.247964e-03 & -3.138855e-02 &  3.483321e-03 \\
106 & -7.492111e-04 & -2.922975e-03 &        0 &        0 &  1.693799e-03 & -4.614625e-03 & -1.366631e-02 &  2.071822e-03 \\
107 & -9.175876e-05 & -5.763812e-04 &        0 &        0 &  1.377909e-03 & -2.851387e-03 & -3.135674e-03 &  8.305007e-04 \\
108 & -3.369020e-05 & -1.098630e-04 &        0 &        0 &  1.254801e-03 & -1.749443e-03 & -5.634439e-05 &  3.154212e-04 \\
109 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.159026e-06 &  5.797796e-06 &  5.883022e-07 & -3.904369e-06 \\
110 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.982250e-08 &  3.884795e-07 & -5.961660e-08 &  9.226124e-08 \\
111 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.504604e-06 & -7.331128e-06 & -5.989498e-08 &  4.849307e-07 \\
112 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.021971e-07 &  1.388899e-05 & -3.111393e-07 &  2.385632e-06 \\
113 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -2.587492e-06 &  1.364018e-06 & -2.446866e-07 &  1.266303e-06 \\
114 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.692745e-06 & -8.251351e-06 &  1.243647e-07 & -7.809046e-07 \\
115 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.464686e-06 & -4.861578e-06 &  2.802562e-07 & -9.093445e-07 \\
116 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  6.496020e-07 &  3.976188e-06 &  9.435713e-08 & -1.311564e-06 \\
117 & -7.138287e-05 &  9.401501e-05 &        0 &        0 &  1.152383e-03 &  1.944178e-01 &  2.761401e-03 & -1.147488e-03 \\
118 & -1.156889e-04 &  3.392055e-04 &        0 &        0 &  1.137495e-03 &  1.805482e-01 &  3.059743e-03 & -1.270312e-03 \\
119 & -6.257918e-05 &  4.124090e-04 &        0 &        0 &  8.223259e-04 &  2.021767e-02 &  3.058757e-03 & -1.201581e-03 \\
120 &  2.634020e-04 &  1.524655e-03 &        0 &        0 & -6.608202e-04 &  1.079938e-02 &  1.225422e-02 & -3.881325e-04 \\
121 &  1.331130e-03 &  4.056589e-03 &        0 &        0 &  2.068892e-03 & -1.286384e-02 &  2.177619e-02 &  5.504851e-04 \\
122 &  2.899639e-03 &  8.369691e-03 &        0 &        0 & -7.255810e-04 &  5.682551e-03 &  3.165159e-02 & -1.407477e-03 \\
123 &  6.657351e-03 &  1.378415e-02 &        0 &        0 &  7.774867e-04 & -3.215047e-03 &  4.725188e-02 & -3.194979e-03 \\
124 &  1.286944e-02 &  1.637358e-02 &        0 &        0 & -1.565622e-03 &  7.909028e-04 &  4.449701e-02 & -4.036621e-03 \\
125 &  1.569124e-02 &  9.267574e-03 &        0 &        0 &  3.116873e-03 &  5.333401e-04 &  5.906325e-02 &  2.786687e-03 \\
126 &  1.311932e-02 & -1.400892e-02 &        0 &        0 & -7.771826e-04 & -3.592217e-04 &  6.395621e-02 &  1.098124e-02 \\
127 &  9.264380e-03 & -4.952581e-02 &        0 &        0 & -5.012668e-05 & -5.966737e-04 &  3.124575e-02 &  1.630009e-02 \\
128 &  7.338180e-03 & -8.039221e-02 &        0 &        0 & -3.331033e-04 &  3.646417e-05 & -4.208354e-02 &  6.962902e-03 \\
129 &  6.813228e-03 & -9.717647e-02 &        0 &        0 &  3.045173e-03 & -1.917153e-04 & -9.194045e-02 &  2.134992e-03 \\
130 &  9.757079e-03 & -8.696903e-02 &        0 &        0 &  2.904477e-04 & -8.690626e-04 & -8.471706e-02 &  4.609307e-03 \\
131 &  8.858076e-03 & -6.424213e-02 &        0 &        0 &  4.388131e-04 &  1.583222e-03 & -6.738663e-02 &  1.217701e-02 \\
132 &  7.963181e-03 & -3.948800e-02 &        0 &        0 &  4.227089e-04 & -1.902014e-03 & -3.322352e-02 &  8.637163e-03 \\
133 &  5.787918e-03 & -1.854834e-02 &        0 &        0 & -1.794323e-03 &  2.104809e-03 & -4.736541e-03 &  4.710578e-03 \\
134 &  3.387146e-03 & -7.747196e-03 &        0 &        0 &  1.076445e-03 & -1.861993e-03 & -5.085763e-03 &  4.581657e-04 \\
135 &  9.322443e-04 & -2.584242e-03 &        0 &        0 &  3.452901e-03 &  3.878325e-04 & -3.386620e-03 &  5.975815e-04 \\
136 &  6.996322e-05 & -3.698171e-04 &        0 &        0 &  5.654847e-03 & -1.552297e-03 &  1.620393e-03 &  1.049694e-03 \\
137 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.797633e-06 & -8.723434e-07 & -6.116675e-08 &  1.280839e-06 \\
138 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -4.067987e-06 &  1.063641e-07 & -2.397021e-07 &  8.292085e-07 \\
139 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -2.016470e-06 &  9.634008e-07 &  1.011187e-07 & -1.222461e-06 \\
140 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  3.907960e-06 &  3.475411e-06 & -1.876725e-07 &  1.721498e-08 \\
141 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.458799e-06 & -4.367545e-06 &  2.875731e-07 & -1.732995e-06 \\
142 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.378693e-06 &  1.072799e-06 & -5.543837e-08 &  8.021034e-07 \\
143 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  4.749959e-07 &  6.604598e-07 &  2.587938e-07 & -2.150926e-06 \\
144 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.223055e-07 & -2.548626e-06 & -3.282027e-08 & -3.683626e-07 \\
145 & -1.251045e-04 &  2.363775e-04 &        0 &        0 &  8.052741e-04 &  1.269303e-01 &  2.066698e-03 & -5.046173e-04 \\
146 & -1.210471e-04 &  6.101562e-04 &        0 &        0 & -4.115893e-04 & -4.759189e-03 &  3.679950e-03 & -8.491156e-04 \\
147 &  3.820411e-04 &  1.253653e-03 &        0 &        0 &  1.393960e-03 &  3.688546e-02 &  8.174374e-03 &  1.938140e-03 \\
148 &  1.734804e-03 &  3.378955e-03 &        0 &        0 & -2.019147e-03 & -6.562839e-03 &  1.293704e-02 &  4.269953e-03 \\
149 &  6.008441e-03 &  1.060866e-02 &        0 &        0 & -5.665504e-04 &  3.144285e-05 &  1.822606e-02 & -4.351703e-03 \\
150 &  1.365205e-02 &  2.181865e-02 &        0 &        0 & -1.299037e-04 &  1.288466e-03 &  2.987388e-02 & -1.217051e-02 \\
151 &  2.472075e-02 &  3.232027e-02 &        0 &        0 &  1.254177e-04 & -1.364909e-03 &  3.130453e-02 & -1.749409e-02 \\
152 &  3.595335e-02 &  3.184118e-02 &        0 &        0 &  1.609113e-03 & -6.058883e-03 &  2.879876e-02 & -2.582040e-02 \\
153 &  4.277292e-02 &  1.333671e-02 &        0 &        0 & -1.495348e-03 &  2.285457e-03 &  2.781512e-02 & -1.988517e-02 \\
154 &  4.743285e-02 & -2.678380e-02 &        0 &        0 &  2.233092e-03 &  2.515694e-04 &  1.223864e-03 & -1.028760e-03 \\
155 &  5.222111e-02 & -6.701449e-02 &        0 &        0 & -1.434879e-03 & -2.383377e-04 & -5.210971e-02 &  8.577259e-03 \\
156 &  5.514287e-02 & -9.991765e-02 &        0 &        0 &  9.048169e-04 & -8.125299e-04 & -1.026133e-01 &  8.547071e-03 \\
157 &  5.569360e-02 & -1.019238e-01 &        0 &        0 & -3.019834e-03 &  2.291138e-03 & -1.011595e-01 &  2.053335e-02 \\
158 &  5.290066e-02 & -8.799980e-02 &        0 &        0 & -6.284229e-05 & -2.143120e-03 & -6.148447e-02 &  2.897981e-02 \\
159 &  4.380542e-02 & -6.304552e-02 &        0 &        0 & -4.615493e-04 & -8.740335e-04 & -2.101353e-02 &  2.707549e-02 \\
160 &  3.177715e-02 & -4.135115e-02 &        0 &        0 & -2.771838e-04 & -8.376385e-04 &  1.052108e-02 &  5.809640e-03 \\
161 &  1.973962e-02 & -2.548976e-02 &        0 &        0 &  1.396615e-03 & -6.428923e-04 &  1.478854e-02 &  4.470043e-04 \\
162 &  1.008593e-02 & -1.208031e-02 &        0 &        0 &  1.078053e-04 &  1.175869e-03 &  2.721647e-03 &  1.016314e-04 \\
163 &  3.861963e-03 & -4.649759e-03 &        0 &        0 &  2.024584e-03 & -1.647458e-03 & -1.202709e-03 & -3.977961e-03 \\
164 &  2.897579e-04 & -7.528212e-04 &        0 &        0 & -1.346726e-02 &  3.940025e-03 &  2.195769e-03 &  6.405918e-05 \\
165 & -8.066816e-05 & -3.339117e-05 &        0 &        0 & -3.330325e-01 &  2.075505e-03 & -5.713578e-04 & -8.043891e-04 \\
166 & -3.007965e-05 & -1.245095e-05 &        0 &        0 & -3.330428e-01 &  2.074308e-03 & -2.127506e-04 & -3.017864e-04 \\
167 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -4.824262e-07 &  1.054770e-07 &  3.908043e-09 & -4.705205e-07 \\
168 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  6.410822e-07 &  2.492222e-07 & -5.856235e-09 &  1.003655e-06 \\
169 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.354939e-06 &  1.159788e-06 &  4.974537e-09 &  1.548525e-07 \\
170 & -5.627283e-05 & -1.383398e-04 &        0 &        0 &  2.893956e-04 & -1.027259e-03 & -1.050145e-04 & -8.971636e-05 \\
171 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  7.804176e-07 & -8.571932e-07 & -4.593088e-08 & -3.057906e-07 \\
172 &  6.522522e-05 & -2.401202e-06 &        0 &        0 &  9.282806e-04 & -7.218847e-03 &  4.338796e-04 &  4.967391e-04 \\
173 &  1.316882e-04 &  3.378439e-04 &        0 &        0 & -4.951055e-05 &  4.176402e-02 &  1.787407e-03 &  1.625026e-03 \\
174 &  2.291243e-05 &  1.185045e-03 &        0 &        0 & -7.532118e-04 & -3.798422e-02 &  3.789626e-03 &  2.264872e-03 \\
175 &  1.024071e-03 &  2.934611e-03 &        0 &        0 &  1.046341e-03 &  1.185261e-03 &  9.408618e-03 &  6.254492e-03 \\
176 &  5.954498e-03 &  1.026360e-02 &        0 &        0 &  1.158441e-03 &  3.378737e-03 &  9.878000e-03 & -3.853460e-04 \\
177 &  1.597677e-02 &  2.823196e-02 &        0 &        0 & -8.026006e-04 &  2.056054e-03 &  2.021320e-02 & -8.639235e-03 \\
178 &  2.954823e-02 &  4.785384e-02 &        0 &        0 & -1.952957e-03 &  2.062859e-03 &  8.239589e-03 & -1.710549e-02 \\
179 &  4.136372e-02 &  5.956442e-02 &        0 &        0 &  3.852578e-04 &  2.282116e-03 &  1.421842e-02 & -1.924334e-02 \\
180 &  4.497906e-02 &  5.729651e-02 &        0 &        0 & -3.811882e-04 &  1.073826e-03 &  2.839637e-02 &  2.391400e-04 \\
181 &  4.402591e-02 &  2.582406e-02 &        0 &        0 & -4.751830e-04 &  1.679792e-05 &  1.254537e-02 &  2.809340e-02 \\
182 &  3.998317e-02 & -1.535832e-02 &        0 &        0 & -7.009333e-04 &  1.693941e-03 & -1.644922e-02 &  2.522816e-02 \\
183 &  4.400987e-02 & -4.638144e-02 &        0 &        0 &  7.711938e-04 & -1.718202e-03 & -9.299993e-02 &  9.943485e-03 \\
184 &  5.277107e-02 & -5.871937e-02 &        0 &        0 & -8.181267e-04 &  5.408773e-05 & -1.287909e-01 & -8.568827e-03 \\
185 &  6.290146e-02 & -5.552335e-02 &        0 &        0 &  2.157449e-04 & -8.345176e-04 & -9.404176e-02 & -2.016437e-02 \\
186 &  7.117507e-02 & -5.207776e-02 &        0 &        0 &  1.857116e-04 &  1.128190e-03 & -3.826330e-02 & -2.023313e-02 \\
187 &  6.912736e-02 & -4.528827e-02 &        0 &        0 &  3.166423e-03 &  9.361180e-04 &  1.276936e-02 & -1.079074e-02 \\
188 &  5.536405e-02 & -3.595713e-02 &        0 &        0 &  1.335039e-04 & -1.096838e-03 &  1.412686e-02 & -3.557488e-03 \\
189 &  3.548228e-02 & -2.809118e-02 &        0 &        0 &  2.483543e-03 & -3.362994e-04 &  1.143316e-02 & -4.466227e-03 \\
190 &  1.911255e-02 & -1.681022e-02 &        0 &        0 &  3.583623e-04 & -3.646510e-04 &  5.419857e-03 & -8.347525e-03 \\
191 &  7.089838e-03 & -6.747210e-03 &        0 &        0 & -4.558504e-03 &  3.197279e-03 & -4.611832e-03 & -5.148611e-03 \\
192 &  9.676955e-04 & -1.084003e-03 &        0 &        0 &  3.304332e-03 & -2.308276e-03 & -1.236085e-03 & -8.824327e-04 \\
193 & -1.729580e-04 & -7.159294e-05 &        0 &        0 & -3.330285e-01 &  2.074625e-03 & -1.223583e-03 & -1.735707e-03 \\
194 & -1.647545e-04 & -6.819723e-05 &        0 &        0 & -3.330340e-01 &  2.074949e-03 & -1.165766e-03 & -1.652575e-03 \\
195 & -1.086969e-04 & -4.499319e-05 &        0 &        0 & -3.330342e-01 &  2.074270e-03 & -7.690943e-04 & -1.090504e-03 \\
196 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.540650e-06 & -8.877397e-08 &  2.251559e-07 & -1.699407e-06 \\
197 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -8.572121e-07 &  1.740215e-07 &  3.805576e-07 & -2.419989e-06 \\
198 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -8.933034e-07 &  1.023552e-07 & -1.962615e-07 &  4.138023e-07 \\
199 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.915184e-06 & -1.181459e-07 & -2.098446e-07 &  2.109878e-06 \\
200 &  1.633480e-04 &  1.098214e-04 &        0 &        0 & -9.470826e-05 & -2.830022e-03 &  4.036889e-04 &  1.147816e-03 \\
201 &  1.999829e-04 &  8.654850e-04 &        0 &        0 & -4.325034e-04 & -3.932451e-03 &  2.585766e-03 &  3.962193e-03 \\
202 &  2.062677e-04 &  2.838421e-03 &        0 &        0 & -1.816102e-04 & -7.430159e-03 &  6.208753e-03 &  7.107975e-03 \\
203 &  3.560550e-03 &  9.608646e-03 &        0 &        0 &  2.700015e-04 & -9.119778e-04 &  5.902177e-03 &  1.000133e-02 \\
204 &  1.367321e-02 &  2.788301e-02 &        0 &        0 &  1.374533e-04 & -1.002077e-03 &  1.600274e-02 &  9.856037e-03 \\
205 &  2.762204e-02 &  5.814557e-02 &        0 &        0 &  2.859023e-03 & -3.498501e-03 &  1.691340e-02 &  3.551279e-03 \\
206 &  3.864827e-02 &  8.256651e-02 &        0 &        0 & -1.049506e-03 & -3.451814e-04 &  1.663752e-02 &  1.277544e-02 \\
207 &  4.098186e-02 &  8.831626e-02 &        0 &        0 & -1.364629e-03 &  2.077215e-03 &  3.694749e-02 &  1.420120e-02 \\
208 &  3.480176e-02 &  6.551694e-02 &        0 &        0 &  1.847322e-03 & -2.991173e-03 &  4.133140e-02 &  2.459384e-02 \\
209 &  2.037823e-02 &  1.900851e-02 &        0 &        0 &  1.841113e-03 &  5.646355e-04 &  1.726503e-02 &  3.177645e-02 \\
210 &  1.382713e-02 & -1.780674e-02 &        0 &        0 & -1.555063e-03 &  1.461838e-03 & -5.316876e-02 &  9.517265e-03 \\
211 &  1.707932e-02 & -1.965567e-02 &        0 &        0 &  6.995866e-04 & -2.339385e-03 & -1.169534e-01 & -5.635277e-03 \\
212 &  2.773375e-02 & -1.499177e-03 &        0 &        0 & -6.616742e-04 &  9.388266e-04 & -1.040581e-01 & -1.582951e-02 \\
213 &  4.674119e-02 &  6.835317e-03 &        0 &        0 & -5.003101e-04 &  2.709551e-03 & -7.131707e-02 & -2.977362e-02 \\
214 &  6.547373e-02 &  4.576927e-04 &        0 &        0 &  9.038635e-04 & -1.682997e-03 & -1.225335e-02 & -3.467263e-02 \\
215 &  7.586307e-02 & -1.363797e-02 &        0 &        0 &  3.125358e-06 & -3.915097e-04 &  1.110148e-02 & -3.479285e-02 \\
216 &  7.234087e-02 & -2.209391e-02 &        0 &        0 & -2.584703e-03 &  2.830038e-03 &  2.340518e-02 & -2.175147e-02 \\
217 &  5.214218e-02 & -2.577106e-02 &        0 &        0 & -1.228526e-03 & -1.432320e-04 &  1.135243e-02 & -1.305274e-02 \\
218 &  2.927749e-02 & -1.850385e-02 &        0 &        0 & -5.112419e-03 & -1.873545e-04 &  4.840924e-03 & -1.433712e-02 \\
219 &  1.247424e-02 & -9.588674e-03 &        0 &        0 & -1.762360e-03 & -3.194369e-04 & -5.484895e-03 & -8.253232e-03 \\
220 &  2.515076e-03 & -2.292836e-03 &        0 &        0 & -1.252722e-03 &  1.675879e-03 & -3.199098e-03 & -5.730627e-04 \\
221 & -1.210022e-04 & -5.008676e-05 &        0 &        0 & -3.330351e-01 &  2.074161e-03 & -8.562145e-04 & -1.213149e-03 \\
222 & -1.497146e-04 & -6.197175e-05 &        0 &        0 & -3.330335e-01 &  2.074483e-03 & -1.059259e-03 & -1.502078e-03 \\
223 & -7.041373e-05 & -2.914653e-05 &        0 &        0 & -3.330366e-01 &  2.074667e-03 & -4.984145e-04 & -7.047446e-04 \\
224 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.394096e-06 &  1.229652e-07 & -2.379207e-07 &  1.770738e-06 \\
225 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.920370e-06 & -2.301995e-07 &  4.496891e-07 & -3.252939e-06 \\
226 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  3.833874e-07 &  6.895831e-09 &  1.371086e-07 & -2.017864e-06 \\
227 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.111779e-06 &  7.951871e-08 & -5.400791e-07 &  3.346727e-06 \\
228 &  3.110846e-05 &  3.627977e-04 &        0 &        0 & -3.296726e-05 & -3.122695e-03 &  8.171448e-04 &  1.722452e-03 \\
229 &  1.445993e-04 &  1.693850e-03 &        0 &        0 & -7.148435e-04 & -1.606920e-02 &  4.089012e-03 &  6.287067e-03 \\
230 &  1.581891e-03 &  7.520171e-03 &        0 &        0 & -4.059942e-04 &  7.058869e-03 &  7.403244e-03 &  1.460086e-02 \\
231 &  7.911462e-03 &  2.289063e-02 &        0 &        0 & -7.283118e-04 & -3.962751e-03 &  1.436404e-02 &  2.511709e-02 \\
232 &  2.375448e-02 &  5.589778e-02 &        0 &        0 &  2.939372e-04 &  9.910753e-04 &  2.126130e-02 &  2.059224e-02 \\
233 &  3.624391e-02 &  8.943528e-02 &        0 &        0 & -2.320082e-03 & -3.709033e-04 &  2.741716e-02 &  2.063443e-02 \\
234 &  4.280926e-02 &  1.062182e-01 &        0 &        0 & -1.433816e-06 & -1.389634e-03 &  8.435209e-03 &  1.328599e-02 \\
235 &  3.463758e-02 &  8.197379e-02 &        0 &        0 & -1.694896e-03 &  2.292871e-04 &  3.402488e-02 &  9.773301e-03 \\
236 &  1.841313e-02 &  2.013262e-02 &        0 &        0 & -4.466901e-03 & -1.259755e-04 &  2.205393e-02 &  1.772822e-03 \\
237 &  6.693173e-03 & -3.963558e-02 &        0 &        0 &  4.022034e-04 &  8.353032e-06 & -2.932778e-03 & -4.926695e-03 \\
238 &  6.309805e-03 & -5.636792e-02 &        0 &        0 & -4.097260e-04 &  4.131823e-04 & -8.871295e-02 &  6.602951e-03 \\
239 &  1.298399e-02 & -2.717078e-02 &        0 &        0 & -2.231179e-04 &  2.846380e-03 & -1.044275e-01 &  1.566164e-02 \\
240 &  1.834058e-02 &  1.331563e-02 &        0 &        0 &  4.642507e-04 & -3.076323e-03 & -6.044529e-02 &  2.315998e-02 \\
241 &  3.058347e-02 &  4.834010e-02 &        0 &        0 &  5.151253e-04 & -2.074180e-03 & -2.264082e-02 &  1.357823e-02 \\
242 &  4.952563e-02 &  4.569430e-02 &        0 &        0 & -1.314564e-03 & -6.543904e-04 & -8.691329e-03 & -1.554583e-02 \\
243 &  6.894904e-02 &  2.004894e-02 &        0 &        0 &  7.682583e-04 &  6.829166e-04 &  2.959755e-03 & -2.618548e-02 \\
244 &  8.144461e-02 & -1.943059e-03 &        0 &        0 & -5.329954e-04 & -2.867216e-03 &  2.027984e-02 & -2.413909e-02 \\
245 &  7.162280e-02 & -1.473840e-02 &        0 &        0 &  9.356454e-04 &  1.118364e-04 &  1.906843e-02 & -9.975051e-03 \\
246 &  4.548716e-02 & -1.646192e-02 &        0 &        0 &  6.917212e-04 &  1.340380e-03 &  1.104145e-02 & -1.515624e-02 \\
247 &  1.903851e-02 & -1.050544e-02 &        0 &        0 &  2.963209e-03 & -2.496292e-03 &  5.161797e-03 & -7.306891e-03 \\
248 &  4.887873e-03 & -3.474227e-03 &        0 &        0 & -1.240918e-04 & -3.019563e-03 & -5.282435e-03 & -3.174470e-03 \\
249 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.058169e-07 & -4.048667e-08 &  1.131316e-07 & -9.858401e-07 \\
250 & -2.255974e-05 & -9.338210e-06 &        0 &        0 & -3.330354e-01 &  2.074517e-03 & -1.602690e-04 & -2.209168e-04 \\
251 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  5.572289e-08 & -1.196328e-08 &  3.474731e-07 & -2.156630e-06 \\
252 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  6.218983e-08 & -7.617817e-09 &  1.991719e-07 & -9.158273e-07 \\
253 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.689455e-08 & -4.044146e-09 &  4.459271e-07 & -2.556393e-06 \\
254 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  7.905541e-08 & -2.158799e-08 & -2.010454e-07 &  7.666123e-07 \\
255 & -1.806227e-06 &  1.250102e-07 &        0 &        0 &  3.448362e-04 & -1.430228e-03 & -6.894355e-07 & -8.318660e-06 \\
256 & -4.261459e-05 &  4.237075e-04 &        0 &        0 &  5.447074e-05 & -3.223159e-03 &  1.001403e-03 &  1.601067e-03 \\
257 &  5.310753e-04 &  3.541685e-03 &        0 &        0 &  1.417715e-06 & -1.832521e-03 &  6.534587e-03 &  9.364089e-03 \\
258 &  5.954837e-03 &  1.749092e-02 &        0 &        0 &  1.088029e-03 & -2.196035e-04 &  1.211538e-02 &  2.431176e-02 \\
259 &  1.969940e-02 &  4.716677e-02 &        0 &        0 & -8.265622e-04 &  4.213155e-04 &  2.397525e-02 &  3.414995e-02 \\
260 &  3.445040e-02 &  8.439321e-02 &        0 &        0 &  2.682532e-03 &  8.597559e-04 &  1.895525e-02 &  2.821526e-02 \\
261 &  4.431605e-02 &  1.116138e-01 &        0 &        0 &  7.913464e-04 &  3.438147e-04 &  1.173204e-02 &  1.641414e-02 \\
262 &  4.190729e-02 &  9.422575e-02 &        0 &        0 &  1.079719e-04 &  7.329797e-04 &  2.321959e-02 & -7.866571e-03 \\
263 &  2.555445e-02 &  1.930649e-02 &        0 &        0 &  4.086408e-03 & -1.560559e-04 &  2.708584e-02 & -3.533746e-02 \\
264 &  9.662934e-03 & -6.476891e-02 &        0 &        0 & -5.979764e-05 & -8.371228e-04 &  1.218333e-02 & -3.720488e-02 \\
265 &  4.807616e-03 & -1.050871e-01 &        0 &        0 &  2.225947e-03 &  5.285093e-04 & -2.993524e-02 & -1.339889e-02 \\
266 &  9.841996e-03 & -8.677611e-02 &        0 &        0 &  8.223395e-04 & -3.641181e-03 & -8.529826e-02 &  1.239982e-02 \\
267 &  1.527816e-02 & -3.561875e-02 &        0 &        0 & -5.824441e-04 &  9.451511e-04 & -7.172535e-02 &  3.752800e-02 \\
268 &  1.611879e-02 &  1.910152e-02 &        0 &        0 & -1.161708e-03 &  2.148744e-03 & -4.492613e-02 &  4.275862e-02 \\
269 &  1.678727e-02 &  5.992320e-02 &        0 &        0 &  1.410073e-03 &  7.736559e-04 & -1.812440e-02 &  3.933988e-02 \\
270 &  2.486721e-02 &  6.122335e-02 &        0 &        0 &  2.862544e-03 &  5.007300e-04 & -1.827130e-02 &  2.733005e-03 \\
271 &  5.465794e-02 &  3.667305e-02 &        0 &        0 & -8.683327e-04 & -9.223246e-04 & -2.125283e-02 & -2.673820e-02 \\
272 &  8.324814e-02 &  1.037150e-02 &        0 &        0 & -5.243819e-04 & -4.244095e-04 &  4.194959e-03 & -2.016496e-02 \\
273 &  8.541441e-02 & -4.104105e-03 &        0 &        0 & -1.699577e-03 &  2.692053e-03 &  1.348883e-02 & -7.777721e-03 \\
274 &  6.426636e-02 & -8.927401e-03 &        0 &        0 &  1.477322e-03 &  3.500031e-04 &  8.729917e-03 & -4.139081e-03 \\
275 &  2.896006e-02 & -7.891790e-03 &        0 &        0 &  1.478500e-03 &  3.314983e-03 &  1.189878e-02 & -5.356080e-03 \\
276 &  6.790206e-03 & -4.099027e-03 &        0 &        0 &  3.975620e-03 &  1.132004e-03 & -2.921045e-03 & -3.267382e-03 \\
277 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.682899e-09 &  2.578314e-09 &  7.925007e-08 & -2.997202e-07 \\
278 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -9.487827e-09 &  4.644473e-09 & -1.051740e-07 &  1.356546e-06 \\
279 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -9.137552e-09 &  5.240198e-09 & -1.163973e-08 &  4.490082e-07 \\
280 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.499655e-09 &  2.258718e-10 & -3.507197e-07 &  3.231069e-06 \\
281 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.892518e-09 &  2.602129e-09 &  1.110255e-07 & -8.459967e-07 \\
282 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  4.977411e-09 & -3.290702e-09 &  1.447549e-08 &  6.243819e-08 \\
283 & -9.934250e-06 &  6.875560e-07 &        0 &        0 &  3.447432e-04 & -1.430285e-03 & -4.294428e-06 & -4.299828e-05 \\
284 & -2.608480e-04 &  8.097027e-04 &        0 &        0 &  3.605222e-04 & -2.514887e-03 &  1.181770e-03 &  1.617775e-03 \\
285 &  2.295603e-03 &  9.214676e-03 &        0 &        0 &  9.234138e-05 &  1.716369e-03 &  1.962479e-03 &  1.261181e-02 \\
286 &  1.374171e-02 &  3.164817e-02 &        0 &        0 &  4.464097e-05 &  8.162186e-04 &  1.508075e-02 &  3.094646e-02 \\
287 &  3.201368e-02 &  6.750542e-02 &        0 &        0 & -5.008596e-04 &  8.336045e-04 &  1.385800e-02 &  3.030264e-02 \\
288 &  4.773905e-02 &  1.035205e-01 &        0 &        0 &  1.103921e-03 & -2.473493e-03 &  1.840206e-02 &  3.344232e-02 \\
289 &  5.094931e-02 &  1.007151e-01 &        0 &        0 &  2.152268e-03 &  8.008409e-04 &  1.702951e-02 &  1.142087e-03 \\
290 &  3.568082e-02 &  3.623160e-02 &        0 &        0 & -3.235697e-03 &  9.319354e-04 &  2.815190e-02 & -3.793903e-02 \\
291 &  1.314764e-02 & -6.436143e-02 &        0 &        0 &  1.108672e-03 &  6.897462e-06 &  2.724819e-02 & -5.265451e-02 \\
292 &  3.803192e-03 & -1.284903e-01 &        0 &        0 & -1.297315e-03 & -4.867592e-04 &  5.344066e-04 & -2.544125e-02 \\
293 &  5.411465e-03 & -1.244492e-01 &        0 &        0 & -2.145442e-03 &  3.530008e-03 & -5.344789e-02 &  1.249137e-02 \\
294 &  1.214839e-02 & -7.476118e-02 &        0 &        0 &  1.946677e-03 & -1.516760e-03 & -5.902551e-02 &  2.428244e-02 \\
295 &  1.152507e-02 & -1.804704e-02 &        0 &        0 & -2.299484e-03 & -2.862993e-04 & -3.768227e-02 &  2.848369e-02 \\
296 &  3.177039e-03 &  3.126974e-02 &        0 &        0 &  1.339901e-03 &  7.033501e-04 & -3.961905e-02 &  3.104717e-02 \\
297 & -7.432576e-03 &  6.221649e-02 &        0 &        0 &  5.109363e-04 & -2.116267e-03 & -4.379894e-02 &  1.606925e-02 \\
298 & -2.387503e-03 &  6.538691e-02 &        0 &        0 & -5.269717e-03 & -1.540039e-04 & -3.404292e-02 & -1.684192e-02 \\
299 &  3.158190e-02 &  4.242301e-02 &        0 &        0 & -2.725374e-04 &  1.374430e-04 & -1.909373e-02 & -2.979832e-02 \\
300 &  7.561203e-02 &  1.212145e-02 &        0 &        0 &  2.191091e-04 &  8.751421e-04 & -1.033367e-02 & -1.855912e-02 \\
301 &  9.283560e-02 & -8.826274e-05 &        0 &        0 &  5.441554e-04 & -2.775922e-03 & -6.563526e-03 & -2.220282e-02 \\
302 &  7.764164e-02 & -1.871672e-03 &        0 &        0 &  1.686300e-03 & -2.509097e-03 &  3.960507e-03 & -8.172079e-03 \\
303 &  4.160391e-02 & -1.088527e-03 &        0 &        0 & -1.445355e-03 & -4.031709e-03 &  1.094620e-02 & -4.910407e-03 \\
304 &  9.140620e-03 & -1.918530e-03 &        0 &        0 & -1.257436e-03 & -1.559388e-03 &  6.780523e-03 & -4.211610e-03 \\
305 &  3.283541e-06 &  3.082221e-06 &        0 &        0 &  4.653427e-04 & -6.377570e-03 &  1.107718e-04 &  4.463779e-05 \\
306 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  3.806314e-11 & -2.531042e-11 & -1.992939e-07 &  1.445213e-06 \\
307 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  3.101849e-10 & -4.222915e-10 & -1.216079e-07 &  1.175457e-06 \\
308 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  4.194903e-10 & -5.712142e-10 & -3.647380e-07 &  2.916986e-06 \\
309 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.893499e-10 & -3.974474e-10 & -1.196171e-07 &  1.187960e-06 \\
310 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  4.495405e-11 & -6.400969e-11 & -4.771508e-07 &  3.121739e-06 \\
311 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.427996e-10 & -2.071250e-10 & -7.625140e-08 &  9.022594e-07 \\
312 &  9.021367e-05 &  1.655042e-03 &        0 &        0 &  4.667946e-05 &  1.049365e-03 &  1.839740e-03 &  3.704712e-03 \\
313 &  7.119709e-03 &  1.688933e-02 &        0 &        0 & -1.651997e-03 & -1.818392e-03 &  5.603309e-03 &  2.114590e-02 \\
314 &  2.533149e-02 &  4.840603e-02 &        0 &        0 &  7.826887e-04 &  7.038427e-04 &  1.943180e-02 &  3.258578e-02 \\
315 &  4.699944e-02 &  8.409440e-02 &        0 &        0 &  6.804135e-04 &  3.612798e-03 & -9.773616e-04 &  2.575259e-02 \\
316 &  5.935011e-02 &  1.025058e-01 &        0 &        0 &  3.735464e-05 & -3.380494e-04 &  1.475428e-02 &  3.442632e-02 \\
317 &  4.913115e-02 &  6.148478e-02 &        0 &        0 & -6.900237e-04 &  1.006212e-03 &  2.329552e-02 & -1.759344e-02 \\
318 &  2.129208e-02 & -3.832988e-02 &        0 &        0 &  6.747025e-04 & -1.536749e-03 &  3.709729e-02 & -5.058395e-02 \\
319 &  1.928456e-03 & -1.250855e-01 &        0 &        0 & -9.311208e-04 &  1.362280e-03 &  1.128625e-02 & -4.920457e-02 \\
320 & -6.284024e-03 & -1.414838e-01 &        0 &        0 &  3.002781e-03 & -2.771766e-03 & -3.441774e-02 & -3.383452e-03 \\
321 & -2.015483e-03 & -9.860571e-02 &        0 &        0 &  3.431272e-04 &  3.071664e-03 & -6.475204e-02 &  2.196304e-02 \\
322 &  5.192634e-04 & -3.773683e-02 &        0 &        0 & -6.990366e-04 & -1.940794e-04 & -4.925621e-02 &  2.937030e-02 \\
323 & -4.972070e-03 &  9.027878e-03 &        0 &        0 &  2.350723e-03 &  1.259484e-03 & -1.909201e-02 &  2.508603e-02 \\
324 & -2.224169e-02 &  4.372036e-02 &        0 &        0 & -9.541546e-04 & -3.127708e-03 & -2.138189e-02 &  2.235049e-03 \\
325 & -4.054789e-02 &  6.720367e-02 &        0 &        0 &  5.963654e-04 &  3.330359e-03 &  7.433933e-03 & -3.538823e-02 \\
326 & -3.135463e-02 &  5.834093e-02 &        0 &        0 &  1.991482e-04 &  6.659203e-04 &  5.204925e-02 & -5.740059e-02 \\
327 &  8.852872e-03 &  3.115753e-02 &        0 &        0 &  3.811205e-03 & -1.185686e-03 &  4.254519e-02 & -6.342915e-02 \\
328 &  6.436927e-02 &  9.921402e-04 &        0 &        0 & -8.429106e-04 &  2.964328e-03 &  2.112199e-02 & -3.890042e-02 \\
329 &  9.568454e-02 & -9.292618e-04 &        0 &        0 &  2.008078e-03 &  9.461651e-04 & -2.583997e-03 & -3.355305e-02 \\
330 &  8.855565e-02 &  5.073064e-03 &        0 &        0 & -6.359969e-04 &  1.378034e-03 &  4.152790e-03 & -1.416490e-02 \\
331 &  5.220304e-02 &  1.024417e-02 &        0 &        0 & -1.647666e-03 &  1.309493e-04 &  1.587129e-02 & -1.827507e-03 \\
332 &  1.265877e-02 &  3.293765e-03 &        0 &        0 & -4.042292e-04 &  4.087180e-03 &  1.572511e-02 & -7.717619e-04 \\
333 &  8.426079e-05 & -9.065435e-05 &        0 &        0 & -1.179499e-04 & -3.339266e-02 &  4.276802e-04 & -1.452771e-04 \\
334 &  8.892566e-05 & -2.353774e-04 &        0 &        0 & -4.869199e-05 &  4.284496e-03 & -2.003412e-03 & -1.190947e-03 \\
335 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -2.876848e-13 &  8.325562e-13 &  1.727183e-07 & -6.822585e-07 \\
336 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.014514e-12 & -6.634915e-12 &  3.866707e-07 & -2.134737e-06 \\
337 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  7.976610e-13 & -2.896350e-12 &  1.076901e-07 & -5.938045e-07 \\
338 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.606350e-13 &  5.838663e-13 &  8.841511e-08 & -9.555390e-07 \\
339 &  3.394577e-05 &  5.198206e-04 &        0 &        0 &  1.001373e-03 & -1.190282e-03 &  6.781662e-04 &  7.772485e-04 \\
340 &  1.054173e-03 &  3.408999e-03 &        0 &        0 &  9.695555e-04 & -7.055715e-04 &  2.699960e-03 &  5.564711e-03 \\
341 &  1.443340e-02 &  2.491738e-02 &        0 &        0 &  6.920073e-04 &  1.904665e-03 &  1.219149e-02 &  2.058770e-02 \\
342 &  3.981670e-02 &  6.056805e-02 &        0 &        0 &  3.211769e-05 & -1.232939e-03 &  2.628208e-02 &  3.331340e-02 \\
343 &  6.405361e-02 &  8.806525e-02 &        0 &        0 & -3.005410e-03 &  1.025157e-03 &  1.404000e-02 &  3.660942e-02 \\
344 &  6.787671e-02 &  8.123593e-02 &        0 &        0 & -1.183961e-05 & -1.477526e-03 &  2.025490e-02 &  3.685606e-02 \\
345 &  4.034511e-02 &  7.867103e-03 &        0 &        0 &  1.193566e-03 &  2.138199e-03 &  5.092607e-02 & -4.016467e-03 \\
346 &  4.948801e-03 & -8.995444e-02 &        0 &        0 &  1.409046e-04 &  4.278224e-03 &  3.135744e-02 & -6.012894e-02 \\
347 & -1.628813e-02 & -1.371429e-01 &        0 &        0 & -1.320023e-04 &  1.002292e-03 & -1.622169e-02 & -4.976011e-02 \\
348 & -2.295727e-02 & -1.116327e-01 &        0 &        0 & -3.117264e-03 & -2.318138e-04 & -7.005765e-02 & -1.424142e-02 \\
349 & -1.737069e-02 & -5.099849e-02 &        0 &        0 &  2.122857e-03 &  1.600711e-05 & -7.334473e-02 & -1.292048e-02 \\
350 & -1.723184e-02 & -3.762399e-03 &        0 &        0 & -1.851415e-03 & -1.800424e-03 & -2.730570e-02 & -1.594783e-02 \\
351 & -3.186261e-02 &  2.845454e-02 &        0 &        0 & -1.357090e-03 & -9.519552e-04 &  1.667915e-02 & -4.621436e-02 \\
352 & -5.665690e-02 &  4.994358e-02 &        0 &        0 &  1.738200e-03 &  8.967334e-04 &  7.333204e-02 & -9.041090e-02 \\
353 & -7.181438e-02 &  5.847855e-02 &        0 &        0 & -8.641849e-05 & -2.999043e-03 &  1.344356e-01 & -1.028256e-01 \\
354 & -5.496553e-02 &  3.177716e-02 &        0 &        0 &  4.699491e-04 & -1.416149e-03 &  1.714588e-01 & -9.678963e-02 \\
355 & -9.629146e-03 & -3.884583e-03 &        0 &        0 & -2.536080e-03 &  7.239886e-04 &  1.389698e-01 & -7.200859e-02 \\
356 &  5.530467e-02 & -2.645573e-02 &        0 &        0 & -8.104289e-04 & -2.410777e-03 &  8.928863e-02 & -4.525002e-02 \\
357 &  9.656842e-02 & -1.237361e-02 &        0 &        0 & -2.537642e-03 & -1.466548e-04 &  3.731737e-02 & -2.288320e-02 \\
358 &  9.407973e-02 &  9.507559e-03 &        0 &        0 &  2.808311e-03 & -2.010869e-03 &  1.850381e-02 & -2.798970e-02 \\
359 &  5.905179e-02 &  1.978161e-02 &        0 &        0 &  3.513560e-04 & -1.082444e-03 &  3.295155e-02 & -6.547530e-03 \\
360 &  1.637587e-02 &  9.386046e-03 &        0 &        0 &  7.511296e-04 & -1.680709e-03 &  3.343360e-02 & -3.609019e-03 \\
361 &  2.523526e-04 &  5.284371e-04 &        0 &        0 & -1.248632e-03 & -2.738061e-05 &  6.162962e-03 &  3.767563e-05 \\
362 &  7.089465e-05 & -1.876511e-04 &        0 &        0 & -4.796517e-05 &  4.311236e-03 & -1.596783e-03 & -9.516287e-04 \\
363 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -7.018518e-14 &  1.181431e-13 & -1.363344e-07 &  1.326155e-06 \\
364 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.585711e-14 & -1.882938e-13 & -1.185822e-07 &  9.518825e-07 \\
365 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -8.673184e-15 & -4.263256e-14 & -1.521118e-07 &  9.145232e-07 \\
366 &  1.679913e-06 & -5.367623e-05 &        0 &        0 &  2.008466e-05 &  8.018260e-05 &  1.134096e-04 &  9.097350e-05 \\
367 &  5.087579e-05 &  8.739215e-04 &        0 &        0 &  1.086917e-03 & -1.511564e-03 &  8.292898e-04 &  1.518988e-03 \\
368 &  2.941337e-03 &  4.445601e-03 &        0 &        0 & -1.988949e-03 &  1.544927e-03 &  5.253445e-03 &  7.837142e-03 \\
369 &  2.410312e-02 &  3.107291e-02 &        0 &        0 & -1.328090e-03 & -2.554024e-03 &  1.209327e-02 &  1.299492e-02 \\
370 &  5.698829e-02 &  6.230892e-02 &        0 &        0 &  1.524522e-03 & -5.910147e-04 &  1.465621e-02 &  2.633635e-02 \\
371 &  7.914471e-02 &  7.534519e-02 &        0 &        0 & -4.868814e-04 &  1.084716e-03 &  1.193858e-02 &  4.101881e-02 \\
372 &  6.720995e-02 &  4.703325e-02 &        0 &        0 & -1.267435e-03 &  2.390455e-03 &  4.531425e-02 &  7.278080e-02 \\
373 &  2.516440e-02 & -3.249911e-02 &        0 &        0 &  5.933461e-04 & -2.102458e-03 &  5.564795e-02 &  1.759276e-02 \\
374 & -1.837830e-02 & -1.066063e-01 &        0 &        0 &  7.594822e-04 & -7.519429e-04 &  2.056413e-02 & -5.911944e-02 \\
375 & -4.216498e-02 & -1.138195e-01 &        0 &        0 & -1.085200e-03 &  1.785359e-03 & -3.460873e-02 & -7.403761e-02 \\
376 & -4.290858e-02 & -6.557591e-02 &        0 &        0 &  5.186741e-04 & -1.368246e-03 & -7.242869e-02 & -6.295939e-02 \\
377 & -4.096203e-02 & -8.989045e-03 &        0 &        0 & -1.138959e-03 &  2.199795e-03 & -3.716073e-02 & -7.974540e-02 \\
378 & -4.983524e-02 &  1.870392e-02 &        0 &        0 & -1.021112e-03 &  3.114696e-03 &  1.353724e-02 & -1.142325e-01 \\
379 & -6.963342e-02 &  3.178839e-02 &        0 &        0 &  1.497677e-03 &  1.272745e-03 &  9.431300e-02 & -1.442474e-01 \\
380 & -8.858358e-02 &  4.065950e-02 &        0 &        0 & -5.188105e-06 &  1.079988e-03 &  1.360147e-01 & -1.374813e-01 \\
381 & -9.166698e-02 &  3.653284e-02 &        0 &        0 & -1.364595e-03 &  8.336072e-04 &  1.783641e-01 & -9.151796e-02 \\
382 & -6.479911e-02 & -1.440538e-03 &        0 &        0 &  8.657431e-04 &  1.759997e-03 &  2.117182e-01 & -5.505681e-02 \\
383 & -1.418123e-02 & -4.303752e-02 &        0 &        0 &  2.843114e-04 &  2.938638e-04 &  1.895114e-01 & -3.498808e-02 \\
384 &  5.123211e-02 & -5.927085e-02 &        0 &        0 &  7.596206e-04 &  2.736790e-04 &  1.243113e-01 & -2.361375e-02 \\
385 &  9.362461e-02 & -2.870326e-02 &        0 &        0 &  1.668972e-03 & -1.014649e-03 &  7.705789e-02 & -1.731500e-02 \\
386 &  9.408389e-02 &  9.074641e-03 &        0 &        0 & -3.732744e-03 &  2.894457e-03 &  3.837346e-02 & -2.276065e-02 \\
387 &  6.190191e-02 &  2.736712e-02 &        0 &        0 &  6.429803e-04 &  1.186565e-03 &  3.829929e-02 & -1.491439e-02 \\
388 &  1.885906e-02 &  1.522801e-02 &        0 &        0 &  1.226231e-03 & -2.317789e-03 &  3.815003e-02 & -5.600297e-03 \\
389 &  1.770216e-04 &  1.739070e-03 &        0 &        0 &  4.110445e-05 & -3.691252e-02 &  1.518592e-02 & -1.630655e-03 \\
390 & -1.675360e-05 &  6.985899e-07 &        0 &        0 &  4.690168e-04 &  1.918514e-03 & -1.108533e-04 & -2.050171e-04 \\
391 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.082523e-15 &  3.530509e-14 & -1.208187e-07 &  9.274896e-07 \\
392 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -8.253131e-14 & -1.865175e-14 &  4.590230e-08 & -6.761280e-07 \\
393 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  4.786471e-14 &  5.573320e-14 &  2.439973e-07 & -1.276365e-06 \\
394 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.547330e-14 & -5.773160e-15 &  8.875892e-08 &  3.347113e-07 \\
395 &  7.047425e-05 &  9.620912e-04 &        0 &        0 &  1.239601e-03 & -2.252831e-03 &  9.244248e-04 &  1.863390e-03 \\
396 &  6.155614e-03 &  5.076919e-03 &        0 &        0 &  2.363839e-03 & -4.084481e-03 &  4.277583e-03 &  1.088639e-02 \\
397 &  3.754922e-02 &  3.300558e-02 &        0 &        0 &  2.559410e-04 &  4.370749e-04 &  9.753321e-03 &  1.526647e-02 \\
398 &  7.483877e-02 &  5.442254e-02 &        0 &        0 & -3.724503e-04 & -2.340446e-03 &  2.939456e-03 &  1.689347e-02 \\
399 &  9.124810e-02 &  5.169287e-02 &        0 &        0 &  9.757185e-04 & -2.854992e-03 &  1.682686e-02 &  4.791707e-02 \\
400 &  6.649142e-02 &  1.032219e-02 &        0 &        0 &  8.716695e-04 &  5.197888e-04 &  6.801545e-02 &  1.000112e-01 \\
401 &  7.966177e-03 & -5.940281e-02 &        0 &        0 &  1.141338e-03 & -3.845328e-03 &  7.261498e-02 &  5.620876e-02 \\
402 & -4.388661e-02 & -9.285212e-02 &        0 &        0 &  1.457446e-03 & -3.155484e-03 &  3.374957e-02 & -1.572092e-02 \\
403 & -6.672558e-02 & -6.563932e-02 &        0 &        0 &  9.208409e-04 & -1.348386e-03 & -3.097859e-02 & -6.197420e-02 \\
404 & -6.467824e-02 & -1.334170e-02 &        0 &        0 & -3.446620e-04 & -1.111286e-03 & -4.568920e-02 & -8.677753e-02 \\
405 & -6.434286e-02 &  1.844592e-02 &        0 &        0 &  1.199259e-04 &  5.089864e-04 &  3.048474e-02 & -9.813305e-02 \\
406 & -7.642489e-02 &  2.107656e-02 &        0 &        0 &  7.554759e-04 & -2.613478e-03 &  8.874888e-02 & -1.147430e-01 \\
407 & -9.292521e-02 &  1.698786e-02 &        0 &        0 & -2.941204e-03 & -1.849305e-03 &  1.032172e-01 & -1.048453e-01 \\
408 & -1.048330e-01 &  2.177050e-02 &        0 &        0 &  8.788072e-04 & -6.969195e-04 &  8.097983e-02 & -5.085586e-02 \\
409 & -9.697084e-02 &  1.119570e-02 &        0 &        0 &  1.437833e-03 &  8.661213e-05 &  1.029940e-01 &  3.065118e-02 \\
410 & -5.813400e-02 & -2.703691e-02 &        0 &        0 & -4.207809e-04 &  9.281782e-05 &  1.465979e-01 &  5.522495e-02 \\
411 & -4.154117e-03 & -7.154267e-02 &        0 &        0 & -8.484168e-04 &  1.349793e-03 &  1.283957e-01 &  3.043040e-02 \\
412 &  5.266117e-02 & -8.154170e-02 &        0 &        0 &  2.120215e-03 & -2.644981e-03 &  1.151814e-01 &  1.047104e-02 \\
413 &  9.126633e-02 & -3.512781e-02 &        0 &        0 & -8.521765e-04 &  1.610960e-03 &  8.097819e-02 & -5.507105e-03 \\
414 &  8.972638e-02 &  1.218363e-02 &        0 &        0 &  1.660634e-03 &  2.672932e-03 &  5.284516e-02 & -9.934377e-03 \\
415 &  6.018858e-02 &  3.326567e-02 &        0 &        0 & -7.765975e-04 &  7.531458e-04 &  4.106946e-02 & -1.483876e-02 \\
416 &  1.826655e-02 &  1.882446e-02 &        0 &        0 & -4.793815e-04 &  4.953023e-03 &  3.548859e-02 & -7.167529e-03 \\
417 &  4.253158e-04 &  2.588471e-03 &        0 &        0 &  3.021855e-04 & -6.680737e-03 &  1.852855e-02 & -2.962119e-03 \\
418 & -2.974749e-05 &  2.669858e-05 &        0 &        0 &  5.176454e-04 & -2.384990e-03 &  8.753286e-05 & -1.101980e-04 \\
419 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.521029e-15 & -3.411160e-14 &  1.252435e-08 & -1.491459e-07 \\
420 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.093551e-14 &  2.556289e-14 &  2.817228e-07 & -2.154480e-06 \\
421 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -4.576672e-14 &  4.307665e-14 &  1.923447e-07 & -1.724265e-06 \\
422 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.038056e-15 &  7.049916e-15 & -4.620479e-07 &  3.759549e-06 \\
423 &  1.552190e-05 &  3.339614e-04 &        0 &        0 &  6.428742e-04 & -4.368280e-04 &  1.291813e-03 &  4.742078e-04 \\
424 &  8.975598e-03 &  4.179106e-03 &        0 &        0 & -1.391411e-05 &  2.824727e-03 & -1.194871e-04 &  8.766804e-03 \\
425 &  4.945257e-02 &  2.888740e-02 &        0 &        0 & -1.137947e-03 & -3.228132e-03 &  3.896647e-04 &  4.673838e-03 \\
426 &  8.826920e-02 &  3.913029e-02 &        0 &        0 &  2.620996e-03 &  2.883815e-03 & -2.682495e-03 &  1.105778e-02 \\
427 &  9.945629e-02 &  1.974494e-02 &        0 &        0 &  1.705262e-03 & -1.713752e-03 &  3.094321e-02 &  4.696624e-02 \\
428 &  6.258743e-02 & -2.423452e-02 &        0 &        0 &  4.356440e-04 & -6.415647e-03 &  7.815152e-02 &  9.886277e-02 \\
429 & -5.483893e-03 & -7.016265e-02 &        0 &        0 & -2.696846e-03 &  1.437217e-03 &  8.507448e-02 &  9.957023e-02 \\
430 & -5.949497e-02 & -6.743302e-02 &        0 &        0 & -1.136007e-03 &  1.691109e-03 &  4.387637e-02 &  5.658791e-02 \\
431 & -7.522377e-02 & -2.589138e-02 &        0 &        0 &  1.368637e-03 &  5.573597e-04 & -2.224237e-03 &  2.090368e-02 \\
432 & -7.258667e-02 &  9.027686e-03 &        0 &        0 &  2.597185e-03 & -2.445974e-03 &  2.264715e-02 &  2.427445e-03 \\
433 & -7.186759e-02 &  1.529349e-02 &        0 &        0 &  2.722647e-03 &  5.252034e-04 &  8.417543e-02 & -4.019480e-03 \\
434 & -7.908519e-02 &  6.370004e-03 &        0 &        0 & -1.288251e-03 &  5.664493e-04 &  1.019138e-01 & -1.941300e-02 \\
435 & -9.227256e-02 &  4.919124e-03 &        0 &        0 &  5.411641e-04 &  1.069374e-03 &  4.209068e-02 & -2.434920e-02 \\
436 & -1.017815e-01 &  1.328808e-02 &        0 &        0 & -3.414323e-04 &  3.561837e-04 & -1.491966e-02 &  4.380531e-02 \\
437 & -8.529941e-02 & -2.592119e-03 &        0 &        0 & -5.466641e-04 & -2.613007e-03 &  2.170280e-03 &  1.332915e-01 \\
438 & -4.165669e-02 & -4.746341e-02 &        0 &        0 & -1.331552e-03 &  5.738230e-04 &  3.317131e-02 &  1.306086e-01 \\
439 &  1.314376e-02 & -9.107650e-02 &        0 &        0 &  1.381850e-04 & -2.692647e-03 &  5.077036e-02 &  6.563392e-02 \\
440 &  5.901622e-02 & -8.828631e-02 &        0 &        0 & -1.666101e-03 &  4.396004e-03 &  7.005657e-02 &  1.889331e-03 \\
441 &  8.755210e-02 & -3.237144e-02 &        0 &        0 & -7.732441e-04 & -8.965144e-04 &  6.283610e-02 & -4.024082e-03 \\
442 &  8.145104e-02 &  2.023003e-02 &        0 &        0 &  7.142622e-04 & -3.510319e-03 &  5.690489e-02 & -3.787136e-04 \\
443 &  5.234840e-02 &  3.760152e-02 &        0 &        0 & -2.691638e-03 &  4.077927e-04 &  5.053489e-02 & -5.091874e-03 \\
444 &  1.604047e-02 &  2.113886e-02 &        0 &        0 & -4.760873e-04 &  9.819434e-05 &  3.655801e-02 & -5.924576e-03 \\
445 &  2.678692e-04 &  2.366621e-03 &        0 &        0 &  3.095721e-04 &  4.843874e-03 &  1.495134e-02 & -1.869493e-03 \\
446 & -6.409453e-05 &  2.465922e-05 &        0 &        0 &  6.117222e-04 & -2.553222e-03 &  8.951108e-05 & -2.126801e-04 \\
447 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.196467e-14 &  2.423062e-14 &  3.951739e-07 & -4.035827e-06 \\
448 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.088781e-14 &  2.478573e-14 &  4.343822e-07 & -3.106266e-06 \\
449 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.379306e-14 &  1.082467e-14 & -2.876896e-07 &  1.813940e-06 \\
450 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -1.184816e-15 &  1.561251e-15 &  1.506566e-07 & -1.345398e-06 \\
451 &  1.835935e-05 &  9.192519e-05 &        0 &        0 & -1.491575e-04 &  6.831004e-04 &  3.853833e-04 &  3.388369e-04 \\
452 &  1.251791e-02 &  2.291251e-03 &        0 &        0 & -1.433576e-03 &  1.437001e-03 &  9.343884e-04 &  7.592367e-03 \\
453 &  5.871765e-02 &  1.890333e-02 &        0 &        0 &  1.790948e-03 &  1.726467e-04 & -8.633512e-03 & -4.749019e-03 \\
454 &  9.654511e-02 &  2.085875e-02 &        0 &        0 & -4.314712e-03 & -6.275796e-04 & -1.384463e-02 & -1.903878e-03 \\
455 &  1.042438e-01 & -8.126535e-03 &        0 &        0 & -1.015425e-03 &  5.391172e-04 &  2.201322e-02 &  2.456953e-02 \\
456 &  6.249088e-02 & -5.232125e-02 &        0 &        0 & -5.307908e-04 &  6.098284e-03 &  7.298642e-02 &  7.823747e-02 \\
457 & -7.622896e-03 & -7.522217e-02 &        0 &        0 &  1.524682e-03 &  1.154359e-03 &  7.719708e-02 &  1.121826e-01 \\
458 & -5.819822e-02 & -5.080256e-02 &        0 &        0 &  2.733057e-04 & -1.900949e-03 &  5.893838e-02 &  1.162261e-01 \\
459 & -7.062683e-02 & -1.260937e-02 &        0 &        0 & -2.002287e-03 &  1.222468e-03 &  3.116194e-02 &  1.004945e-01 \\
460 & -6.535696e-02 &  2.360640e-03 &        0 &        0 & -1.962480e-03 &  1.783913e-03 &  5.323533e-02 &  8.830437e-02 \\
461 & -6.417512e-02 & -6.514181e-03 &        0 &        0 & -7.367611e-04 &  1.399188e-04 &  7.242820e-02 &  5.743104e-02 \\
462 & -7.112499e-02 & -1.059698e-02 &        0 &        0 & -1.621861e-03 &  6.331979e-04 &  5.520281e-02 &  7.351246e-04 \\
463 & -8.404058e-02 &  4.523746e-03 &        0 &        0 & -5.445309e-04 & -1.708710e-04 &  3.246133e-03 & -1.650769e-02 \\
464 & -8.427049e-02 &  1.561988e-02 &        0 &        0 & -1.752419e-05 &  2.009065e-03 & -4.267724e-02 &  6.520626e-02 \\
465 & -6.015368e-02 & -1.013320e-02 &        0 &        0 &  4.833478e-04 &  4.370816e-04 & -4.585757e-02 &  1.589275e-01 \\
466 & -1.879203e-02 & -6.710146e-02 &        0 &        0 & -4.236634e-04 &  1.653237e-03 & -2.919871e-02 &  1.518758e-01 \\
467 &  3.021051e-02 & -1.049629e-01 &        0 &        0 &  1.182523e-03 &  3.782896e-03 &  2.402180e-04 &  6.579812e-02 \\
468 &  6.689114e-02 & -8.413442e-02 &        0 &        0 & -4.800647e-05 & -1.581293e-03 &  3.235207e-02 & -1.380262e-03 \\
469 &  8.356364e-02 & -1.754262e-02 &        0 &        0 & -9.169920e-04 &  1.037583e-03 &  6.263354e-02 &  1.676284e-03 \\
470 &  7.197319e-02 &  3.093720e-02 &        0 &        0 & -2.986810e-04 &  4.339747e-04 &  5.928246e-02 & -1.640076e-03 \\
471 &  4.202402e-02 &  3.778507e-02 &        0 &        0 &  3.502005e-03 & -1.758937e-05 &  5.498961e-02 &  1.001988e-03 \\
472 &  1.222199e-02 &  1.866686e-02 &        0 &        0 & -1.502453e-03 &  2.072321e-03 &  4.010114e-02 &  8.079559e-04 \\
473 &  1.698400e-04 &  1.736450e-03 &        0 &        0 &  4.990044e-04 &  5.017016e-02 &  1.055408e-02 & -5.881325e-04 \\
474 & -1.679294e-05 &  1.507178e-05 &        0 &        0 &  5.176633e-04 & -2.385132e-03 &  4.925117e-05 & -6.028732e-05 \\
475 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.596068e-15 &  3.594347e-15 & -2.930475e-07 &  2.123501e-06 \\
476 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  2.940790e-15 &  5.551115e-16 &  4.399090e-07 & -3.526421e-06 \\
477 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -5.313106e-15 &  5.551115e-17 & -1.654843e-08 & -5.618685e-08 \\
478 & -4.733328e-05 & -4.117850e-06 &        0 &        0 &  3.821563e-04 & -1.167173e-03 & -1.672417e-05 & -1.581030e-04 \\
479 &  3.655494e-05 &  1.668983e-04 &        0 &        0 &  5.911663e-04 & -1.232225e-03 &  1.982398e-04 &  4.303919e-04 \\
480 &  1.570415e-02 & -1.010326e-03 &        0 &        0 &  1.628386e-03 & -7.352694e-04 &  4.863015e-03 &  6.587558e-03 \\
481 &  6.387308e-02 &  5.977159e-03 &        0 &        0 &  2.315333e-03 & -2.760068e-03 & -1.285066e-02 &  6.555640e-04 \\
482 &  9.978635e-02 &  2.889506e-03 &        0 &        0 &  4.311686e-03 & -6.881288e-04 & -1.172387e-02 & -3.955149e-03 \\
483 &  1.055375e-01 & -2.755672e-02 &        0 &        0 & -7.002536e-05 &  1.040764e-03 &  1.839650e-02 & -4.553415e-04 \\
484 &  6.654498e-02 & -6.731432e-02 &        0 &        0 &  8.719087e-04 & -3.308632e-03 &  4.017947e-02 &  2.322496e-02 \\
485 &  3.715793e-03 & -8.228019e-02 &        0 &        0 & -9.730253e-04 & -2.469982e-03 &  4.196675e-02 &  6.535127e-02 \\
486 & -4.482330e-02 & -5.763649e-02 &        0 &        0 & -1.617515e-04 &  3.507599e-03 &  5.240587e-02 &  8.623339e-02 \\
487 & -5.595698e-02 & -3.172329e-02 &        0 &        0 & -6.041759e-04 & -5.724546e-04 &  6.059018e-02 &  9.513359e-02 \\
488 & -5.290929e-02 & -2.567268e-02 &        0 &        0 &  3.792917e-04 & -9.360762e-04 &  4.564777e-02 &  6.781990e-02 \\
489 & -5.363413e-02 & -2.541235e-02 &        0 &        0 &  3.765390e-05 & -1.871644e-04 &  3.446155e-02 &  3.591354e-03 \\
490 & -6.292798e-02 & -1.650322e-02 &        0 &        0 &  5.594425e-04 &  1.365171e-04 &  3.099538e-02 & -6.401923e-02 \\
491 & -6.985920e-02 &  2.394025e-04 &        0 &        0 &  4.657724e-03 & -1.461815e-03 & -1.179381e-03 & -4.942805e-02 \\
492 & -6.315657e-02 & -3.499813e-03 &        0 &        0 & -2.629017e-03 & -1.347953e-03 & -3.972303e-02 &  5.960744e-02 \\
493 & -3.610494e-02 & -4.286480e-02 &        0 &        0 &  7.438028e-05 &  1.481621e-03 & -5.236998e-02 &  1.448600e-01 \\
494 &  8.405211e-03 & -8.886582e-02 &        0 &        0 &  2.705404e-03 & -2.354368e-03 & -3.477491e-02 &  1.299100e-01 \\
495 &  4.663673e-02 & -9.983921e-02 &        0 &        0 & -1.354154e-03 &  8.881547e-04 & -6.821736e-03 &  5.111066e-02 \\
496 &  7.408325e-02 & -5.546932e-02 &        0 &        0 &  9.789323e-04 & -1.427635e-03 &  4.153451e-02 &  3.060866e-03 \\
497 &  7.496817e-02 &  8.368043e-03 &        0 &        0 &  8.345918e-04 & -2.396345e-04 &  6.117162e-02 &  3.607936e-03 \\
498 &  5.926795e-02 &  4.044215e-02 &        0 &        0 &  6.218130e-05 & -2.003489e-03 &  5.476582e-02 & -2.292298e-03 \\
499 &  3.018331e-02 &  3.296366e-02 &        0 &        0 & -1.248869e-03 &  1.643801e-03 &  4.754873e-02 &  3.952154e-03 \\
500 &  8.919220e-03 &  1.463304e-02 &        0 &        0 &  3.457112e-03 & -1.482336e-02 &  2.246510e-02 &  7.306659e-04 \\
501 & -6.875459e-05 &  9.420436e-04 &        0 &        0 &  1.851976e-03 &  1.668053e-01 &  5.121402e-03 &  4.069198e-04 \\
502 & -8.994523e-05 & -2.192261e-04 &        0 &        0 &  2.878012e-04 & -1.013412e-03 & -1.019078e-04 &  7.787675e-05 \\
503 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  1.140488e-17 & -1.703498e-15 &  2.244402e-07 & -2.043643e-06 \\
504 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -4.452475e-18 &  1.734723e-17 &  2.420686e-07 & -1.880008e-06 \\
505 &  0.000000e+00 & -0.000000e+00 &        0 &        0 & -3.227672e-18 & -1.077263e-15 & -3.782194e-07 &  3.049864e-06 \\
506 & -1.092968e-04 & -9.508491e-06 &        0 &        0 &  3.821723e-04 & -1.167217e-03 & -3.836907e-05 & -3.659483e-04 \\
507 &  1.167069e-04 &  2.542461e-04 &        0 &        0 &  3.769310e-04 & -3.841156e-04 &  1.908319e-04 & -2.484070e-05 \\
508 &  1.664089e-02 & -5.159328e-03 &        0 &        0 &  1.075477e-03 & -4.520919e-04 &  3.510825e-03 &  4.444259e-03 \\
509 &  6.089805e-02 & -4.493563e-03 &        0 &        0 & -5.373320e-03 &  5.007039e-04 & -2.746319e-04 &  1.393440e-02 \\
510 &  9.862495e-02 & -1.063296e-02 &        0 &        0 & -7.980557e-04 &  1.399916e-03 & -7.634501e-03 &  5.760866e-03 \\
511 &  1.067131e-01 & -3.594151e-02 &        0 &        0 & -1.301948e-03 & -1.699238e-03 & -1.955687e-04 & -4.438639e-03 \\
512 &  7.437911e-02 & -6.654549e-02 &        0 &        0 & -3.804326e-04 &  2.144322e-03 &  1.443168e-02 & -6.450393e-03 \\
513 &  1.850121e-02 & -8.262181e-02 &        0 &        0 &  3.210795e-04 &  9.583763e-04 &  1.256237e-03 &  8.780269e-03 \\
514 & -2.599462e-02 & -7.138437e-02 &        0 &        0 &  8.502654e-04 & -2.658723e-03 &  1.392832e-02 &  3.080585e-02 \\
515 & -4.285949e-02 & -5.735454e-02 &        0 &        0 & -2.393164e-04 & -5.508754e-04 &  4.995834e-02 &  3.501798e-02 \\
516 & -4.314758e-02 & -5.065376e-02 &        0 &        0 &  1.156516e-03 &  5.671604e-04 &  4.646771e-02 &  7.764621e-03 \\
517 & -4.559122e-02 & -4.500944e-02 &        0 &        0 & -1.350221e-03 &  3.009991e-04 &  3.139169e-02 & -7.113715e-02 \\
518 & -5.560814e-02 & -3.327660e-02 &        0 &        0 & -1.710049e-03 &  2.115096e-03 &  3.132938e-02 & -1.267264e-01 \\
519 & -5.465414e-02 & -2.717696e-02 &        0 &        0 &  1.381755e-03 &  4.550644e-04 &  1.181231e-02 & -7.527976e-02 \\
520 & -3.873710e-02 & -4.211561e-02 &        0 &        0 &  7.477672e-04 & -2.116296e-03 &  5.024252e-03 &  5.525617e-02 \\
521 & -4.467340e-03 & -7.719329e-02 &        0 &        0 & -2.286714e-03 &  9.229425e-04 & -7.036472e-03 &  1.265207e-01 \\
522 &  3.210299e-02 & -9.052169e-02 &        0 &        0 & -2.322935e-03 &  1.712680e-03 &  1.669445e-02 &  1.051698e-01 \\
523 &  6.222136e-02 & -6.353747e-02 &        0 &        0 &  1.961316e-03 & -1.493485e-03 &  2.152062e-02 &  3.816297e-02 \\
524 &  7.369980e-02 & -8.788008e-03 &        0 &        0 & -3.527079e-03 &  3.549405e-03 &  3.303942e-02 &  8.008512e-03 \\
525 &  6.453579e-02 &  3.327573e-02 &        0 &        0 &  1.389495e-03 &  1.102241e-04 &  4.335333e-02 &  5.989899e-03 \\
526 &  4.184823e-02 &  3.873306e-02 &        0 &        0 &  1.580926e-03 & -1.179459e-03 &  4.564468e-02 &  7.434930e-03 \\
527 &  1.833588e-02 &  2.475373e-02 &        0 &        0 & -6.360094e-04 & -5.522450e-03 &  3.704352e-02 &  2.850024e-03 \\
528 &  4.689209e-03 &  8.677920e-03 &        0 &        0 & -1.762278e-03 &  1.431052e-02 &  1.204888e-02 & -2.554290e-03 \\
529 &  4.731361e-05 &  5.472002e-04 &        0 &        0 &  1.356520e-03 &  8.789641e-02 &  1.212318e-03 & -3.937037e-04 \\
530 & -2.969890e-05 & -7.238599e-05 &        0 &        0 &  2.878026e-04 & -1.013728e-03 & -3.388102e-05 &  2.769902e-05 \\
531 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 &  2.802597e-45 &  3.523747e-07 & -2.064749e-06 \\
532 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -2.802597e-45 & -2.243782e-07 &  2.234083e-06 \\
533 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -1.401298e-45 &  2.376405e-07 & -1.131182e-06 \\
534 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.427395e-07 &  7.283712e-07 \\
535 &  3.015029e-04 & -3.913403e-05 &        0 &        0 & -3.792841e-04 & -2.147494e-04 &  7.728665e-04 &  6.531082e-05 \\
536 &  1.513378e-02 & -7.389839e-03 &        0 &        0 & -1.170938e-03 &  1.493678e-03 &  6.505148e-03 &  4.433888e-03 \\
537 &  5.354056e-02 & -1.195369e-02 &        0 &        0 &  2.111004e-03 & -1.773393e-04 &  9.625450e-03 &  2.011165e-02 \\
538 &  9.206271e-02 & -1.825214e-02 &        0 &        0 & -2.461146e-03 &  7.797713e-04 &  5.049277e-03 &  2.436139e-02 \\
539 &  1.069718e-01 & -3.536911e-02 &        0 &        0 & -1.332844e-03 &  3.182423e-03 & -1.650365e-02 &  1.570156e-03 \\
540 &  8.663077e-02 & -5.651399e-02 &        0 &        0 &  7.517337e-04 & -1.541406e-03 & -1.968020e-02 & -9.957856e-03 \\
541 &  4.459374e-02 & -7.724973e-02 &        0 &        0 & -1.848963e-03 & -2.794492e-05 & -3.303907e-02 & -1.056077e-02 \\
542 &  1.743508e-05 & -8.755506e-02 &        0 &        0 & -3.402084e-04 &  1.340803e-03 & -3.378036e-02 & -9.148789e-03 \\
543 & -2.625140e-02 & -8.673331e-02 &        0 &        0 &  3.758317e-03 & -7.340623e-04 & -3.882835e-03 & -1.346979e-02 \\
544 & -3.549173e-02 & -8.053968e-02 &        0 &        0 & -4.014035e-03 & -7.284177e-05 &  1.098579e-02 & -5.497911e-02 \\
545 & -3.936584e-02 & -7.175883e-02 &        0 &        0 &  1.087721e-03 & -4.488376e-04 &  2.344645e-02 & -1.160977e-01 \\
546 & -4.216276e-02 & -6.271975e-02 &        0 &        0 & -8.057453e-04 & -1.586996e-03 &  4.059148e-02 & -1.256112e-01 \\
547 & -3.111870e-02 & -6.684347e-02 &        0 &        0 &  2.369415e-03 &  3.507957e-03 &  3.700091e-02 & -4.787555e-02 \\
548 & -6.009239e-03 & -8.061605e-02 &        0 &        0 & -1.234991e-03 &  7.863627e-04 &  4.902243e-02 &  6.309130e-02 \\
549 &  2.207684e-02 & -8.137573e-02 &        0 &        0 &  1.726303e-03 & -3.599152e-03 &  3.871360e-02 &  1.149755e-01 \\
550 &  5.226185e-02 & -5.653497e-02 &        0 &        0 &  1.416340e-03 & -2.074750e-03 &  3.328073e-02 &  8.300701e-02 \\
551 &  6.770914e-02 & -5.122448e-03 &        0 &        0 &  1.757754e-03 & -7.145692e-04 &  3.547673e-02 &  4.495745e-02 \\
552 &  6.351522e-02 &  2.960468e-02 &        0 &        0 &  1.870087e-03 & -2.028304e-06 &  3.995662e-02 &  2.087376e-02 \\
553 &  4.881008e-02 &  4.113524e-02 &        0 &        0 & -6.250195e-04 &  1.571972e-03 &  3.057149e-02 &  1.216284e-02 \\
554 &  2.484706e-02 &  3.031299e-02 &        0 &        0 &  9.434856e-04 &  4.051698e-03 &  3.053223e-02 &  8.026638e-03 \\
555 &  9.057751e-03 &  1.631278e-02 &        0 &        0 & -2.366512e-04 &  5.369901e-03 &  2.726399e-02 &  2.612095e-03 \\
556 &  1.692447e-03 &  3.996991e-03 &        0 &        0 &  1.058079e-03 &  6.988393e-03 &  2.973481e-03 & -1.688880e-03 \\
557 &  9.884904e-06 &  2.415830e-04 &        0 &        0 &  3.066746e-04 & -4.189415e-02 &  2.041492e-04 &  2.624973e-04 \\
558 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -6.047679e-07 &  4.747717e-06 \\
559 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  8.090803e-08 & -1.911675e-06 \\
560 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.444234e-07 & -2.098830e-06 \\
561 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.806929e-07 & -1.954777e-06 \\
562 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.569509e-07 & -2.169791e-06 \\
563 &  2.429149e-04 &  9.168984e-05 &        0 &        0 &  1.073085e-04 & -2.495466e-04 &  2.091895e-04 & -7.663926e-04 \\
564 &  1.111912e-02 & -6.530905e-03 &        0 &        0 &  1.329734e-03 &  1.765625e-05 &  9.394308e-03 &  8.317900e-04 \\
565 &  3.802970e-02 & -1.631012e-02 &        0 &        0 & -8.874123e-04 & -2.573819e-04 &  1.565990e-02 &  1.193408e-02 \\
566 &  7.792551e-02 & -2.318909e-02 &        0 &        0 & -1.049686e-03 & -8.009258e-06 &  1.782169e-02 &  3.536505e-02 \\
567 &  1.023534e-01 & -3.292897e-02 &        0 &        0 &  3.201089e-03 & -5.385852e-03 &  4.239147e-04 &  2.016757e-02 \\
568 &  1.007139e-01 & -4.649304e-02 &        0 &        0 & -4.826927e-04 &  1.443185e-03 & -3.458597e-02 & -2.444849e-03 \\
569 &  7.821464e-02 & -6.977329e-02 &        0 &        0 &  1.260943e-03 &  6.673170e-04 & -7.043002e-02 & -1.688016e-02 \\
570 &  4.158062e-02 & -9.426947e-02 &        0 &        0 & -1.937611e-03 & -8.037576e-05 & -8.614165e-02 & -1.238491e-02 \\
571 &  1.225991e-02 & -1.069838e-01 &        0 &        0 &  3.682945e-04 & -7.768826e-04 & -6.301524e-02 & -3.972654e-02 \\
572 & -7.334650e-03 & -1.047990e-01 &        0 &        0 & -2.806774e-03 &  4.908323e-04 & -3.816872e-02 & -8.687642e-02 \\
573 & -1.449466e-02 & -9.684847e-02 &        0 &        0 & -1.659917e-04 &  2.948347e-03 &  2.443682e-03 & -1.180360e-01 \\
574 & -1.111428e-02 & -9.035068e-02 &        0 &        0 & -4.268601e-04 & -1.279428e-03 &  3.122604e-02 & -9.816577e-02 \\
575 &  4.958595e-03 & -8.463857e-02 &        0 &        0 &  1.297600e-03 & -9.752343e-04 &  5.067951e-02 &  7.944889e-04 \\
576 &  2.637485e-02 & -6.911177e-02 &        0 &        0 &  2.790097e-04 &  1.392522e-03 &  5.998503e-02 &  8.698937e-02 \\
577 &  4.932604e-02 & -3.418568e-02 &        0 &        0 & -2.540660e-03 &  1.820103e-03 &  5.281621e-02 &  1.065391e-01 \\
578 &  6.338564e-02 &  9.694172e-03 &        0 &        0 & -3.644945e-03 &  5.379051e-03 &  2.888535e-02 &  7.785012e-02 \\
579 &  6.006904e-02 &  4.423507e-02 &        0 &        0 & -1.522917e-03 &  5.880949e-04 &  3.374554e-02 &  6.786382e-02 \\
580 &  4.786930e-02 &  4.703956e-02 &        0 &        0 & -7.199313e-04 &  4.311919e-03 &  2.543267e-02 &  3.390920e-02 \\
581 &  2.944711e-02 &  3.505368e-02 &        0 &        0 &  4.692244e-04 &  2.300350e-03 &  1.786155e-02 &  1.333262e-02 \\
582 &  1.238627e-02 &  2.027627e-02 &        0 &        0 & -3.120510e-03 &  6.532167e-03 &  2.157942e-02 &  7.077929e-03 \\
583 &  3.625255e-03 &  8.087916e-03 &        0 &        0 & -2.059745e-04 & -4.324569e-03 &  1.071784e-02 & -2.064722e-03 \\
584 &  3.534136e-04 &  1.723241e-03 &        0 &        0 & -2.084024e-03 & -1.666497e-02 & -8.146887e-04 & -7.445823e-04 \\
585 &  3.216547e-05 & -4.045504e-05 &        0 &        0 &  2.699661e-04 &  7.868290e-03 & -5.908757e-04 & -1.890210e-04 \\
586 &  5.901057e-05 & -1.561951e-04 &        0 &        0 & -4.849267e-05 &  4.231611e-03 & -1.329444e-03 & -7.893200e-04 \\
587 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -7.366426e-08 &  3.142441e-07 \\
588 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.626003e-08 & -2.054824e-08 \\
589 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.929321e-08 & -1.232666e-07 \\
590 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.275120e-08 & -8.397158e-07 \\
591 &  1.276555e-04 &  4.204526e-05 &        0 &        0 &  3.637722e-04 & -3.588747e-04 & -2.629940e-04 & -1.253168e-03 \\
592 &  6.372182e-03 & -4.323671e-03 &        0 &        0 & -4.671818e-04 & -1.661435e-03 &  5.587624e-03 &  4.668748e-03 \\
593 &  2.507423e-02 & -1.627059e-02 &        0 &        0 & -1.077033e-03 &  3.373921e-03 &  2.406951e-02 &  1.023851e-02 \\
594 &  5.439854e-02 & -2.488212e-02 &        0 &        0 &  6.907541e-04 &  9.332220e-04 &  2.567044e-02 &  3.203932e-02 \\
595 &  8.859094e-02 & -3.348173e-02 &        0 &        0 &  1.540087e-04 &  2.779735e-03 &  3.006591e-02 &  3.766542e-02 \\
596 &  1.050620e-01 & -3.868530e-02 &        0 &        0 & -1.691291e-03 &  7.690844e-04 & -6.783161e-03 &  1.799297e-02 \\
597 &  1.039182e-01 & -5.644294e-02 &        0 &        0 & -5.025968e-04 & -8.306441e-04 & -5.429895e-02 & -1.273134e-02 \\
598 &  8.618146e-02 & -8.023461e-02 &        0 &        0 &  1.956389e-03 & -4.550548e-04 & -9.227337e-02 & -3.883307e-02 \\
599 &  6.125428e-02 & -9.533455e-02 &        0 &        0 &  1.097497e-03 & -1.954060e-03 & -1.070770e-01 & -8.124238e-02 \\
600 &  3.792580e-02 & -9.987853e-02 &        0 &        0 & -5.903750e-04 &  3.515719e-05 & -9.642137e-02 & -1.236538e-01 \\
601 &  2.707400e-02 & -9.054899e-02 &        0 &        0 & -2.294029e-03 &  1.091562e-03 & -5.121158e-02 & -1.198446e-01 \\
602 &  2.870875e-02 & -7.112199e-02 &        0 &        0 &  4.298768e-03 & -3.043547e-03 & -1.391633e-02 & -5.485141e-02 \\
603 &  4.084742e-02 & -4.547397e-02 &        0 &        0 & -2.093314e-03 &  3.931113e-03 &  6.789429e-03 &  3.494007e-02 \\
604 &  5.424670e-02 & -6.992183e-03 &        0 &        0 & -4.437275e-04 & -1.983115e-03 &  5.548583e-03 &  7.001117e-02 \\
605 &  6.037220e-02 &  3.381457e-02 &        0 &        0 &  3.527609e-03 & -3.503054e-03 & -2.186429e-02 &  8.038967e-02 \\
606 &  5.478670e-02 &  5.531070e-02 &        0 &        0 & -1.918909e-03 & -3.045071e-03 & -1.567783e-02 &  7.103469e-02 \\
607 &  4.122003e-02 &  5.860691e-02 &        0 &        0 &  7.740329e-04 & -4.858990e-03 & -4.111150e-03 &  5.647432e-02 \\
608 &  2.596459e-02 &  4.131405e-02 &        0 &        0 &  8.464827e-05 & -3.083760e-03 & -2.858590e-03 &  2.845046e-02 \\
609 &  1.217398e-02 &  2.233534e-02 &        0 &        0 &  2.247428e-03 & -4.499941e-03 &  9.554746e-03 &  1.080655e-02 \\
610 &  4.212561e-03 &  9.264887e-03 &        0 &        0 &  2.138684e-03 & -7.601440e-04 &  5.283329e-03 & -1.928222e-03 \\
611 &  8.417400e-04 &  2.421735e-03 &        0 &        0 & -5.100264e-05 & -1.475279e-02 & -7.954889e-04 & -2.626483e-03 \\
612 &  1.510842e-04 &  8.917165e-04 &        0 &        0 & -6.839969e-04 & -3.156442e-02 & -1.697560e-03 & -1.425414e-03 \\
613 &  4.466773e-05 & -1.182310e-04 &        0 &        0 & -4.873530e-05 &  4.238613e-03 & -1.006337e-03 & -5.981478e-04 \\
614 &  1.028587e-04 & -2.722568e-04 &        0 &        0 & -4.885215e-05 &  4.276739e-03 & -2.316952e-03 & -1.380458e-03 \\
615 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  8.733876e-08 & -7.953335e-07 \\
616 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.059554e-08 &  1.140726e-06 \\
617 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.319158e-07 &  1.488832e-06 \\
618 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.914210e-09 &  2.223589e-07 \\
619 &  1.230253e-04 &  2.582013e-05 &        0 &        0 & -1.939634e-04 &  6.921972e-04 & -2.843997e-04 & -1.290912e-03 \\
620 &  2.658393e-03 & -2.263636e-03 &        0 &        0 & -1.692542e-03 &  2.043281e-03 &  2.672342e-03 &  5.722581e-04 \\
621 &  1.221136e-02 & -1.060761e-02 &        0 &        0 &  2.008374e-03 & -1.215382e-03 &  1.131489e-02 &  1.036975e-02 \\
622 &  3.075766e-02 & -2.044075e-02 &        0 &        0 &  5.059090e-04 & -3.108585e-03 &  2.328934e-02 &  2.293025e-02 \\
623 &  5.775459e-02 & -3.040094e-02 &        0 &        0 &  2.530837e-03 & -7.946021e-04 &  4.003782e-02 &  3.113570e-02 \\
624 &  8.156595e-02 & -3.536701e-02 &        0 &        0 & -3.906437e-03 & -5.689979e-04 &  3.622289e-02 &  2.306829e-02 \\
625 &  9.709215e-02 & -3.461159e-02 &        0 &        0 &  1.749079e-03 &  8.827187e-04 &  2.303199e-02 & -2.826852e-03 \\
626 &  9.786162e-02 & -3.750784e-02 &        0 &        0 &  8.799255e-04 & -8.964743e-04 & -2.043311e-02 & -4.919775e-02 \\
627 &  8.692649e-02 & -3.627468e-02 &        0 &        0 & -1.213746e-03 &  2.571889e-03 & -5.105252e-02 & -1.052544e-01 \\
628 &  7.272435e-02 & -3.220522e-02 &        0 &        0 & -2.642968e-03 &  4.359278e-04 & -7.257839e-02 & -1.407251e-01 \\
629 &  6.540714e-02 & -1.941404e-02 &        0 &        0 &  3.955272e-03 & -1.046725e-03 & -8.237362e-02 & -1.129374e-01 \\
630 &  6.183351e-02 &  1.198580e-03 &        0 &        0 & -1.946169e-03 & -1.299323e-03 & -6.787993e-02 & -5.457350e-02 \\
631 &  5.890587e-02 &  2.771604e-02 &        0 &        0 &  6.983911e-04 &  3.993406e-03 & -6.772083e-02 &  2.354615e-03 \\
632 &  5.185140e-02 &  5.343954e-02 &        0 &        0 &  2.017964e-04 & -8.064960e-04 & -6.912005e-02 &  4.081725e-02 \\
633 &  4.069575e-02 &  6.399125e-02 &        0 &        0 &  3.343243e-04 &  1.736092e-03 & -5.384049e-02 &  6.036503e-02 \\
634 &  2.832176e-02 &  5.928236e-02 &        0 &        0 &  1.225039e-03 &  1.567753e-03 & -2.659494e-02 &  5.812136e-02 \\
635 &  1.683285e-02 &  4.717893e-02 &        0 &        0 & -2.244276e-03 & -1.183912e-03 & -8.398516e-03 &  5.176928e-02 \\
636 &  8.309360e-03 &  2.743941e-02 &        0 &        0 & -2.620565e-03 & -2.551326e-03 &  2.138040e-03 &  2.583253e-02 \\
637 &  2.690998e-03 &  1.175390e-02 &        0 &        0 &  2.836800e-05 &  3.440898e-03 & -2.205101e-04 &  6.587142e-03 \\
638 &  9.310233e-04 &  3.647568e-03 &        0 &        0 & -1.026480e-03 & -1.307797e-04 &  4.387198e-04 & -1.350458e-05 \\
639 &  3.192033e-04 &  1.164713e-03 &        0 &        0 & -3.849785e-04 &  1.040071e-02 & -1.170744e-03 &  5.538182e-04 \\
640 & -7.677444e-06 &  3.484058e-04 &        0 &        0 & -6.645045e-04 & -2.399386e-02 & -2.855862e-04 &  5.884768e-05 \\
641 &  2.540733e-05 & -6.725069e-05 &        0 &        0 & -4.762684e-05 &  4.272141e-03 & -5.720577e-04 & -3.424596e-04 \\
642 &  5.819098e-05 & -1.540258e-04 &        0 &        0 & -4.807901e-05 &  4.223644e-03 & -1.310673e-03 & -7.813136e-04 \\
643 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.107696e-07 & -1.604061e-06 \\
644 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.648483e-07 & -1.390793e-06 \\
645 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.728228e-07 &  2.100987e-06 \\
646 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  5.770281e-08 & -4.231386e-07 \\
647 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.375539e-07 &  2.052733e-06 \\
648 &  2.291542e-04 & -3.020889e-04 &        0 &        0 &  1.123414e-03 &  1.313229e-03 &  3.560426e-03 & -2.144073e-04 \\
649 &  2.408616e-03 & -3.279394e-03 &        0 &        0 & -1.670524e-03 & -1.004012e-03 &  8.696351e-03 &  6.521142e-03 \\
650 &  8.526450e-03 & -8.032160e-03 &        0 &        0 & -7.951548e-05 &  4.500682e-04 &  1.036790e-02 &  6.483553e-03 \\
651 &  1.951367e-02 & -1.451157e-02 &        0 &        0 & -6.499246e-04 &  3.328614e-04 &  1.510442e-02 &  9.972623e-03 \\
652 &  3.855296e-02 & -2.310323e-02 &        0 &        0 &  1.102603e-04 &  2.455033e-03 &  3.035231e-02 &  8.889450e-03 \\
653 &  5.365519e-02 & -2.357878e-02 &        0 &        0 & -9.278198e-04 & -1.173370e-03 &  3.617799e-02 & -1.077494e-02 \\
654 &  6.145365e-02 & -1.742478e-02 &        0 &        0 &  1.302409e-03 & -1.094883e-03 &  3.216454e-02 & -5.090202e-02 \\
655 &  6.127720e-02 & -3.034293e-03 &        0 &        0 & -9.489240e-04 & -1.529546e-03 &  2.502675e-02 & -9.685246e-02 \\
656 &  5.645513e-02 &  1.528913e-02 &        0 &        0 & -3.893249e-03 &  2.093064e-03 &  8.626384e-03 & -1.106020e-01 \\
657 &  4.896479e-02 &  3.153395e-02 &        0 &        0 &  3.340570e-03 & -1.645126e-03 & -2.278399e-02 & -9.298614e-02 \\
658 &  3.973411e-02 &  4.833956e-02 &        0 &        0 &  5.239055e-04 & -7.074072e-04 & -3.990441e-02 & -5.196040e-02 \\
659 &  3.034684e-02 &  5.767274e-02 &        0 &        0 &  1.109734e-03 & -7.215829e-05 & -2.901702e-02 & -1.859467e-03 \\
660 &  1.752414e-02 &  6.063379e-02 &        0 &        0 & -5.063970e-04 &  1.083473e-03 & -3.019254e-02 &  4.045401e-02 \\
661 &  7.440881e-03 &  5.320686e-02 &        0 &        0 & -1.534009e-03 & -1.437789e-03 & -2.522086e-02 &  6.011892e-02 \\
662 &  2.638265e-03 &  4.213233e-02 &        0 &        0 &  1.411888e-04 &  4.676921e-03 & -7.724718e-03 &  6.767354e-02 \\
663 & -2.865327e-04 &  2.941350e-02 &        0 &        0 &  2.010003e-03 &  3.967871e-04 &  3.794883e-03 &  5.776774e-02 \\
664 & -1.090387e-03 &  1.694903e-02 &        0 &        0 & -2.790807e-04 & -2.663077e-03 &  5.068693e-03 &  3.297992e-02 \\
665 & -7.282639e-04 &  7.911555e-03 &        0 &        0 & -1.997747e-03 & -2.109175e-03 &  4.391878e-03 &  1.598516e-02 \\
666 & -8.854806e-05 &  3.342777e-03 &        0 &        0 &  3.259605e-04 &  6.964695e-03 &  5.083521e-04 &  5.181583e-03 \\
667 &  1.950718e-05 &  9.590923e-04 &        0 &        0 &  2.039971e-04 &  1.668076e-02 & -1.286693e-04 &  2.169381e-03 \\
668 &  1.131031e-05 &  2.181070e-04 &        0 &        0 &  7.356443e-04 &  1.684992e-03 & -3.764074e-05 &  5.768995e-04 \\
669 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.559628e-07 & -1.245331e-06 \\
670 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  8.690056e-08 & -4.056711e-07 \\
671 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  6.806872e-08 & -2.433024e-07 \\
672 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.207071e-07 &  1.007841e-06 \\
673 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.120671e-07 & -1.126850e-06 \\
674 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.300091e-07 &  7.148799e-07 \\
675 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.533684e-07 & -2.013164e-06 \\
676 &  5.752142e-05 & -1.241147e-05 &        0 &        0 &  2.979243e-04 & -1.749378e-03 &  1.024412e-03 & -6.314591e-04 \\
677 & -3.026679e-04 & -1.016699e-04 &        0 &        0 & -2.542523e-04 &  1.113277e-03 &  2.282989e-03 & -2.648844e-03 \\
678 & -5.263870e-04 & -2.437918e-04 &        0 &        0 & -1.518919e-03 &  7.894478e-04 & -3.448436e-04 & -6.898165e-03 \\
679 & -9.710172e-04 & -4.902747e-04 &        0 &        0 &  1.867188e-03 & -1.108736e-03 & -7.176565e-03 & -1.692733e-02 \\
680 & -1.539147e-03 &  7.842676e-04 &        0 &        0 & -2.536817e-05 & -2.970775e-04 & -3.027042e-03 & -2.879378e-02 \\
681 & -3.141459e-04 &  4.779197e-03 &        0 &        0 & -6.301547e-04 &  2.453712e-03 & -1.729831e-03 & -4.652813e-02 \\
682 & -2.076723e-03 &  1.210361e-02 &        0 &        0 &  1.697556e-03 & -1.673684e-03 &  3.501668e-03 & -7.604027e-02 \\
683 & -3.029087e-03 &  1.990605e-02 &        0 &        0 & -1.533078e-03 &  1.341376e-04 &  4.421163e-03 & -9.415513e-02 \\
684 & -2.437847e-03 &  2.802250e-02 &        0 &        0 &  3.812373e-03 & -1.371769e-03 & -2.808198e-03 & -8.649659e-02 \\
685 & -2.227851e-03 &  3.498498e-02 &        0 &        0 & -8.959979e-04 & -1.060860e-03 & -8.458067e-03 & -5.419107e-02 \\
686 & -4.497360e-03 &  3.873036e-02 &        0 &        0 & -1.274695e-04 &  1.874716e-03 & -1.233313e-02 & -1.991986e-02 \\
687 & -7.155401e-03 &  4.032266e-02 &        0 &        0 & -8.596012e-04 & -1.220093e-03 & -1.291461e-02 &  2.658309e-02 \\
688 & -9.749078e-03 &  4.098683e-02 &        0 &        0 &  2.403407e-03 &  1.419855e-03 & -5.429373e-03 &  6.536811e-02 \\
689 & -9.896484e-03 &  3.560768e-02 &        0 &        0 & -8.529057e-04 & -1.482973e-03 &  8.088358e-03 &  8.282008e-02 \\
690 & -8.035330e-03 &  2.877713e-02 &        0 &        0 & -7.105966e-04 &  3.497114e-04 &  1.217831e-02 &  7.974280e-02 \\
691 & -4.470358e-03 &  1.997129e-02 &        0 &        0 & -1.797304e-04 & -3.500160e-03 &  1.280573e-02 &  5.798037e-02 \\
692 & -2.639555e-03 &  1.379105e-02 &        0 &        0 &  2.369316e-03 &  8.204823e-03 &  9.948906e-03 &  3.891929e-02 \\
693 & -1.611075e-03 &  7.851650e-03 &        0 &        0 &  1.465724e-03 &  1.276916e-02 &  6.436381e-03 &  2.189297e-02 \\
694 & -6.684896e-04 &  3.760736e-03 &        0 &        0 &  1.206061e-03 &  1.379977e-02 &  3.560263e-03 &  1.002855e-02 \\
695 & -1.581033e-04 &  1.284376e-03 &        0 &        0 &  1.362796e-03 &  3.716244e-03 &  1.072603e-03 &  3.207809e-03 \\
696 &  1.569320e-05 &  1.844352e-04 &        0 &        0 &  7.211482e-04 &  3.666438e-03 & -2.469670e-05 &  5.565534e-04 \\
697 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.874466e-07 &  1.272941e-06 \\
698 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.364296e-07 &  1.523434e-06 \\
699 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.958519e-07 &  1.393056e-06 \\
700 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -7.964441e-07 &  5.984207e-06 \\
701 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.750126e-07 &  1.505852e-06 \\
702 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.578868e-08 & -1.210094e-06 \\
703 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.261442e-07 &  2.146378e-06 \\
704 & -5.656005e-05 &  7.435762e-06 &        0 &        0 &  4.801383e-04 & -3.018557e-03 & -6.238199e-05 & -2.382077e-04 \\
705 & -5.820547e-04 &  3.144388e-05 &        0 &        0 &  7.624410e-04 & -4.150980e-03 & -5.346205e-04 & -3.095694e-03 \\
706 & -1.403600e-03 &  8.507014e-05 &        0 &        0 &  1.257621e-03 & -5.703846e-03 & -1.135298e-03 & -7.204609e-03 \\
707 & -3.259427e-03 &  2.521216e-04 &        0 &        0 &  1.923377e-03 & -7.267389e-03 & -2.566949e-03 & -1.765047e-02 \\
708 & -6.386035e-03 &  1.775353e-03 &        0 &        0 & -2.589965e-04 &  6.545213e-04 & -3.671900e-03 & -3.719072e-02 \\
709 & -1.047250e-02 &  5.648505e-03 &        0 &        0 &  8.791606e-05 & -7.834184e-04 & -4.043827e-03 & -6.009235e-02 \\
710 & -1.477581e-02 &  1.069580e-02 &        0 &        0 & -3.189530e-04 & -1.029635e-03 & -6.226771e-03 & -8.027372e-02 \\
711 & -1.667399e-02 &  1.454276e-02 &        0 &        0 & -4.720623e-05 & -2.117163e-03 & -7.404146e-03 & -7.999208e-02 \\
712 & -1.667474e-02 &  1.831108e-02 &        0 &        0 & -4.390325e-04 &  1.126803e-03 & -7.880757e-03 & -5.840238e-02 \\
713 & -1.540295e-02 &  1.979781e-02 &        0 &        0 & -8.065292e-04 &  2.799086e-03 & -5.440661e-03 & -2.352277e-02 \\
714 & -1.375604e-02 &  2.066811e-02 &        0 &        0 & -1.823079e-04 & -3.435751e-04 & -9.385225e-04 &  7.063822e-03 \\
715 & -1.295598e-02 &  2.302605e-02 &        0 &        0 &  1.408122e-04 & -1.496174e-03 &  1.445463e-03 &  3.477551e-02 \\
716 & -1.224512e-02 &  2.513088e-02 &        0 &        0 &  4.389574e-03 & -1.563694e-02 &  5.124301e-03 &  5.897572e-02 \\
717 & -1.025611e-02 &  2.440067e-02 &        0 &        0 &  4.201773e-03 & -1.677160e-02 &  7.993529e-03 &  6.786777e-02 \\
718 & -7.095916e-03 &  1.922932e-02 &        0 &        0 &  3.932051e-03 & -1.672007e-02 &  8.361240e-03 &  5.705012e-02 \\
719 & -3.501526e-03 &  1.275257e-02 &        0 &        0 &  3.247515e-03 & -1.238979e-02 &  7.693153e-03 &  3.888613e-02 \\
720 & -2.074388e-03 &  9.981586e-03 &        0 &        0 &  3.168770e-03 & -1.004380e-02 &  7.789845e-03 &  3.052979e-02 \\
721 & -1.199328e-03 &  5.825877e-03 &        0 &        0 &  2.577584e-03 & -5.364812e-03 &  5.881463e-03 &  1.780930e-02 \\
722 & -4.827425e-04 &  2.289409e-03 &        0 &        0 &  2.013705e-03 & -1.976114e-03 &  1.876908e-03 &  6.689220e-03 \\
723 & -7.144247e-05 &  8.653296e-04 &        0 &        0 &  1.338511e-03 &  1.032021e-03 &  6.002393e-04 &  2.318554e-03 \\
724 &  1.799549e-05 &  1.147735e-04 &        0 &        0 &  7.134833e-04 &  1.805383e-03 & -2.059450e-06 &  3.871980e-04 \\
725 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.053511e-07 &  1.603449e-06 \\
726 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.628189e-07 & -2.775430e-06 \\
727 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -2.121736e-07 &  1.098053e-06 \\
728 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.554652e-08 &  2.507246e-07 \\
729 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.653951e-07 &  2.711407e-06 \\
730 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.619260e-07 & -4.531765e-06 \\
731 & -2.539976e-05 &  3.776514e-06 &        0 &        0 &  4.075603e-04 & -2.682511e-03 & -3.157832e-05 & -8.944806e-05 \\
732 & -2.294575e-04 &  4.397760e-05 &        0 &        0 &  5.070693e-04 & -3.210839e-03 & -2.296889e-04 & -8.498275e-04 \\
733 & -2.738462e-04 &  7.203465e-05 &        0 &        0 &  6.234298e-04 & -3.415640e-03 & -2.140380e-04 & -1.114763e-03 \\
734 & -6.135806e-04 &  2.877789e-04 &        0 &        0 &  1.039610e-03 & -3.942357e-03 & -3.777316e-04 & -2.573742e-03 \\
735 & -1.152899e-03 &  2.874451e-04 &        0 &        0 &  1.309093e-03 & -4.957458e-03 & -6.886852e-04 & -5.634530e-03 \\
736 & -2.504250e-03 &  1.231505e-03 &        0 &        0 &  1.452820e-03 & -5.796370e-03 & -1.182716e-03 & -1.307078e-02 \\
737 & -3.500268e-03 &  2.205908e-03 &        0 &        0 &  1.821299e-03 & -7.194959e-03 & -5.157759e-04 & -1.825424e-02 \\
738 & -4.122172e-03 &  3.315886e-03 &        0 &        0 &  2.020664e-03 & -7.528529e-03 & -7.865079e-04 & -2.040024e-02 \\
739 & -4.730412e-03 &  4.723346e-03 &        0 &        0 &  2.284612e-03 & -7.711842e-03 & -2.057993e-03 & -2.228362e-02 \\
740 & -4.602826e-03 &  5.233970e-03 &        0 &        0 &  2.596169e-03 & -7.639656e-03 & -2.110275e-03 & -1.471045e-02 \\
741 & -4.687762e-03 &  5.631350e-03 &        0 &        0 &  2.589763e-03 & -7.380886e-03 & -1.685145e-03 & -6.924358e-03 \\
742 & -4.594130e-03 &  6.861088e-03 &        0 &        0 &  2.653358e-03 & -7.986959e-03 & -4.720930e-04 &  2.957146e-03 \\
743 & -3.194886e-03 &  5.962465e-03 &        0 &        0 &  2.506563e-03 & -8.312009e-03 &  4.699280e-04 &  9.232595e-03 \\
744 & -3.138126e-03 &  5.993809e-03 &        0 &        0 &  2.759348e-03 & -1.021936e-02 & -2.052871e-04 &  1.080728e-02 \\
745 & -3.120424e-03 &  5.910728e-03 &        0 &        0 &  2.790179e-03 & -1.150426e-02 &  1.088090e-03 &  1.481753e-02 \\
746 & -1.902058e-03 &  4.865051e-03 &        0 &        0 &  2.662167e-03 & -1.154675e-02 &  1.455103e-03 &  1.401418e-02 \\
747 & -7.870360e-04 &  3.124732e-03 &        0 &        0 &  2.322850e-03 & -9.592799e-03 &  1.673265e-03 &  9.132533e-03 \\
748 & -5.203996e-04 &  2.650716e-03 &        0 &        0 &  2.270236e-03 & -8.774401e-03 &  2.063943e-03 &  7.664802e-03 \\
749 & -3.035289e-04 &  1.405776e-03 &        0 &        0 &  1.755095e-03 & -7.045795e-03 &  1.495945e-03 &  4.152378e-03 \\
750 & -1.336764e-04 &  6.661387e-04 &        0 &        0 &  1.338670e-03 & -5.880489e-03 &  9.119532e-04 &  1.904064e-03 \\
751 & -6.115193e-05 &  1.684902e-04 &        0 &        0 &  8.708382e-04 & -6.086616e-03 &  3.093695e-04 &  6.676371e-04 \\
752 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.277224e-08 &  3.678207e-07 \\
753 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -9.432101e-08 &  6.297361e-07 \\
754 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  3.887771e-07 & -2.257308e-06 \\
755 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.121910e-07 &  2.923001e-06 \\
756 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.698289e-07 & -8.280658e-07 \\
757 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.326109e-08 &  2.203798e-07 \\
758 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.829657e-07 &  6.956469e-07 \\
759 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.219401e-07 & -1.221734e-07 \\
760 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  4.143857e-08 & -5.400419e-07 \\
761 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.448895e-07 & -7.887377e-07 \\
762 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.155962e-07 &  2.835623e-07 \\
763 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -3.047080e-07 &  1.436881e-06 \\
764 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.165546e-07 & -5.583973e-08 \\
765 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.706236e-07 & -3.528978e-06 \\
766 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.127575e-07 & -7.334223e-07 \\
767 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -4.601625e-07 &  2.197969e-06 \\
768 & -1.143231e-04 &  1.686249e-04 &        0 &        0 &  8.932923e-04 & -2.657314e-03 &  2.274475e-05 & -2.905560e-04 \\
769 & -1.526303e-04 &  2.251274e-04 &        0 &        0 &  8.932279e-04 & -2.657234e-03 &  2.974565e-05 & -3.828062e-04 \\
770 & -2.166498e-04 &  2.988404e-04 &        0 &        0 &  9.664795e-04 & -2.926651e-03 &  9.634065e-05 & -9.480504e-05 \\
771 & -9.736587e-05 &  1.977599e-04 &        0 &        0 &  5.543896e-04 & -1.764739e-03 & -2.327252e-04 &  3.348210e-04 \\
772 & -2.781882e-05 &  5.650283e-05 &        0 &        0 &  5.544265e-04 & -1.764233e-03 & -6.641999e-05 &  9.534805e-05 \\
773 & -6.131117e-06 &  1.867469e-05 &        0 &        0 &  7.252392e-04 & -3.394297e-03 & -1.906180e-05 &  5.326081e-05 \\
774 & -9.765993e-05 &  2.974611e-04 &        0 &        0 &  7.252445e-04 & -3.394531e-03 & -3.036544e-04 &  8.470606e-04 \\
775 & -1.312188e-04 &  3.809572e-04 &        0 &        0 &  1.156035e-03 & -5.660519e-03 &  1.585996e-04 &  1.076871e-03 \\
776 & -7.612529e-05 &  2.147086e-04 &        0 &        0 &  9.028760e-04 & -4.529890e-03 &  2.825623e-04 &  6.055212e-04 \\
777 & -1.064689e-06 &  3.002917e-06 &        0 &        0 &  9.027813e-04 & -4.529981e-03 &  4.099209e-06 &  7.418294e-06 \\
778 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.176837e-07 &  1.236332e-06 \\
779 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  1.891777e-07 & -7.408221e-07 \\
780 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.893937e-07 &  2.044022e-06 \\
781 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.548861e-07 &  2.498715e-07 \\
782 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 & -1.560577e-07 &  1.256534e-06 \\
783 &  0.000000e+00 & -0.000000e+00 &        0 &        0 &  0.000000e+00 & -0.000000e+00 &  2.580391e-07 & -2.282799e-06 \\
\bottomrule
\end{tabular}


==> supp_material/tables/mnist3.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &       PCA (x) &       PCA (y) &       LDA (x) &  LDA (y) &      cPCA (x) &      cPCA (y) &      ULCA (x) &      ULCA (y) \\
\midrule
0   & -4.183592e-19 & -1.224049e-17 &  1.295342e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.354788e-07 & -7.421505e-07 \\
1   &  7.787969e-20 &  4.517303e-18 &  9.532343e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -7.634806e-08 & -9.811310e-07 \\
2   &  3.176460e-21 &  8.245845e-19 &  2.359764e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -2.730045e-09 &  8.759358e-08 \\
3   & -1.105794e-22 & -7.281876e-20 &  3.944335e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  6.074020e-09 & -1.893867e-07 \\
4   &  7.444040e-23 &  3.719896e-21 &  1.198318e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -5.784275e-08 & -6.370762e-07 \\
5   &  1.609595e-23 &  2.362441e-21 &  7.919001e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -4.079243e-08 & -1.256134e-07 \\
6   &  5.758668e-24 & -1.401921e-22 & -3.132630e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.700731e-07 & -1.980026e-06 \\
7   & -5.086133e-25 &  6.883605e-22 &  3.528930e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -3.563317e-07 & -2.277381e-06 \\
8   &  3.802730e-25 &  7.673368e-22 &  3.026526e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -4.015076e-08 & -4.242980e-07 \\
9   &  2.087752e-24 & -2.585275e-24 & -1.885094e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  9.904881e-09 &  2.522994e-07 \\
10  &  1.247072e-25 &  1.231171e-23 & -1.843702e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.568180e-09 & -1.918425e-07 \\
11  &  0.000000e+00 & -0.000000e+00 & -4.573644e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  5.098312e-08 &  3.772624e-07 \\
12  &  0.000000e+00 & -0.000000e+00 &  1.648613e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -2.904843e-08 & -1.102173e-06 \\
13  &  0.000000e+00 & -0.000000e+00 & -9.420464e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 &  4.830415e-09 & -2.232441e-07 \\
14  &  0.000000e+00 & -0.000000e+00 &  1.688551e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  6.149314e-09 &  1.924714e-07 \\
15  &  0.000000e+00 & -0.000000e+00 &  1.577888e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -2.342155e-07 & -1.719210e-06 \\
16  &  0.000000e+00 & -0.000000e+00 & -4.386907e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -9.289876e-08 & -7.485167e-07 \\
17  &  0.000000e+00 & -0.000000e+00 &  2.496563e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -5.586895e-09 &  4.811977e-07 \\
18  &  0.000000e+00 & -0.000000e+00 & -1.251645e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -2.258506e-07 & -1.655178e-06 \\
19  &  0.000000e+00 & -0.000000e+00 & -5.117860e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.474375e-07 & -1.640953e-06 \\
20  &  0.000000e+00 & -0.000000e+00 & -3.087279e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -9.420554e-08 & -1.119158e-06 \\
21  &  0.000000e+00 & -0.000000e+00 & -3.177542e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  3.615324e-09 & -4.517746e-09 \\
22  &  0.000000e+00 & -0.000000e+00 & -3.912037e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.847213e-07 &  2.294921e-06 \\
23  &  0.000000e+00 & -0.000000e+00 &  1.761772e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -7.604932e-08 & -5.346135e-07 \\
24  &  0.000000e+00 & -0.000000e+00 & -8.351365e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 &  8.597319e-09 &  6.009680e-07 \\
25  &  0.000000e+00 & -0.000000e+00 & -5.393091e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 &  9.017562e-08 &  7.283661e-07 \\
26  &  0.000000e+00 & -0.000000e+00 & -1.474810e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -8.422908e-08 & -1.912820e-07 \\
27  &  0.000000e+00 & -0.000000e+00 & -2.985699e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.315837e-07 &  1.083695e-06 \\
28  &  0.000000e+00 & -0.000000e+00 & -3.161739e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  6.130403e-08 &  3.137327e-07 \\
29  &  0.000000e+00 & -0.000000e+00 &  3.070915e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -4.565161e-08 & -9.973168e-07 \\
30  &  0.000000e+00 & -0.000000e+00 &  4.721684e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.054850e-07 & -1.171744e-06 \\
31  &  0.000000e+00 & -0.000000e+00 &  4.866497e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.754731e-07 &  1.964277e-06 \\
32  &  0.000000e+00 & -0.000000e+00 &  7.151554e-15 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.437797e-08 & -4.325023e-07 \\
33  &  0.000000e+00 & -0.000000e+00 & -1.819240e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 &  6.925413e-09 &  4.527182e-07 \\
34  &  0.000000e+00 & -0.000000e+00 & -5.666469e-14 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.258627e-08 & -3.619929e-07 \\
35  &  2.141479e-05 &  1.420014e-04 & -7.352240e+01 &      0.0 &  1.583297e-03 &  2.335186e-01 &  2.568555e-04 & -5.793345e-04 \\
36  &  6.934092e-05 &  4.678014e-04 & -1.962945e+01 &      0.0 &  1.949582e-03 &  2.806236e-01 &  8.152129e-04 & -1.984736e-03 \\
37  &  9.065501e-05 &  6.198905e-04 & -7.149667e+00 &      0.0 &  2.050037e-03 &  2.923686e-01 &  1.048452e-03 & -2.709241e-03 \\
38  &  4.795025e-05 &  3.302028e-04 & -3.658729e-01 &      0.0 &  2.006537e-03 &  2.386235e-01 &  8.427568e-04 & -1.612413e-03 \\
39  & -1.469842e-04 & -3.991379e-05 &  1.872275e+00 &      0.0 &  1.027811e-03 &  3.597852e-02 &  1.455993e-03 & -1.798044e-03 \\
40  & -1.864405e-04 & -1.747396e-04 & -4.550300e+00 &      0.0 &  1.029379e-03 &  2.293562e-02 &  1.193725e-03 & -1.714106e-03 \\
41  & -3.504243e-04 & -1.612665e-04 &  3.758025e+00 &      0.0 &  8.124271e-04 &  2.308845e-03 &  1.935696e-03 & -9.220551e-04 \\
42  & -1.462095e-04 &  3.774568e-05 & -2.003086e+00 &      0.0 &  8.027485e-04 & -1.347593e-03 &  7.821252e-04 &  4.996679e-04 \\
43  & -2.795246e-04 & -1.016705e-04 &  1.043152e+00 &      0.0 &  1.099934e-03 & -2.285887e-03 &  8.327130e-04 &  7.155515e-04 \\
44  & -1.122669e-04 & -3.305159e-04 &  1.897205e-01 &      0.0 &  1.130170e-03 & -1.920199e-03 &  1.291988e-03 &  2.736125e-03 \\
45  & -1.704614e-04 & -9.559968e-05 & -1.446782e+00 &      0.0 &  9.266115e-04 & -2.979863e-03 &  2.305191e-03 &  2.034194e-03 \\
46  & -2.150866e-04 & -2.517954e-04 &  1.245240e+01 &      0.0 &  7.163069e-04 & -2.519505e-03 &  1.470769e-03 &  1.437517e-03 \\
47  & -2.070278e-04 & -4.578286e-04 & -4.575480e+01 &      0.0 &  5.698027e-04 & -2.648679e-03 &  3.631574e-04 &  4.204306e-04 \\
48  & -2.751982e-04 & -6.870285e-04 &  4.937909e+01 &      0.0 &  5.177502e-04 & -2.630828e-03 &  1.487770e-04 & -4.626427e-04 \\
49  & -1.766674e-04 & -3.502529e-04 & -1.712983e+02 &      0.0 &  5.979898e-04 & -2.736392e-03 &  1.169930e-04 & -1.739498e-04 \\
50  & -9.764449e-05 & -1.747686e-04 &  2.420220e+02 &      0.0 &  5.077856e-04 & -2.224043e-03 &  9.561329e-05 &  2.421866e-05 \\
51  &  0.000000e+00 & -0.000000e+00 & -3.956954e-14 &      0.0 & -5.737915e-06 &  1.334266e-05 &  3.825847e-08 &  5.069149e-07 \\
52  &  0.000000e+00 & -0.000000e+00 &  1.653090e-14 &      0.0 &  2.409297e-06 & -4.034532e-05 & -8.884417e-09 &  6.404168e-07 \\
53  &  0.000000e+00 & -0.000000e+00 & -2.343674e-14 &      0.0 &  1.424714e-06 & -2.870812e-05 & -1.717234e-07 & -1.758253e-06 \\
54  &  0.000000e+00 & -0.000000e+00 & -1.182942e-14 &      0.0 & -1.936585e-06 & -5.577442e-06 & -1.950183e-07 & -1.915032e-06 \\
55  &  0.000000e+00 & -0.000000e+00 & -1.045322e-14 &      0.0 & -3.847935e-06 &  2.021725e-05 & -4.298687e-08 & -1.706686e-07 \\
56  &  0.000000e+00 & -0.000000e+00 &  1.686125e-14 &      0.0 & -2.354756e-06 & -2.691240e-05 & -3.391964e-07 & -2.790238e-06 \\
57  &  0.000000e+00 & -0.000000e+00 & -2.782510e-14 &      0.0 & -2.872221e-06 & -4.063779e-05 &  1.411951e-07 &  1.241352e-06 \\
58  &  0.000000e+00 & -0.000000e+00 & -5.383498e-15 &      0.0 &  6.304099e-08 &  1.294663e-05 & -2.217247e-07 & -1.610221e-06 \\
59  &  0.000000e+00 & -0.000000e+00 &  2.034847e-14 &      0.0 & -5.616317e-06 & -5.771643e-06 &  3.642761e-08 &  7.666309e-07 \\
60  & -1.454007e-05 & -1.217337e-04 &  1.378513e+01 &      0.0 &  4.699355e-04 &  1.493275e-02 &  1.175857e-04 &  2.141112e-05 \\
61  & -3.233936e-06 & -7.997807e-06 & -2.051496e+02 &      0.0 &  1.188110e-03 &  1.798177e-01 &  3.647649e-05 & -8.396540e-05 \\
62  & -8.019936e-06 &  2.130564e-05 & -6.591551e+01 &      0.0 &  1.102102e-03 &  1.965552e-01 &  1.125136e-04 & -4.013025e-04 \\
63  &  1.521343e-05 &  1.342131e-04 &  2.131554e+02 &      0.0 &  2.299375e-03 &  3.378341e-01 &  2.914481e-04 & -6.619439e-04 \\
64  &  8.817533e-05 &  7.078329e-04 &  7.837141e+00 &      0.0 &  2.237729e-03 &  2.969654e-01 &  1.914838e-03 & -2.540221e-03 \\
65  &  1.996231e-04 &  1.101083e-03 &  3.259697e+00 &      0.0 &  2.241431e-03 &  2.541362e-01 &  2.805111e-03 & -4.616191e-03 \\
66  & -7.881816e-05 &  1.358876e-03 & -2.473768e+00 &      0.0 &  2.375113e-03 &  2.017457e-01 &  5.725711e-03 & -8.323195e-03 \\
67  & -4.682708e-04 &  1.021616e-03 &  3.772784e+00 &      0.0 &  1.935793e-03 &  6.533136e-02 &  7.092321e-03 & -7.317551e-03 \\
68  & -9.109280e-04 &  1.299545e-03 & -3.852478e+00 &      0.0 &  2.077393e-03 &  2.399036e-02 &  9.427266e-03 & -6.122367e-03 \\
69  & -2.388379e-03 &  1.444104e-03 &  2.132826e-01 &      0.0 &  2.384291e-03 &  2.680245e-03 &  1.775380e-02 & -6.408553e-03 \\
70  & -4.785381e-03 & -8.411673e-04 & -7.592319e-01 &      0.0 &  3.023460e-03 & -5.692958e-03 &  2.762537e-02 & -2.031032e-03 \\
71  & -6.699286e-03 & -6.605259e-03 & -7.583703e-01 &      0.0 &  3.575491e-03 & -8.521369e-03 &  3.241505e-02 &  9.007608e-03 \\
72  & -1.019139e-02 & -1.725007e-02 & -3.520139e-01 &      0.0 &  4.136666e-03 & -1.204051e-02 &  3.959255e-02 &  1.734984e-02 \\
73  & -1.050355e-02 & -2.418862e-02 & -2.039317e-01 &      0.0 &  4.117270e-03 & -1.149372e-02 &  3.615650e-02 &  1.829145e-02 \\
74  & -8.755442e-03 & -2.466402e-02 & -1.721708e-01 &      0.0 &  3.513699e-03 & -9.111856e-03 &  2.263078e-02 &  1.349063e-02 \\
75  & -6.277631e-03 & -1.914394e-02 & -2.077700e-01 &      0.0 &  2.649492e-03 & -7.408460e-03 &  1.208623e-02 &  1.630178e-02 \\
76  & -3.390335e-03 & -1.048849e-02 &  6.003296e-01 &      0.0 &  1.981627e-03 & -7.469066e-03 &  3.823859e-03 &  1.742398e-02 \\
77  & -1.540892e-03 & -4.769707e-03 & -3.422104e-01 &      0.0 &  1.475993e-03 & -6.115922e-03 &  1.314321e-03 &  7.576187e-03 \\
78  & -4.380928e-04 & -1.390021e-03 & -4.435657e+00 &      0.0 &  1.019801e-03 & -4.293997e-03 &  3.647472e-04 &  2.300950e-03 \\
79  & -2.505553e-05 & -9.833882e-05 &  1.290757e+01 &      0.0 &  5.692455e-04 & -2.147084e-03 &  6.754745e-05 &  3.512360e-04 \\
80  & -6.520683e-06 & -2.126382e-05 & -2.726552e+01 &      0.0 &  1.248884e-03 & -1.713421e-03 &  4.163268e-05 &  9.981409e-05 \\
81  &  0.000000e+00 & -0.000000e+00 &  4.232255e-15 &      0.0 &  4.023413e-07 &  2.100001e-05 & -7.556030e-08 & -7.566073e-07 \\
82  &  0.000000e+00 & -0.000000e+00 &  2.501949e-14 &      0.0 & -1.948925e-06 & -1.342980e-05 & -1.640708e-08 &  1.506199e-07 \\
83  &  0.000000e+00 & -0.000000e+00 &  1.473186e-14 &      0.0 & -3.084184e-06 &  7.520904e-06 &  8.912627e-08 &  8.417636e-07 \\
84  &  0.000000e+00 & -0.000000e+00 & -1.254162e-14 &      0.0 & -3.754817e-06 & -2.678965e-05 &  6.660525e-08 &  7.408630e-07 \\
85  &  0.000000e+00 & -0.000000e+00 &  7.282512e-15 &      0.0 & -9.156694e-07 &  2.497910e-05 & -4.829052e-09 & -4.822623e-07 \\
86  &  0.000000e+00 & -0.000000e+00 & -1.132276e-14 &      0.0 &  1.994162e-06 &  2.416565e-05 &  6.411659e-08 &  3.815773e-07 \\
87  &  0.000000e+00 & -0.000000e+00 & -8.967950e-15 &      0.0 &  5.126476e-06 &  1.230141e-05 & -2.028810e-07 & -2.183019e-06 \\
88  & -1.504145e-06 & -1.259314e-05 &  1.332563e+02 &      0.0 &  4.689365e-04 &  1.489937e-02 &  1.240606e-05 &  4.053650e-06 \\
89  & -2.745557e-05 &  7.017322e-05 & -1.940460e+01 &      0.0 &  1.100655e-03 &  1.966946e-01 &  3.834838e-04 & -1.361757e-03 \\
90  & -8.530241e-06 & -1.859624e-05 & -8.658566e-01 &      0.0 &  1.171200e-03 &  1.772907e-01 &  8.212000e-04 & -2.560975e-03 \\
91  & -2.847442e-05 &  1.613056e-04 & -1.001353e+02 &      0.0 &  1.609475e-03 &  2.367045e-01 &  4.334857e-04 & -1.602711e-03 \\
92  &  2.245414e-04 &  1.232845e-03 & -2.600890e+00 &      0.0 &  2.146825e-03 &  2.600684e-01 &  2.392344e-03 & -3.558123e-03 \\
93  &  1.814068e-04 &  1.778926e-03 &  4.474007e-01 &      0.0 & -2.074319e-03 &  2.903133e-02 &  4.185012e-03 & -5.543069e-03 \\
94  & -1.128339e-04 &  2.853918e-03 & -1.943171e+00 &      0.0 &  1.904411e-04 & -2.357457e-02 &  9.347135e-03 & -9.802133e-03 \\
95  & -4.200657e-04 &  3.848930e-03 &  7.453172e-01 &      0.0 &  2.284668e-03 & -1.783358e-03 &  1.218302e-02 & -1.198881e-02 \\
96  & -1.188916e-03 &  4.396880e-03 &  1.376382e+00 &      0.0 & -1.635598e-03 &  2.536130e-03 &  1.893957e-02 & -1.737063e-02 \\
97  & -3.756395e-03 &  2.019962e-03 & -1.094334e-01 &      0.0 & -3.585004e-04 & -5.895626e-04 &  2.985720e-02 & -1.777519e-02 \\
98  & -1.005784e-02 & -6.120505e-03 &  4.431842e-01 &      0.0 &  2.404350e-04 & -2.779238e-05 &  4.546214e-02 & -1.101806e-02 \\
99  & -1.605898e-02 & -2.511137e-02 &  3.288672e-01 &      0.0 & -6.997421e-04 & -8.768929e-04 &  5.765001e-02 &  7.019447e-03 \\
100 & -2.054124e-02 & -4.378049e-02 & -6.547455e-01 &      0.0 &  1.058115e-03 & -2.300214e-04 &  5.772202e-02 &  2.441825e-02 \\
101 & -2.231438e-02 & -5.559642e-02 &  4.536576e-01 &      0.0 & -1.482627e-03 &  8.686634e-04 &  3.603985e-02 &  2.593713e-02 \\
102 & -1.835703e-02 & -5.298794e-02 & -1.073841e+00 &      0.0 &  6.196251e-04 & -3.101986e-03 &  1.845212e-02 &  2.477313e-02 \\
103 & -1.288975e-02 & -4.037894e-02 &  2.842032e-01 &      0.0 & -1.607644e-03 &  5.638135e-03 &  4.303889e-03 &  2.259102e-02 \\
104 & -6.496134e-03 & -2.143974e-02 & -1.232521e+00 &      0.0 & -1.834041e-05 & -7.295467e-03 & -5.097892e-04 &  2.176031e-02 \\
105 & -2.715744e-03 & -8.899738e-03 & -4.340858e-01 &      0.0 &  9.557631e-04 &  2.247964e-03 &  1.620572e-04 &  1.123431e-02 \\
106 & -7.492111e-04 & -2.922975e-03 &  2.436918e+00 &      0.0 &  1.693799e-03 & -4.614625e-03 & -1.282651e-03 &  4.810104e-03 \\
107 & -9.175876e-05 & -5.763812e-04 &  7.551969e-01 &      0.0 &  1.377909e-03 & -2.851387e-03 & -3.342139e-04 &  1.561901e-03 \\
108 & -3.369020e-05 & -1.098631e-04 & -5.277197e+00 &      0.0 &  1.254801e-03 & -1.749443e-03 &  2.153909e-04 &  5.187235e-04 \\
109 &  0.000000e+00 & -0.000000e+00 & -2.161919e-15 &      0.0 &  1.159026e-06 &  5.797796e-06 &  1.195789e-07 &  1.599583e-06 \\
110 &  0.000000e+00 & -0.000000e+00 & -1.884866e-15 &      0.0 & -5.982250e-08 &  3.884795e-07 & -1.775528e-07 & -8.071493e-07 \\
111 &  0.000000e+00 & -0.000000e+00 & -3.935844e-15 &      0.0 & -1.504604e-06 & -7.331128e-06 &  9.324869e-09 &  6.950427e-08 \\
112 &  0.000000e+00 & -0.000000e+00 & -6.011358e-15 &      0.0 & -3.021971e-07 &  1.388899e-05 &  1.500831e-08 & -1.491739e-07 \\
113 &  0.000000e+00 & -0.000000e+00 & -2.366015e-14 &      0.0 & -2.587492e-06 &  1.364018e-06 &  7.199675e-08 &  1.135389e-06 \\
114 &  0.000000e+00 & -0.000000e+00 &  2.036192e-14 &      0.0 & -1.692745e-06 & -8.251351e-06 & -9.281951e-08 & -8.944730e-07 \\
115 &  0.000000e+00 & -0.000000e+00 &  6.113864e-15 &      0.0 &  1.464686e-06 & -4.861578e-06 &  4.927244e-08 &  8.991079e-07 \\
116 &  0.000000e+00 & -0.000000e+00 &  1.009409e-14 &      0.0 &  6.496020e-07 &  3.976188e-06 & -5.477153e-08 & -7.348395e-07 \\
117 & -7.138287e-05 &  9.401514e-05 &  1.733693e+01 &      0.0 &  1.152383e-03 &  1.944178e-01 &  8.776674e-04 & -1.649640e-03 \\
118 & -1.156889e-04 &  3.392056e-04 &  3.131016e+01 &      0.0 &  1.137495e-03 &  1.805482e-01 &  8.068791e-04 & -1.974064e-03 \\
119 & -6.257918e-05 &  4.124090e-04 & -4.223956e+00 &      0.0 &  8.223259e-04 &  2.021767e-02 &  6.111788e-04 & -1.911138e-03 \\
120 &  2.634020e-04 &  1.524656e-03 &  4.592596e+00 &      0.0 & -6.608202e-04 &  1.079938e-02 &  3.573131e-03 & -1.854958e-03 \\
121 &  1.331130e-03 &  4.056590e-03 & -1.516058e+00 &      0.0 &  2.068892e-03 & -1.286384e-02 &  5.830813e-03 & -1.547803e-03 \\
122 &  2.899638e-03 &  8.369691e-03 &  1.437533e-01 &      0.0 & -7.255810e-04 &  5.682551e-03 &  3.552649e-03 & -5.595703e-03 \\
123 &  6.657351e-03 &  1.378415e-02 &  4.817704e-01 &      0.0 &  7.774867e-04 & -3.215047e-03 &  8.154367e-03 & -8.247516e-03 \\
124 &  1.286944e-02 &  1.637358e-02 &  2.922874e-02 &      0.0 & -1.565622e-03 &  7.909028e-04 &  1.105989e-02 & -4.800733e-03 \\
125 &  1.569124e-02 &  9.267577e-03 &  7.214196e-01 &      0.0 &  3.116873e-03 &  5.333401e-04 &  6.943305e-03 &  5.612332e-03 \\
126 &  1.311932e-02 & -1.400892e-02 & -3.545032e-01 &      0.0 & -7.771826e-04 & -3.592217e-04 &  1.006170e-02 &  1.336734e-02 \\
127 &  9.264380e-03 & -4.952581e-02 & -1.316895e-01 &      0.0 & -5.012668e-05 & -5.966737e-04 &  7.657054e-04 &  2.030192e-02 \\
128 &  7.338180e-03 & -8.039222e-02 &  6.413841e-01 &      0.0 & -3.331033e-04 &  3.646417e-05 &  3.709570e-03 &  1.574496e-02 \\
129 &  6.813228e-03 & -9.717648e-02 & -1.565044e-01 &      0.0 &  3.045173e-03 & -1.917153e-04 & -1.133095e-03 &  8.069645e-03 \\
130 &  9.757079e-03 & -8.696903e-02 & -3.213763e-01 &      0.0 &  2.904477e-04 & -8.690626e-04 & -1.328411e-03 &  8.507856e-03 \\
131 &  8.858076e-03 & -6.424213e-02 & -1.831677e-01 &      0.0 &  4.388131e-04 &  1.583222e-03 & -6.701082e-03 &  1.627124e-02 \\
132 &  7.963181e-03 & -3.948799e-02 &  5.342854e-01 &      0.0 &  4.227089e-04 & -1.902014e-03 & -1.103940e-02 &  8.113407e-03 \\
133 &  5.787917e-03 & -1.854834e-02 &  1.084560e+00 &      0.0 & -1.794323e-03 &  2.104809e-03 & -2.193081e-03 &  5.135453e-03 \\
134 &  3.387146e-03 & -7.747195e-03 & -4.060578e+00 &      0.0 &  1.076445e-03 & -1.861993e-03 & -2.184317e-03 & -1.011369e-03 \\
135 &  9.322443e-04 & -2.584241e-03 & -4.106842e+00 &      0.0 &  3.452901e-03 &  3.878325e-04 & -2.894550e-03 &  3.220095e-04 \\
136 &  6.996322e-05 & -3.698171e-04 &  8.589507e+00 &      0.0 &  5.654847e-03 & -1.552297e-03 & -6.340515e-04 &  1.452668e-03 \\
137 &  0.000000e+00 & -0.000000e+00 &  4.553096e-15 &      0.0 &  1.797633e-06 & -8.723434e-07 & -7.663152e-08 & -5.353559e-07 \\
138 &  0.000000e+00 & -0.000000e+00 &  1.689656e-14 &      0.0 & -4.067987e-06 &  1.063641e-07 &  5.426203e-08 & -3.382396e-08 \\
139 &  0.000000e+00 & -0.000000e+00 & -4.780969e-15 &      0.0 & -2.016470e-06 &  9.634008e-07 &  1.478461e-07 &  1.401136e-06 \\
140 &  0.000000e+00 & -0.000000e+00 &  8.647896e-16 &      0.0 &  3.907960e-06 &  3.475411e-06 &  3.801073e-07 &  2.888445e-06 \\
141 &  0.000000e+00 & -0.000000e+00 & -3.203118e-14 &      0.0 & -5.458799e-06 & -4.367545e-06 &  1.613562e-07 &  1.153519e-06 \\
142 &  0.000000e+00 & -0.000000e+00 & -1.564351e-15 &      0.0 & -3.378693e-06 &  1.072799e-06 &  1.429644e-07 &  1.117041e-06 \\
143 &  0.000000e+00 & -0.000000e+00 & -3.000313e-15 &      0.0 &  4.749959e-07 &  6.604598e-07 & -1.151740e-07 & -1.068662e-06 \\
144 &  0.000000e+00 & -0.000000e+00 & -2.154724e-15 &      0.0 &  2.223055e-07 & -2.548626e-06 & -5.044116e-09 &  3.607451e-07 \\
145 & -1.251045e-04 &  2.363775e-04 & -4.139221e+00 &      0.0 &  8.052741e-04 &  1.269303e-01 &  7.610704e-04 & -8.556050e-04 \\
146 & -1.210471e-04 &  6.101562e-04 &  3.853743e+01 &      0.0 & -4.115893e-04 & -4.759189e-03 &  9.486833e-04 & -1.502851e-03 \\
147 &  3.820411e-04 &  1.253653e-03 & -7.396709e+00 &      0.0 &  1.393960e-03 &  3.688546e-02 &  3.116627e-03 &  1.881333e-03 \\
148 &  1.734804e-03 &  3.378955e-03 & -3.748866e-01 &      0.0 & -2.019147e-03 & -6.562839e-03 &  4.603685e-03 &  5.304134e-03 \\
149 &  6.008440e-03 &  1.060866e-02 &  4.653185e-02 &      0.0 & -5.665504e-04 &  3.144285e-05 &  4.116455e-03 & -6.798833e-03 \\
150 &  1.365205e-02 &  2.181865e-02 & -8.547039e-01 &      0.0 & -1.299037e-04 &  1.288466e-03 &  4.252688e-03 & -1.549066e-02 \\
151 &  2.472075e-02 &  3.232028e-02 & -4.992507e-02 &      0.0 &  1.254177e-04 & -1.364909e-03 &  4.350867e-03 & -1.334554e-02 \\
152 &  3.595335e-02 &  3.184119e-02 & -3.392902e-01 &      0.0 &  1.609113e-03 & -6.058883e-03 & -2.445677e-03 & -2.529504e-02 \\
153 &  4.277292e-02 &  1.333671e-02 & -1.533186e-01 &      0.0 & -1.495348e-03 &  2.285457e-03 & -2.350012e-02 & -1.902786e-02 \\
154 &  4.743285e-02 & -2.678379e-02 &  7.969963e-01 &      0.0 &  2.233092e-03 &  2.515694e-04 & -3.623234e-02 &  4.120354e-03 \\
155 &  5.222111e-02 & -6.701449e-02 & -2.276980e-03 &      0.0 & -1.434879e-03 & -2.383377e-04 & -4.658780e-02 &  1.939362e-02 \\
156 &  5.514287e-02 & -9.991765e-02 & -1.711004e-01 &      0.0 &  9.048169e-04 & -8.125299e-04 & -5.265509e-02 &  1.971078e-02 \\
157 &  5.569360e-02 & -1.019238e-01 &  8.566710e-01 &      0.0 & -3.019834e-03 &  2.291138e-03 & -6.048824e-02 &  3.001086e-02 \\
158 &  5.290066e-02 & -8.799979e-02 &  4.216087e-01 &      0.0 & -6.284229e-05 & -2.143120e-03 & -4.981147e-02 &  3.510656e-02 \\
159 &  4.380542e-02 & -6.304551e-02 & -8.055944e-01 &      0.0 & -4.615493e-04 & -8.740335e-04 & -3.503442e-02 &  3.180764e-02 \\
160 &  3.177715e-02 & -4.135114e-02 &  3.185210e-01 &      0.0 & -2.771838e-04 & -8.376385e-04 & -2.365527e-02 &  7.431765e-04 \\
161 &  1.973962e-02 & -2.548976e-02 & -8.609382e-01 &      0.0 &  1.396615e-03 & -6.428923e-04 & -1.708848e-02 & -8.946855e-03 \\
162 &  1.008593e-02 & -1.208031e-02 &  2.542571e-01 &      0.0 &  1.078053e-04 &  1.175869e-03 & -9.180211e-03 & -6.310483e-04 \\
163 &  3.861963e-03 & -4.649758e-03 &  6.879613e+00 &      0.0 &  2.024584e-03 & -1.647458e-03 & -6.302767e-03 & -7.690566e-03 \\
164 &  2.897579e-04 & -7.528210e-04 & -2.460380e-01 &      0.0 & -1.346726e-02 &  3.940025e-03 & -3.027336e-03 & -3.702843e-05 \\
165 & -8.066816e-05 & -3.339117e-05 & -1.070437e+00 &      0.0 & -3.330325e-01 &  2.075505e-03 & -1.231915e-05 & -6.390129e-04 \\
166 & -3.007965e-05 & -1.245094e-05 & -2.870716e+00 &      0.0 & -3.330428e-01 &  2.074308e-03 & -4.844431e-06 & -2.403516e-04 \\
167 &  0.000000e+00 & -0.000000e+00 & -9.745627e-15 &      0.0 & -4.824262e-07 &  1.054770e-07 &  3.019986e-08 & -8.751268e-08 \\
168 &  0.000000e+00 & -0.000000e+00 &  1.672590e-16 &      0.0 &  6.410822e-07 &  2.492222e-07 &  1.206807e-07 &  2.533316e-07 \\
169 &  0.000000e+00 & -0.000000e+00 &  3.731657e-15 &      0.0 & -3.354939e-06 &  1.159788e-06 & -3.858551e-08 &  2.901102e-08 \\
170 & -5.627283e-05 & -1.383398e-04 & -1.382523e+00 &      0.0 &  2.893956e-04 & -1.027259e-03 &  8.846844e-05 & -6.086032e-05 \\
171 &  0.000000e+00 & -0.000000e+00 &  8.956407e-16 &      0.0 &  7.804176e-07 & -8.571932e-07 & -1.383092e-07 & -9.608059e-07 \\
172 &  6.522522e-05 & -2.401218e-06 &  6.450038e+01 &      0.0 &  9.282806e-04 & -7.218847e-03 & -2.132378e-06 &  5.352960e-04 \\
173 &  1.316882e-04 &  3.378439e-04 & -2.740025e+01 &      0.0 & -4.951055e-05 &  4.176402e-02 &  1.009699e-03 &  2.053151e-03 \\
174 &  2.291243e-05 &  1.185045e-03 &  4.268502e+00 &      0.0 & -7.532118e-04 & -3.798422e-02 &  1.851141e-03 &  2.789385e-03 \\
175 &  1.024071e-03 &  2.934610e-03 &  1.661000e+00 &      0.0 &  1.046341e-03 &  1.185261e-03 &  3.568294e-03 &  7.065037e-03 \\
176 &  5.954498e-03 &  1.026360e-02 &  7.696512e-01 &      0.0 &  1.158441e-03 &  3.378737e-03 &  3.275693e-03 & -3.051897e-03 \\
177 &  1.597677e-02 &  2.823196e-02 &  1.407607e+00 &      0.0 & -8.026006e-04 &  2.056054e-03 & -1.277617e-03 & -1.621333e-02 \\
178 &  2.954823e-02 &  4.785385e-02 & -6.961273e-01 &      0.0 & -1.952957e-03 &  2.062859e-03 & -1.283800e-02 & -2.233292e-02 \\
179 &  4.136372e-02 &  5.956443e-02 & -2.730601e-01 &      0.0 &  3.852578e-04 &  2.282116e-03 & -5.385363e-03 & -2.711003e-02 \\
180 &  4.497906e-02 &  5.729653e-02 &  7.892951e-01 &      0.0 & -3.811882e-04 &  1.073826e-03 & -7.619714e-03 & -8.605165e-03 \\
181 &  4.402591e-02 &  2.582407e-02 & -1.284786e-01 &      0.0 & -4.751830e-04 &  1.679792e-05 & -9.487605e-03 &  2.676928e-02 \\
182 &  3.998317e-02 & -1.535831e-02 & -4.243106e-01 &      0.0 & -7.009333e-04 &  1.693941e-03 &  2.659869e-03 &  2.265212e-02 \\
183 &  4.400987e-02 & -4.638143e-02 & -1.543868e-01 &      0.0 &  7.711938e-04 & -1.718202e-03 & -1.429009e-02 &  2.679679e-02 \\
184 &  5.277107e-02 & -5.871936e-02 &  3.142170e-01 &      0.0 & -8.181267e-04 &  5.408773e-05 & -4.929666e-02 &  1.399520e-02 \\
185 &  6.290146e-02 & -5.552334e-02 & -4.217586e-01 &      0.0 &  2.157449e-04 & -8.345176e-04 & -5.703233e-02 & -4.820356e-03 \\
186 &  7.117507e-02 & -5.207774e-02 & -4.689403e-01 &      0.0 &  1.857116e-04 &  1.128190e-03 & -3.850520e-02 & -1.056419e-02 \\
187 &  6.912736e-02 & -4.528825e-02 &  7.594024e-01 &      0.0 &  3.166423e-03 &  9.361180e-04 & -3.182817e-02 & -1.286625e-02 \\
188 &  5.536405e-02 & -3.595712e-02 & -5.267618e-01 &      0.0 &  1.335039e-04 & -1.096838e-03 & -2.698595e-02 & -2.959565e-03 \\
189 &  3.548228e-02 & -2.809118e-02 &  1.475160e+00 &      0.0 &  2.483543e-03 & -3.362994e-04 & -2.918652e-02 & -5.225863e-03 \\
190 &  1.911255e-02 & -1.681021e-02 &  3.955049e-01 &      0.0 &  3.583623e-04 & -3.646510e-04 & -1.239051e-02 & -1.143275e-02 \\
191 &  7.089838e-03 & -6.747208e-03 & -5.568780e+00 &      0.0 & -4.558504e-03 &  3.197279e-03 & -5.623584e-03 & -5.994671e-03 \\
192 &  9.676955e-04 & -1.084003e-03 & -2.448076e+00 &      0.0 &  3.304332e-03 & -2.308276e-03 & -3.398285e-03 &  1.246653e-04 \\
193 & -1.729580e-04 & -7.159293e-05 & -4.992550e-01 &      0.0 & -3.330285e-01 &  2.074625e-03 & -2.695544e-05 & -1.374278e-03 \\
194 & -1.647545e-04 & -6.819722e-05 & -5.241142e-01 &      0.0 & -3.330340e-01 &  2.074949e-03 & -2.544413e-05 & -1.306715e-03 \\
195 & -1.086969e-04 & -4.499319e-05 & -7.944120e-01 &      0.0 & -3.330342e-01 &  2.074270e-03 & -1.679694e-05 & -8.620743e-04 \\
196 &  0.000000e+00 & -0.000000e+00 & -3.673067e-15 &      0.0 &  1.540650e-06 & -8.877397e-08 & -4.217807e-08 & -1.380401e-07 \\
197 &  0.000000e+00 & -0.000000e+00 & -8.551692e-15 &      0.0 & -8.572121e-07 &  1.740215e-07 &  2.873241e-07 &  1.759813e-06 \\
198 &  0.000000e+00 & -0.000000e+00 &  1.104740e-14 &      0.0 & -8.933034e-07 &  1.023552e-07 & -1.424251e-07 & -4.835283e-07 \\
199 &  0.000000e+00 & -0.000000e+00 &  5.607833e-15 &      0.0 &  2.915184e-06 & -1.181459e-07 &  1.202234e-07 &  4.814121e-07 \\
200 &  1.633480e-04 &  1.098213e-04 &  7.030308e+01 &      0.0 & -9.470826e-05 & -2.830022e-03 &  6.845626e-04 &  1.729764e-03 \\
201 &  1.999829e-04 &  8.654848e-04 & -3.700147e+01 &      0.0 & -4.325034e-04 & -3.932451e-03 &  2.165798e-03 &  5.237199e-03 \\
202 &  2.062677e-04 &  2.838421e-03 &  1.774373e+00 &      0.0 & -1.816102e-04 & -7.430159e-03 &  2.919890e-03 &  7.664174e-03 \\
203 &  3.560550e-03 &  9.608647e-03 &  2.082715e+00 &      0.0 &  2.700015e-04 & -9.119778e-04 &  1.675796e-03 &  9.364233e-03 \\
204 &  1.367321e-02 &  2.788302e-02 & -1.303502e+00 &      0.0 &  1.374533e-04 & -1.002077e-03 &  9.675433e-03 &  4.676853e-03 \\
205 &  2.762204e-02 &  5.814558e-02 &  8.922497e-01 &      0.0 &  2.859023e-03 & -3.498501e-03 & -8.744836e-04 & -7.002060e-03 \\
206 &  3.864827e-02 &  8.256653e-02 &  8.548745e-01 &      0.0 & -1.049506e-03 & -3.451814e-04 &  7.151476e-04 &  4.189691e-03 \\
207 &  4.098186e-02 &  8.831628e-02 & -4.978383e-01 &      0.0 & -1.364629e-03 &  2.077215e-03 &  9.480736e-03 & -1.753773e-04 \\
208 &  3.480176e-02 &  6.551695e-02 &  1.627734e-01 &      0.0 &  1.847322e-03 & -2.991173e-03 &  1.314175e-02 &  9.252553e-03 \\
209 &  2.037823e-02 &  1.900852e-02 &  7.086563e-01 &      0.0 &  1.841113e-03 &  5.646355e-04 &  3.257714e-02 &  2.970197e-02 \\
210 &  1.382713e-02 & -1.780674e-02 & -5.569654e-01 &      0.0 & -1.555063e-03 &  1.461838e-03 &  2.852283e-02 &  1.269180e-02 \\
211 &  1.707932e-02 & -1.965567e-02 &  3.462825e-01 &      0.0 &  6.995866e-04 & -2.339385e-03 &  6.449585e-03 &  1.430305e-02 \\
212 &  2.773375e-02 & -1.499179e-03 & -1.921519e-01 &      0.0 & -6.616742e-04 &  9.388266e-04 & -9.768535e-03 &  6.516817e-03 \\
213 &  4.674119e-02 &  6.835312e-03 &  7.677999e-01 &      0.0 & -5.003101e-04 &  2.709551e-03 & -3.746074e-02 & -5.740148e-03 \\
214 &  6.547373e-02 &  4.576879e-04 &  8.884956e-02 &      0.0 &  9.038635e-04 & -1.682997e-03 & -4.067717e-02 & -2.106886e-02 \\
215 &  7.586307e-02 & -1.363796e-02 & -1.500124e-01 &      0.0 &  3.125358e-06 & -3.915097e-04 & -1.610877e-02 & -2.430380e-02 \\
216 &  7.234087e-02 & -2.209390e-02 &  4.887784e-01 &      0.0 & -2.584703e-03 &  2.830038e-03 & -8.252630e-03 & -1.848318e-02 \\
217 &  5.214218e-02 & -2.577105e-02 & -2.790504e-01 &      0.0 & -1.228526e-03 & -1.432320e-04 & -2.709019e-02 & -1.548920e-02 \\
218 &  2.927749e-02 & -1.850384e-02 &  8.388909e-02 &      0.0 & -5.112419e-03 & -1.873545e-04 & -2.373496e-02 & -1.930958e-02 \\
219 &  1.247424e-02 & -9.588672e-03 &  1.414567e+00 &      0.0 & -1.762360e-03 & -3.194369e-04 & -1.767330e-02 & -1.093608e-02 \\
220 &  2.515076e-03 & -2.292836e-03 &  4.765282e+00 &      0.0 & -1.252722e-03 &  1.675879e-03 & -8.684659e-03 & -1.989464e-04 \\
221 & -1.210022e-04 & -5.008675e-05 & -7.136244e-01 &      0.0 & -3.330351e-01 &  2.074161e-03 & -1.881111e-05 & -9.606572e-04 \\
222 & -1.497146e-04 & -6.197175e-05 & -5.767649e-01 &      0.0 & -3.330335e-01 &  2.074483e-03 & -2.314782e-05 & -1.187326e-03 \\
223 & -7.041373e-05 & -2.914653e-05 & -1.226325e+00 &      0.0 & -3.330366e-01 &  2.074667e-03 & -1.103370e-05 & -5.595438e-04 \\
224 &  0.000000e+00 & -0.000000e+00 &  6.685541e-15 &      0.0 & -1.394096e-06 &  1.229652e-07 & -3.360913e-08 & -4.819520e-07 \\
225 &  0.000000e+00 & -0.000000e+00 & -2.472210e-15 &      0.0 &  1.920370e-06 & -2.301995e-07 & -1.599821e-07 & -6.979348e-07 \\
226 &  0.000000e+00 & -0.000000e+00 & -2.156616e-15 &      0.0 &  3.833874e-07 &  6.895831e-09 &  1.382956e-07 &  5.878605e-07 \\
227 &  0.000000e+00 & -0.000000e+00 &  3.143989e-15 &      0.0 & -1.111779e-06 &  7.951871e-08 & -3.343974e-07 & -2.368731e-06 \\
228 &  3.110846e-05 &  3.627976e-04 &  4.651324e+01 &      0.0 & -3.296726e-05 & -3.122695e-03 &  1.018744e-03 &  2.332139e-03 \\
229 &  1.445993e-04 &  1.693850e-03 & -3.296546e+00 &      0.0 & -7.148435e-04 & -1.606920e-02 &  3.401760e-03 &  8.156739e-03 \\
230 &  1.581891e-03 &  7.520171e-03 & -1.951794e+00 &      0.0 & -4.059942e-04 &  7.058869e-03 &  4.432116e-03 &  1.705499e-02 \\
231 &  7.911462e-03 &  2.289063e-02 &  1.526347e-01 &      0.0 & -7.283118e-04 & -3.962751e-03 &  9.450446e-03 &  2.366222e-02 \\
232 &  2.375448e-02 &  5.589779e-02 &  6.637850e-01 &      0.0 &  2.939372e-04 &  9.910753e-04 &  1.609853e-02 &  7.476154e-03 \\
233 &  3.624391e-02 &  8.943530e-02 & -1.547533e+00 &      0.0 & -2.320082e-03 & -3.709033e-04 &  2.186358e-02 &  6.035660e-03 \\
234 &  4.280926e-02 &  1.062182e-01 &  6.914710e-01 &      0.0 & -1.433816e-06 & -1.389634e-03 &  1.255062e-02 &  2.359967e-03 \\
235 &  3.463758e-02 &  8.197380e-02 &  2.454755e-01 &      0.0 & -1.694896e-03 &  2.292871e-04 &  1.504791e-02 & -1.793422e-03 \\
236 &  1.841313e-02 &  2.013261e-02 & -3.753218e-02 &      0.0 & -4.466901e-03 & -1.259755e-04 &  2.887238e-02 & -1.289033e-03 \\
237 &  6.693173e-03 & -3.963559e-02 &  4.189914e-01 &      0.0 &  4.022034e-04 &  8.353032e-06 &  2.702209e-02 & -1.095340e-03 \\
238 &  6.309805e-03 & -5.636792e-02 &  2.740161e-01 &      0.0 & -4.097260e-04 &  4.131823e-04 & -2.482152e-03 &  2.390510e-02 \\
239 &  1.298399e-02 & -2.717078e-02 & -2.332785e-01 &      0.0 & -2.231179e-04 &  2.846380e-03 & -3.262538e-03 &  3.266934e-02 \\
240 &  1.834058e-02 &  1.331563e-02 &  6.094210e-01 &      0.0 &  4.642507e-04 & -3.076323e-03 & -2.252857e-02 &  3.081394e-02 \\
241 &  3.058347e-02 &  4.834009e-02 & -7.435569e-01 &      0.0 &  5.151253e-04 & -2.074180e-03 & -3.561315e-02 &  1.543047e-02 \\
242 &  4.952563e-02 &  4.569427e-02 &  9.055784e-01 &      0.0 & -1.314564e-03 & -6.543904e-04 & -5.347407e-02 & -1.318841e-02 \\
243 &  6.894904e-02 &  2.004893e-02 &  4.750827e-01 &      0.0 &  7.682583e-04 &  6.829166e-04 & -2.008652e-02 & -8.661006e-03 \\
244 &  8.144461e-02 & -1.943053e-03 &  2.487307e-01 &      0.0 & -5.329954e-04 & -2.867216e-03 & -3.764593e-03 & -2.107715e-02 \\
245 &  7.162280e-02 & -1.473839e-02 &  1.260012e-01 &      0.0 &  9.356454e-04 &  1.118364e-04 & -9.654238e-03 & -8.866536e-03 \\
246 &  4.548716e-02 & -1.646191e-02 &  3.143873e-01 &      0.0 &  6.917212e-04 &  1.340380e-03 & -2.255206e-02 & -2.319903e-02 \\
247 &  1.903851e-02 & -1.050544e-02 &  1.125086e-01 &      0.0 &  2.963209e-03 & -2.496292e-03 & -2.216547e-02 & -1.223999e-02 \\
248 &  4.887873e-03 & -3.474226e-03 & -3.100314e+00 &      0.0 & -1.240918e-04 & -3.019563e-03 & -1.408287e-02 & -6.591140e-03 \\
249 &  0.000000e+00 & -0.000000e+00 & -1.609369e-15 &      0.0 &  2.058169e-07 & -4.048667e-08 & -3.036211e-08 & -7.021799e-07 \\
250 & -2.255974e-05 & -9.338208e-06 & -3.827622e+00 &      0.0 & -3.330354e-01 &  2.074517e-03 & -3.247295e-06 & -1.771459e-04 \\
251 &  0.000000e+00 & -0.000000e+00 & -1.396540e-15 &      0.0 &  5.572289e-08 & -1.196328e-08 & -1.175355e-07 & -1.111087e-06 \\
252 &  0.000000e+00 & -0.000000e+00 & -9.141782e-15 &      0.0 &  6.218983e-08 & -7.617817e-09 &  1.384893e-07 &  1.389608e-06 \\
253 &  0.000000e+00 & -0.000000e+00 & -3.298983e-15 &      0.0 &  2.689455e-08 & -4.044146e-09 &  8.819036e-08 &  4.627394e-07 \\
254 &  0.000000e+00 & -0.000000e+00 &  9.402318e-15 &      0.0 &  7.905541e-08 & -2.158799e-08 &  3.071830e-07 &  2.103967e-06 \\
255 & -1.806227e-06 &  1.250096e-07 &  7.813513e+02 &      0.0 &  3.448362e-04 & -1.430228e-03 &  2.430244e-06 & -6.948722e-06 \\
256 & -4.261459e-05 &  4.237074e-04 & -2.636476e+01 &      0.0 &  5.447074e-05 & -3.223159e-03 &  1.220640e-03 &  2.218438e-03 \\
257 &  5.310753e-04 &  3.541684e-03 &  1.757116e+00 &      0.0 &  1.417715e-06 & -1.832521e-03 &  4.717903e-03 &  1.153290e-02 \\
258 &  5.954837e-03 &  1.749092e-02 & -1.533683e-01 &      0.0 &  1.088029e-03 & -2.196035e-04 &  1.029214e-02 &  2.487424e-02 \\
259 &  1.969940e-02 &  4.716678e-02 &  3.177676e-01 &      0.0 & -8.265622e-04 &  4.213155e-04 &  2.187280e-02 &  2.770418e-02 \\
260 &  3.445040e-02 &  8.439322e-02 &  1.501994e+00 &      0.0 &  2.682532e-03 &  8.597559e-04 &  1.668391e-02 &  1.252566e-02 \\
261 &  4.431605e-02 &  1.116138e-01 & -2.124805e-01 &      0.0 &  7.913464e-04 &  3.438147e-04 &  1.067799e-02 & -1.989672e-03 \\
262 &  4.190729e-02 &  9.422576e-02 & -5.706819e-01 &      0.0 &  1.079719e-04 &  7.329797e-04 &  1.606445e-02 & -1.463887e-02 \\
263 &  2.555445e-02 &  1.930648e-02 &  2.211315e-01 &      0.0 &  4.086408e-03 & -1.560559e-04 &  1.316399e-02 & -3.690790e-02 \\
264 &  9.662933e-03 & -6.476892e-02 & -4.954088e-01 &      0.0 & -5.979764e-05 & -8.371228e-04 &  9.503692e-03 & -3.516498e-02 \\
265 &  4.807615e-03 & -1.050871e-01 &  2.784084e-01 &      0.0 &  2.225947e-03 &  5.285093e-04 & -1.658397e-02 & -6.435228e-03 \\
266 &  9.841996e-03 & -8.677611e-02 & -6.151877e-02 &      0.0 &  8.223395e-04 & -3.641181e-03 & -3.714136e-02 &  1.953962e-02 \\
267 &  1.527816e-02 & -3.561875e-02 & -6.365383e-01 &      0.0 & -5.824441e-04 &  9.451511e-04 & -2.875339e-02 &  4.086157e-02 \\
268 &  1.611879e-02 &  1.910152e-02 &  4.048255e-01 &      0.0 & -1.161708e-03 &  2.148744e-03 & -3.988741e-02 &  3.942490e-02 \\
269 &  1.678727e-02 &  5.992319e-02 &  2.367618e-01 &      0.0 &  1.410073e-03 &  7.736559e-04 & -3.467397e-02 &  3.626762e-02 \\
270 &  2.486721e-02 &  6.122332e-02 &  2.580516e-01 &      0.0 &  2.862544e-03 &  5.007300e-04 & -5.136042e-02 &  2.360160e-03 \\
271 &  5.465794e-02 &  3.667302e-02 & -1.506278e-01 &      0.0 & -8.683327e-04 & -9.223246e-04 & -4.416442e-02 & -1.771138e-02 \\
272 &  8.324814e-02 &  1.037149e-02 & -7.924725e-01 &      0.0 & -5.243819e-04 & -4.244095e-04 & -1.528236e-02 & -1.666141e-02 \\
273 &  8.541441e-02 & -4.104096e-03 &  8.461119e-01 &      0.0 & -1.699577e-03 &  2.692053e-03 & -1.421714e-02 & -6.993588e-03 \\
274 &  6.426636e-02 & -8.927391e-03 & -4.458300e-01 &      0.0 &  1.477322e-03 &  3.500031e-04 & -2.317670e-02 & -5.542409e-03 \\
275 &  2.896006e-02 & -7.891787e-03 &  1.287057e-01 &      0.0 &  1.478500e-03 &  3.314983e-03 & -2.041528e-02 & -8.654518e-03 \\
276 &  6.790206e-03 & -4.099027e-03 &  2.687920e+00 &      0.0 &  3.975620e-03 &  1.132004e-03 & -1.505695e-02 & -8.115629e-03 \\
277 &  0.000000e+00 & -0.000000e+00 & -1.464953e-14 &      0.0 & -5.682899e-09 &  2.578314e-09 &  1.860889e-08 & -4.011687e-07 \\
278 &  0.000000e+00 & -0.000000e+00 & -2.618281e-15 &      0.0 & -9.487827e-09 &  4.644473e-09 &  3.364490e-07 &  1.986740e-06 \\
279 &  0.000000e+00 & -0.000000e+00 & -1.004314e-14 &      0.0 & -9.137552e-09 &  5.240198e-09 &  2.753817e-07 &  2.374540e-06 \\
280 &  0.000000e+00 & -0.000000e+00 & -2.143416e-15 &      0.0 &  1.499655e-09 &  2.258718e-10 &  5.829702e-08 &  6.542419e-07 \\
281 &  0.000000e+00 & -0.000000e+00 &  8.872835e-15 &      0.0 & -3.892518e-09 &  2.602129e-09 & -1.558828e-07 & -1.386261e-06 \\
282 &  0.000000e+00 & -0.000000e+00 & -1.110391e-15 &      0.0 &  4.977411e-09 & -3.290702e-09 & -7.049542e-08 & -7.075705e-07 \\
283 & -9.934250e-06 &  6.875529e-07 &  1.420639e+02 &      0.0 &  3.447432e-04 & -1.430285e-03 &  1.292328e-05 & -3.792843e-05 \\
284 & -2.608480e-04 &  8.097026e-04 & -1.116623e+01 &      0.0 &  3.605222e-04 & -2.514887e-03 &  1.677617e-03 &  2.225724e-03 \\
285 &  2.295603e-03 &  9.214675e-03 &  1.268334e+00 &      0.0 &  9.234138e-05 &  1.716369e-03 &  1.831618e-03 &  1.204477e-02 \\
286 &  1.374171e-02 &  3.164817e-02 & -1.806920e+00 &      0.0 &  4.464097e-05 &  8.162186e-04 &  1.480608e-02 &  2.816236e-02 \\
287 &  3.201368e-02 &  6.750542e-02 & -1.426745e+00 &      0.0 & -5.008596e-04 &  8.336045e-04 &  1.868718e-02 &  1.922475e-02 \\
288 &  4.773905e-02 &  1.035205e-01 &  4.663318e-01 &      0.0 &  1.103921e-03 & -2.473493e-03 &  1.553794e-02 &  1.974972e-02 \\
289 &  5.094931e-02 &  1.007151e-01 &  1.446563e+00 &      0.0 &  2.152268e-03 &  8.008409e-04 &  1.133655e-02 & -1.200896e-02 \\
290 &  3.568082e-02 &  3.623159e-02 &  4.783096e-01 &      0.0 & -3.235697e-03 &  9.319354e-04 &  1.461538e-02 & -3.470148e-02 \\
291 &  1.314764e-02 & -6.436144e-02 & -6.210909e-02 &      0.0 &  1.108672e-03 &  6.897462e-06 &  4.910044e-03 & -4.763591e-02 \\
292 &  3.803192e-03 & -1.284903e-01 &  5.362163e-01 &      0.0 & -1.297315e-03 & -4.867592e-04 & -1.779384e-02 & -2.357911e-02 \\
293 &  5.411465e-03 & -1.244492e-01 &  2.053454e-01 &      0.0 & -2.145442e-03 &  3.530008e-03 & -4.432669e-02 &  1.241094e-02 \\
294 &  1.214839e-02 & -7.476117e-02 &  5.199248e-01 &      0.0 &  1.946677e-03 & -1.516760e-03 & -4.539063e-02 &  2.088157e-02 \\
295 &  1.152507e-02 & -1.804703e-02 &  7.922595e-01 &      0.0 & -2.299484e-03 & -2.862993e-04 & -3.646072e-02 &  2.424292e-02 \\
296 &  3.177040e-03 &  3.126975e-02 &  4.922385e-02 &      0.0 &  1.339901e-03 &  7.033501e-04 & -4.582911e-02 &  3.047056e-02 \\
297 & -7.432576e-03 &  6.221649e-02 &  4.715073e-01 &      0.0 &  5.109363e-04 & -2.116267e-03 & -5.152774e-02 &  2.369710e-02 \\
298 & -2.387503e-03 &  6.538689e-02 &  1.830127e-01 &      0.0 & -5.269717e-03 & -1.540039e-04 & -5.504454e-02 & -6.086944e-03 \\
299 &  3.158190e-02 &  4.242299e-02 &  4.890540e-01 &      0.0 & -2.725374e-04 &  1.374430e-04 & -5.161469e-02 & -1.266146e-02 \\
300 &  7.561203e-02 &  1.212144e-02 &  2.319041e-01 &      0.0 &  2.191091e-04 &  8.751421e-04 & -3.017931e-02 & -3.825355e-03 \\
301 &  9.283560e-02 & -8.825593e-05 & -8.058009e-02 &      0.0 &  5.441554e-04 & -2.775922e-03 & -2.523717e-02 & -2.411832e-02 \\
302 &  7.764164e-02 & -1.871664e-03 & -2.737847e-03 &      0.0 &  1.686300e-03 & -2.509097e-03 & -2.912996e-02 & -8.703606e-03 \\
303 &  4.160391e-02 & -1.088524e-03 &  3.917519e-01 &      0.0 & -1.445355e-03 & -4.031709e-03 & -2.214887e-02 & -8.984512e-03 \\
304 &  9.140620e-03 & -1.918530e-03 &  6.057148e-01 &      0.0 & -1.257436e-03 & -1.559388e-03 & -1.428100e-02 & -1.105265e-02 \\
305 &  3.283541e-06 &  3.082222e-06 & -3.132105e+01 &      0.0 &  4.653427e-04 & -6.377570e-03 & -1.610262e-05 & -1.350392e-05 \\
306 &  0.000000e+00 & -0.000000e+00 &  2.782522e-15 &      0.0 &  3.806314e-11 & -2.531042e-11 & -8.980358e-09 & -1.076828e-07 \\
307 &  0.000000e+00 & -0.000000e+00 & -2.872911e-15 &      0.0 &  3.101849e-10 & -4.222915e-10 &  2.569360e-08 &  2.701828e-07 \\
308 &  0.000000e+00 & -0.000000e+00 &  9.647483e-15 &      0.0 &  4.194903e-10 & -5.712142e-10 &  8.712406e-08 &  1.334720e-06 \\
309 &  0.000000e+00 & -0.000000e+00 & -4.176625e-15 &      0.0 &  2.893499e-10 & -3.974474e-10 &  5.062358e-08 &  6.306982e-07 \\
310 &  0.000000e+00 & -0.000000e+00 & -7.620231e-16 &      0.0 &  4.495405e-11 & -6.400969e-11 & -1.081168e-07 & -7.019464e-07 \\
311 &  0.000000e+00 & -0.000000e+00 & -3.557255e-15 &      0.0 &  1.427996e-10 & -2.071250e-10 &  3.173752e-08 &  3.115649e-07 \\
312 &  9.021368e-05 &  1.655042e-03 &  1.154898e+01 &      0.0 &  4.667946e-05 &  1.049365e-03 &  2.084572e-03 &  3.761534e-03 \\
313 &  7.119709e-03 &  1.688933e-02 &  4.360545e-01 &      0.0 & -1.651997e-03 & -1.818392e-03 &  4.573221e-03 &  2.115645e-02 \\
314 &  2.533149e-02 &  4.840602e-02 &  1.426945e+00 &      0.0 &  7.826887e-04 &  7.038427e-04 &  1.053919e-02 &  2.710670e-02 \\
315 &  4.699943e-02 &  8.409440e-02 & -6.447275e-01 &      0.0 &  6.804135e-04 &  3.612798e-03 &  1.105932e-02 &  1.602067e-02 \\
316 &  5.935011e-02 &  1.025058e-01 & -7.941569e-01 &      0.0 &  3.735464e-05 & -3.380494e-04 &  1.863937e-02 &  2.316091e-02 \\
317 &  4.913115e-02 &  6.148478e-02 & -6.293191e-01 &      0.0 & -6.900237e-04 &  1.006212e-03 &  1.947405e-02 & -2.631640e-02 \\
318 &  2.129208e-02 & -3.832987e-02 & -4.180951e-01 &      0.0 &  6.747025e-04 & -1.536749e-03 &  2.448041e-02 & -4.155254e-02 \\
319 &  1.928456e-03 & -1.250854e-01 &  8.258212e-02 &      0.0 & -9.311208e-04 &  1.362280e-03 & -1.182508e-02 & -4.206534e-02 \\
320 & -6.284024e-03 & -1.414838e-01 & -1.597403e-01 &      0.0 &  3.002781e-03 & -2.771766e-03 & -2.130980e-02 &  1.413319e-04 \\
321 & -2.015483e-03 & -9.860570e-02 & -1.967887e-01 &      0.0 &  3.431272e-04 &  3.071664e-03 & -3.895143e-02 &  2.528697e-02 \\
322 &  5.192638e-04 & -3.773682e-02 & -4.278198e-01 &      0.0 & -6.990366e-04 & -1.940794e-04 & -2.885424e-02 &  4.182879e-02 \\
323 & -4.972069e-03 &  9.027890e-03 & -1.579853e-01 &      0.0 &  2.350723e-03 &  1.259484e-03 & -2.863432e-02 &  3.047121e-02 \\
324 & -2.224169e-02 &  4.372037e-02 & -4.259094e-02 &      0.0 & -9.541546e-04 & -3.127708e-03 & -1.097671e-02 &  1.419208e-02 \\
325 & -4.054789e-02 &  6.720367e-02 & -9.635130e-02 &      0.0 &  5.963654e-04 &  3.330359e-03 & -6.961478e-03 & -3.158612e-02 \\
326 & -3.135463e-02 &  5.834091e-02 & -3.413832e-01 &      0.0 &  1.991482e-04 &  6.659203e-04 & -2.367001e-02 & -5.944298e-02 \\
327 &  8.852872e-03 &  3.115750e-02 & -2.906799e-01 &      0.0 &  3.811205e-03 & -1.185686e-03 & -4.425399e-02 & -6.192813e-02 \\
328 &  6.436927e-02 &  9.921304e-04 &  4.544756e-01 &      0.0 & -8.429106e-04 &  2.964328e-03 & -2.999248e-02 & -2.792771e-02 \\
329 &  9.568454e-02 & -9.292559e-04 & -3.093404e-01 &      0.0 &  2.008078e-03 &  9.461651e-04 & -2.951988e-02 & -3.847938e-02 \\
330 &  8.855565e-02 &  5.073071e-03 &  3.389231e-01 &      0.0 & -6.359969e-04 &  1.378034e-03 & -2.795744e-02 & -1.262792e-02 \\
331 &  5.220304e-02 &  1.024418e-02 & -3.015822e-01 &      0.0 & -1.647666e-03 &  1.309493e-04 & -1.746175e-02 & -5.967582e-05 \\
332 &  1.265877e-02 &  3.293763e-03 & -3.590853e-01 &      0.0 & -4.042292e-04 &  4.087180e-03 & -1.194412e-02 & -4.748653e-03 \\
333 &  8.426079e-05 & -9.065431e-05 &  2.252994e+00 &      0.0 & -1.179499e-04 & -3.339266e-02 & -4.924084e-04 & -2.334239e-04 \\
334 &  8.892566e-05 & -2.353776e-04 & -1.469159e+00 &      0.0 & -4.869199e-05 &  4.284496e-03 & -1.782874e-03 & -9.991033e-04 \\
335 &  0.000000e+00 & -0.000000e+00 & -7.742553e-15 &      0.0 & -2.876848e-13 &  8.325562e-13 &  5.443779e-10 &  4.211296e-10 \\
336 &  0.000000e+00 & -0.000000e+00 & -9.001077e-15 &      0.0 &  2.014514e-12 & -6.634915e-12 & -4.658962e-08 & -1.977431e-07 \\
337 &  0.000000e+00 & -0.000000e+00 & -1.154470e-14 &      0.0 &  7.976610e-13 & -2.896350e-12 &  5.802169e-08 &  3.277747e-07 \\
338 &  0.000000e+00 & -0.000000e+00 & -7.028881e-15 &      0.0 & -3.606350e-13 &  5.838663e-13 & -1.086459e-08 &  3.019380e-07 \\
339 &  3.394576e-05 &  5.198204e-04 & -1.412701e+00 &      0.0 &  1.001373e-03 & -1.190282e-03 &  3.383961e-04 &  7.383895e-04 \\
340 &  1.054173e-03 &  3.408998e-03 & -3.416903e+00 &      0.0 &  9.695555e-04 & -7.055715e-04 &  3.537240e-03 &  5.121125e-03 \\
341 &  1.443340e-02 &  2.491737e-02 & -4.667227e-01 &      0.0 &  6.920073e-04 &  1.904665e-03 &  5.018009e-03 &  1.834264e-02 \\
342 &  3.981670e-02 &  6.056805e-02 &  4.944544e-02 &      0.0 &  3.211769e-05 & -1.232939e-03 &  6.562181e-03 &  2.553382e-02 \\
343 &  6.405361e-02 &  8.806524e-02 &  1.356666e+00 &      0.0 & -3.005410e-03 &  1.025157e-03 &  1.541366e-02 &  2.804439e-02 \\
344 &  6.787671e-02 &  8.123593e-02 & -3.630609e-01 &      0.0 & -1.183961e-05 & -1.477526e-03 &  2.820753e-02 &  2.353394e-02 \\
345 &  4.034511e-02 &  7.867112e-03 & -1.408595e-01 &      0.0 &  1.193566e-03 &  2.138199e-03 &  3.655751e-02 & -5.974601e-03 \\
346 &  4.948802e-03 & -8.995442e-02 &  4.984844e-01 &      0.0 &  1.409046e-04 &  4.278224e-03 &  1.304704e-02 & -5.928754e-02 \\
347 & -1.628813e-02 & -1.371429e-01 & -3.527129e-01 &      0.0 & -1.320023e-04 &  1.002292e-03 & -1.098811e-02 & -4.712232e-02 \\
348 & -2.295727e-02 & -1.116326e-01 &  3.084366e-01 &      0.0 & -3.117264e-03 & -2.318138e-04 & -1.797384e-02 & -5.008427e-03 \\
349 & -1.737069e-02 & -5.099847e-02 &  6.157894e-02 &      0.0 &  2.122857e-03 &  1.600711e-05 & -3.367711e-02 & -8.909896e-03 \\
350 & -1.723184e-02 & -3.762387e-03 & -2.724880e-01 &      0.0 & -1.851415e-03 & -1.800424e-03 & -4.695906e-03 & -5.602169e-03 \\
351 & -3.186261e-02 &  2.845455e-02 &  3.444314e-02 &      0.0 & -1.357090e-03 & -9.519552e-04 &  2.794967e-02 & -4.606183e-02 \\
352 & -5.665690e-02 &  4.994359e-02 & -3.460454e-01 &      0.0 &  1.738200e-03 &  8.967334e-04 &  8.569073e-02 & -9.890709e-02 \\
353 & -7.181438e-02 &  5.847855e-02 &  4.100470e-02 &      0.0 & -8.641849e-05 & -2.999043e-03 &  8.244558e-02 & -1.259374e-01 \\
354 & -5.496553e-02 &  3.177714e-02 &  3.883305e-01 &      0.0 &  4.699491e-04 & -1.416149e-03 &  4.241553e-02 & -1.254821e-01 \\
355 & -9.629146e-03 & -3.884603e-03 &  9.271420e-02 &      0.0 & -2.536080e-03 &  7.239886e-04 & -1.613842e-02 & -9.356012e-02 \\
356 &  5.530467e-02 & -2.645574e-02 &  1.808190e-01 &      0.0 & -8.104289e-04 & -2.410777e-03 & -1.149981e-02 & -4.826740e-02 \\
357 &  9.656842e-02 & -1.237361e-02 & -4.350438e-01 &      0.0 & -2.537642e-03 & -1.466548e-04 & -1.489514e-02 & -2.501855e-02 \\
358 &  9.407973e-02 &  9.507565e-03 &  3.171488e-01 &      0.0 &  2.808311e-03 & -2.010869e-03 & -2.039310e-02 & -3.331819e-02 \\
359 &  5.905179e-02 &  1.978161e-02 & -7.970372e-02 &      0.0 &  3.513560e-04 & -1.082444e-03 & -1.316006e-02 & -8.247832e-03 \\
360 &  1.637587e-02 &  9.386043e-03 &  7.209535e-02 &      0.0 &  7.511296e-04 & -1.680709e-03 & -9.219046e-03 & -1.195898e-02 \\
361 &  2.523526e-04 &  5.284372e-04 &  1.525990e+00 &      0.0 & -1.248632e-03 & -2.738061e-05 &  9.944039e-04 & -1.009307e-03 \\
362 &  7.089465e-05 & -1.876513e-04 & -1.842818e+00 &      0.0 & -4.796517e-05 &  4.311236e-03 & -1.421395e-03 & -7.954678e-04 \\
363 &  0.000000e+00 & -0.000000e+00 & -2.582864e-15 &      0.0 & -7.018518e-14 &  1.181431e-13 & -1.158946e-07 & -3.713539e-07 \\
364 &  0.000000e+00 & -0.000000e+00 & -2.676773e-15 &      0.0 &  1.585711e-14 & -1.882938e-13 &  1.265740e-07 &  7.998938e-07 \\
365 &  0.000000e+00 & -0.000000e+00 & -6.800958e-15 &      0.0 & -8.673184e-15 & -4.263256e-14 & -3.255379e-07 & -1.673108e-06 \\
366 &  1.679915e-06 & -5.367619e-05 &  8.592923e+00 &      0.0 &  2.008466e-05 &  8.018260e-05 & -3.455380e-04 &  7.355715e-06 \\
367 &  5.087578e-05 &  8.739211e-04 & -1.342396e+01 &      0.0 &  1.086917e-03 & -1.511564e-03 &  4.139844e-04 &  1.494950e-03 \\
368 &  2.941337e-03 &  4.445599e-03 & -1.391095e-01 &      0.0 & -1.988949e-03 &  1.544927e-03 &  4.956049e-03 &  7.365338e-03 \\
369 &  2.410312e-02 &  3.107290e-02 & -3.824478e-01 &      0.0 & -1.328090e-03 & -2.554024e-03 & -3.137061e-03 &  8.556737e-03 \\
370 &  5.698829e-02 &  6.230891e-02 & -6.818253e-01 &      0.0 &  1.524522e-03 & -5.910147e-04 & -8.899617e-03 &  1.849910e-02 \\
371 &  7.914471e-02 &  7.534518e-02 & -1.486259e+00 &      0.0 & -4.868814e-04 &  1.084716e-03 &  1.828242e-02 &  3.033093e-02 \\
372 &  6.720995e-02 &  4.703326e-02 &  2.373564e-01 &      0.0 & -1.267435e-03 &  2.390455e-03 &  3.330538e-02 &  6.352604e-02 \\
373 &  2.516440e-02 & -3.249909e-02 & -4.673581e-01 &      0.0 &  5.933461e-04 & -2.102458e-03 &  4.269175e-02 &  1.739066e-02 \\
374 & -1.837830e-02 & -1.066063e-01 & -4.017909e-02 &      0.0 &  7.594822e-04 & -7.519429e-04 &  1.208409e-02 & -6.073126e-02 \\
375 & -4.216498e-02 & -1.138195e-01 & -1.566409e-01 &      0.0 & -1.085200e-03 &  1.785359e-03 &  1.562601e-03 & -7.780001e-02 \\
376 & -4.290858e-02 & -6.557590e-02 & -3.897630e-01 &      0.0 &  5.186741e-04 & -1.368246e-03 &  5.840365e-03 & -6.079605e-02 \\
377 & -4.096203e-02 & -8.989036e-03 &  2.561047e-01 &      0.0 & -1.138959e-03 &  2.199795e-03 &  2.611667e-02 & -8.606272e-02 \\
378 & -4.983524e-02 &  1.870393e-02 & -8.719822e-01 &      0.0 & -1.021112e-03 &  3.114696e-03 &  8.635224e-02 & -1.243022e-01 \\
379 & -6.963342e-02 &  3.178839e-02 & -5.992048e-02 &      0.0 &  1.497677e-03 &  1.272745e-03 &  1.531449e-01 & -1.647136e-01 \\
380 & -8.858358e-02 &  4.065950e-02 & -9.857839e-02 &      0.0 & -5.188105e-06 &  1.079988e-03 &  1.953083e-01 & -1.576587e-01 \\
381 & -9.166698e-02 &  3.653284e-02 & -4.217727e-01 &      0.0 & -1.364595e-03 &  8.336072e-04 &  1.350794e-01 & -1.240159e-01 \\
382 & -6.479911e-02 & -1.440547e-03 &  8.218100e-02 &      0.0 &  8.657431e-04 &  1.759997e-03 &  7.434467e-02 & -1.016551e-01 \\
383 & -1.418123e-02 & -4.303753e-02 & -9.729801e-02 &      0.0 &  2.843114e-04 &  2.938638e-04 &  1.816729e-02 & -7.255460e-02 \\
384 &  5.123211e-02 & -5.927086e-02 & -2.015731e-01 &      0.0 &  7.596206e-04 &  2.736790e-04 & -5.067274e-04 & -3.739398e-02 \\
385 &  9.362460e-02 & -2.870325e-02 &  3.405749e-01 &      0.0 &  1.668972e-03 & -1.014649e-03 &  6.570716e-03 & -2.501793e-02 \\
386 &  9.408389e-02 &  9.074647e-03 & -3.266230e-01 &      0.0 & -3.732744e-03 &  2.894457e-03 & -1.058952e-02 & -2.646767e-02 \\
387 &  6.190191e-02 &  2.736712e-02 & -8.105770e-01 &      0.0 &  6.429803e-04 &  1.186565e-03 & -1.394302e-02 & -2.232597e-02 \\
388 &  1.885906e-02 &  1.522800e-02 & -5.803022e-01 &      0.0 &  1.226231e-03 & -2.317789e-03 & -9.640590e-03 & -1.135256e-02 \\
389 &  1.770216e-04 &  1.739070e-03 & -2.079563e+00 &      0.0 &  4.110445e-05 & -3.691252e-02 &  3.903032e-03 & -4.649872e-03 \\
390 & -1.675360e-05 &  6.985603e-07 & -2.196667e-01 &      0.0 &  4.690168e-04 &  1.918514e-03 & -8.295975e-05 & -1.663305e-04 \\
391 &  0.000000e+00 & -0.000000e+00 &  7.353148e-16 &      0.0 & -5.082523e-15 &  3.530509e-14 &  2.868597e-08 &  7.946701e-07 \\
392 &  0.000000e+00 & -0.000000e+00 & -5.972661e-16 &      0.0 & -8.253131e-14 & -1.865175e-14 &  2.318697e-07 &  1.597746e-06 \\
393 &  0.000000e+00 & -0.000000e+00 & -2.791911e-16 &      0.0 &  4.786471e-14 &  5.573320e-14 &  1.629144e-07 &  1.923816e-06 \\
394 &  0.000000e+00 & -0.000000e+00 &  4.686398e-16 &      0.0 &  1.547330e-14 & -5.773160e-15 & -2.234328e-07 & -1.029314e-06 \\
395 &  7.047424e-05 &  9.620908e-04 &  2.713327e+00 &      0.0 &  1.239601e-03 & -2.252831e-03 &  4.665159e-04 &  1.806506e-03 \\
396 &  6.155614e-03 &  5.076915e-03 & -1.917500e+00 &      0.0 &  2.363839e-03 & -4.084481e-03 &  4.065849e-03 &  1.470027e-02 \\
397 &  3.754922e-02 &  3.300557e-02 &  3.776668e-01 &      0.0 &  2.559410e-04 &  4.370749e-04 & -1.847815e-02 &  1.408395e-02 \\
398 &  7.483877e-02 &  5.442253e-02 &  8.878428e-01 &      0.0 & -3.724503e-04 & -2.340446e-03 & -1.747430e-02 &  7.071857e-03 \\
399 &  9.124810e-02 &  5.169286e-02 &  8.288885e-01 &      0.0 &  9.757185e-04 & -2.854992e-03 & -2.306675e-03 &  3.356555e-02 \\
400 &  6.649142e-02 &  1.032219e-02 & -1.766713e-03 &      0.0 &  8.716695e-04 &  5.197888e-04 &  3.735373e-02 &  8.818929e-02 \\
401 &  7.966177e-03 & -5.940279e-02 &  6.254691e-01 &      0.0 &  1.141338e-03 & -3.845328e-03 &  4.216896e-02 &  4.781442e-02 \\
402 & -4.388661e-02 & -9.285210e-02 &  2.537269e-01 &      0.0 &  1.457446e-03 & -3.155484e-03 &  3.032908e-02 & -1.882547e-02 \\
403 & -6.672558e-02 & -6.563931e-02 &  6.544642e-01 &      0.0 &  9.208409e-04 & -1.348386e-03 &  3.192020e-02 & -6.301442e-02 \\
404 & -6.467824e-02 & -1.334170e-02 & -5.297457e-01 &      0.0 & -3.446620e-04 & -1.111286e-03 &  4.818083e-02 & -9.328788e-02 \\
405 & -6.434286e-02 &  1.844592e-02 &  4.678429e-01 &      0.0 &  1.199259e-04 &  5.089864e-04 &  1.067825e-01 & -1.026469e-01 \\
406 & -7.642489e-02 &  2.107655e-02 & -5.552209e-01 &      0.0 &  7.554759e-04 & -2.613478e-03 &  1.986629e-01 & -1.095651e-01 \\
407 & -9.292521e-02 &  1.698785e-02 &  1.690190e-01 &      0.0 & -2.941204e-03 & -1.849305e-03 &  2.389082e-01 & -8.875191e-02 \\
408 & -1.048330e-01 &  2.177050e-02 & -9.562339e-01 &      0.0 &  8.788072e-04 & -6.969195e-04 &  2.362384e-01 & -2.443386e-02 \\
409 & -9.697084e-02 &  1.119570e-02 &  8.248732e-02 &      0.0 &  1.437833e-03 &  8.661213e-05 &  1.339937e-01 &  3.516556e-02 \\
410 & -5.813400e-02 & -2.703692e-02 & -6.505999e-01 &      0.0 & -4.207809e-04 &  9.281782e-05 &  5.539951e-02 &  2.607601e-02 \\
411 & -4.154117e-03 & -7.154267e-02 & -1.215256e-01 &      0.0 & -8.484168e-04 &  1.349793e-03 &  1.079560e-02 &  1.778614e-03 \\
412 &  5.266117e-02 & -8.154171e-02 & -2.051698e-01 &      0.0 &  2.120215e-03 & -2.644981e-03 &  9.353055e-03 & -4.114375e-03 \\
413 &  9.126633e-02 & -3.512781e-02 & -3.057209e-01 &      0.0 & -8.521765e-04 &  1.610960e-03 &  2.017350e-02 & -1.473571e-02 \\
414 &  8.972638e-02 &  1.218363e-02 &  3.136067e-01 &      0.0 &  1.660634e-03 &  2.672932e-03 &  7.973540e-03 & -8.764952e-03 \\
415 &  6.018858e-02 &  3.326567e-02 &  1.229151e-01 &      0.0 & -7.765975e-04 &  7.531458e-04 & -8.731761e-03 & -2.025634e-02 \\
416 &  1.826655e-02 &  1.882445e-02 &  4.557304e-01 &      0.0 & -4.793815e-04 &  4.953023e-03 & -1.148217e-02 & -1.042111e-02 \\
417 &  4.253158e-04 &  2.588471e-03 & -1.008389e+00 &      0.0 &  3.021855e-04 & -6.680737e-03 &  4.650513e-03 & -6.957938e-03 \\
418 & -2.974750e-05 &  2.669857e-05 &  1.764271e+00 &      0.0 &  5.176454e-04 & -2.384990e-03 &  9.715468e-05 & -8.805519e-05 \\
419 &  0.000000e+00 & -0.000000e+00 &  9.178320e-17 &      0.0 & -5.521029e-15 & -3.411160e-14 &  1.000827e-08 &  2.423717e-07 \\
420 &  0.000000e+00 & -0.000000e+00 &  9.975771e-17 &      0.0 &  2.093551e-14 &  2.556289e-14 &  6.372745e-08 &  6.105418e-07 \\
421 &  0.000000e+00 & -0.000000e+00 & -1.919648e-16 &      0.0 & -4.576672e-14 &  4.307665e-14 & -3.826940e-08 &  1.759799e-07 \\
422 &  0.000000e+00 & -0.000000e+00 &  2.751036e-16 &      0.0 & -1.038056e-15 &  7.049916e-15 & -3.453018e-08 &  2.968420e-07 \\
423 &  1.552189e-05 &  3.339611e-04 &  1.939945e+01 &      0.0 &  6.428742e-04 & -4.368280e-04 &  2.576235e-04 & -3.072459e-04 \\
424 &  8.975598e-03 &  4.179102e-03 &  7.466158e-01 &      0.0 & -1.391411e-05 &  2.824727e-03 & -1.231814e-04 &  1.343081e-02 \\
425 &  4.945257e-02 &  2.888739e-02 &  8.273307e-01 &      0.0 & -1.137947e-03 & -3.228132e-03 & -2.639202e-02 &  2.737804e-06 \\
426 &  8.826920e-02 &  3.913028e-02 & -5.500841e-01 &      0.0 &  2.620996e-03 &  2.883815e-03 & -1.904372e-02 &  6.772723e-03 \\
427 &  9.945629e-02 &  1.974493e-02 & -4.446346e-01 &      0.0 &  1.705262e-03 & -1.713752e-03 & -8.336584e-03 &  3.553993e-02 \\
428 &  6.258743e-02 & -2.423451e-02 & -2.135028e-01 &      0.0 &  4.356440e-04 & -6.415647e-03 &  2.574444e-02 &  7.900510e-02 \\
429 & -5.483893e-03 & -7.016264e-02 & -2.075023e-01 &      0.0 & -2.696846e-03 &  1.437217e-03 &  3.254246e-02 &  8.802051e-02 \\
430 & -5.949497e-02 & -6.743301e-02 & -2.088404e-02 &      0.0 & -1.136007e-03 &  1.691109e-03 &  4.370950e-02 &  5.414963e-02 \\
431 & -7.522377e-02 & -2.589138e-02 & -4.778959e-01 &      0.0 &  1.368637e-03 &  5.573597e-04 &  6.813285e-02 &  3.018621e-02 \\
432 & -7.258667e-02 &  9.027676e-03 &  2.086048e-01 &      0.0 &  2.597185e-03 & -2.445974e-03 &  1.048078e-01 &  1.407483e-02 \\
433 & -7.186759e-02 &  1.529347e-02 & -1.166690e-02 &      0.0 &  2.722647e-03 &  5.252034e-04 &  1.836152e-01 &  2.626194e-02 \\
434 & -7.908519e-02 &  6.369992e-03 & -5.712415e-01 &      0.0 & -1.288251e-03 &  5.664493e-04 &  2.477873e-01 &  2.721382e-02 \\
435 & -9.227256e-02 &  4.919126e-03 &  7.610144e-02 &      0.0 &  5.411641e-04 &  1.069374e-03 &  2.305170e-01 &  2.867332e-02 \\
436 & -1.017815e-01 &  1.328809e-02 & -4.458476e-01 &      0.0 & -3.414323e-04 &  3.561837e-04 &  1.855620e-01 &  9.638066e-02 \\
437 & -8.529941e-02 & -2.592103e-03 & -1.218665e-01 &      0.0 & -5.466641e-04 & -2.613007e-03 &  9.209357e-02 &  1.531720e-01 \\
438 & -4.165669e-02 & -4.746341e-02 &  5.590709e-01 &      0.0 & -1.331552e-03 &  5.738230e-04 &  2.126554e-02 &  1.149557e-01 \\
439 &  1.314376e-02 & -9.107650e-02 &  4.021968e-01 &      0.0 &  1.381850e-04 & -2.692647e-03 & -2.511180e-03 &  4.559618e-02 \\
440 &  5.901622e-02 & -8.828631e-02 & -1.145449e-01 &      0.0 & -1.666101e-03 &  4.396004e-03 &  9.773907e-03 & -1.503914e-02 \\
441 &  8.755210e-02 & -3.237143e-02 &  5.611527e-02 &      0.0 & -7.732441e-04 & -8.965144e-04 &  2.369589e-02 & -4.262629e-03 \\
442 &  8.145104e-02 &  2.023003e-02 &  1.996200e-02 &      0.0 &  7.142622e-04 & -3.510319e-03 &  1.927574e-02 &  3.219984e-03 \\
443 &  5.234840e-02 &  3.760152e-02 &  5.938880e-01 &      0.0 & -2.691638e-03 &  4.077927e-04 & -1.017104e-02 & -8.024315e-03 \\
444 &  1.604047e-02 &  2.113886e-02 &  1.104892e+00 &      0.0 & -4.760873e-04 &  9.819434e-05 & -5.429563e-03 & -8.595937e-03 \\
445 &  2.678691e-04 &  2.366621e-03 &  2.602497e+00 &      0.0 &  3.095721e-04 &  4.843874e-03 &  3.812018e-03 & -5.114696e-03 \\
446 & -6.409453e-05 &  2.465919e-05 & -4.486952e+00 &      0.0 &  6.117222e-04 & -2.553222e-03 &  1.489682e-04 & -1.605184e-04 \\
447 &  0.000000e+00 & -0.000000e+00 & -2.765754e-17 &      0.0 & -1.196467e-14 &  2.423062e-14 & -1.106678e-07 & -1.421174e-07 \\
448 &  0.000000e+00 & -0.000000e+00 &  6.549300e-18 &      0.0 &  2.088781e-14 &  2.478573e-14 & -8.670253e-08 & -2.268158e-07 \\
449 &  0.000000e+00 & -0.000000e+00 & -5.388378e-17 &      0.0 &  2.379306e-14 &  1.082467e-14 & -9.238395e-08 & -3.421355e-07 \\
450 &  0.000000e+00 & -0.000000e+00 & -7.064422e-17 &      0.0 & -1.184816e-15 &  1.561251e-15 &  5.732065e-08 &  7.651607e-07 \\
451 &  1.835934e-05 &  9.192514e-05 & -4.872328e+01 &      0.0 & -1.491575e-04 &  6.831004e-04 &  1.553970e-04 &  1.480195e-04 \\
452 &  1.251791e-02 &  2.291247e-03 & -9.070356e-01 &      0.0 & -1.433576e-03 &  1.437001e-03 & -2.317377e-03 &  1.099523e-02 \\
453 &  5.871765e-02 &  1.890332e-02 & -1.624141e-01 &      0.0 &  1.790948e-03 &  1.726467e-04 & -2.188896e-02 & -5.004451e-03 \\
454 &  9.654511e-02 &  2.085874e-02 & -4.746976e-02 &      0.0 & -4.314712e-03 & -6.275796e-04 & -2.965818e-02 & -2.038651e-03 \\
455 &  1.042438e-01 & -8.126536e-03 &  5.952638e-01 &      0.0 & -1.015425e-03 &  5.391172e-04 & -2.537422e-02 &  1.062435e-02 \\
456 &  6.249088e-02 & -5.232124e-02 &  2.850851e-02 &      0.0 & -5.307908e-04 &  6.098284e-03 &  7.236992e-03 &  6.004049e-02 \\
457 & -7.622896e-03 & -7.522216e-02 &  4.244443e-01 &      0.0 &  1.524682e-03 &  1.154359e-03 &  2.941000e-03 &  9.707626e-02 \\
458 & -5.819822e-02 & -5.080256e-02 & -1.835008e-01 &      0.0 &  2.733057e-04 & -1.900949e-03 &  3.221315e-02 &  1.169625e-01 \\
459 & -7.062684e-02 & -1.260938e-02 &  2.983147e-01 &      0.0 & -2.002287e-03 &  1.222468e-03 &  6.578226e-02 &  1.117851e-01 \\
460 & -6.535696e-02 &  2.360628e-03 & -4.376209e-01 &      0.0 & -1.962480e-03 &  1.783913e-03 &  1.262739e-01 &  1.190369e-01 \\
461 & -6.417512e-02 & -6.514190e-03 & -1.389174e-01 &      0.0 & -7.367611e-04 &  1.399188e-04 &  2.025205e-01 &  1.116313e-01 \\
462 & -7.112499e-02 & -1.059698e-02 & -4.492926e-01 &      0.0 & -1.621861e-03 &  6.331979e-04 &  2.058825e-01 &  4.936099e-02 \\
463 & -8.404058e-02 &  4.523766e-03 &  2.712752e-02 &      0.0 & -5.445309e-04 & -1.708710e-04 &  1.580346e-01 &  1.925525e-02 \\
464 & -8.427049e-02 &  1.561991e-02 &  5.743537e-03 &      0.0 & -1.752419e-05 &  2.009065e-03 &  9.130601e-02 &  9.135608e-02 \\
465 & -6.015368e-02 & -1.013318e-02 & -2.038401e-01 &      0.0 &  4.833478e-04 &  4.370816e-04 &  1.780704e-02 &  1.613218e-01 \\
466 & -1.879203e-02 & -6.710145e-02 & -8.427111e-01 &      0.0 & -4.236634e-04 &  1.653237e-03 & -1.373005e-02 &  1.411360e-01 \\
467 &  3.021051e-02 & -1.049629e-01 &  5.095989e-02 &      0.0 &  1.182523e-03 &  3.782896e-03 & -1.732924e-02 &  4.633439e-02 \\
468 &  6.689114e-02 & -8.413443e-02 &  4.564882e-01 &      0.0 & -4.800647e-05 & -1.581293e-03 & -1.791949e-04 & -1.401640e-02 \\
469 &  8.356363e-02 & -1.754262e-02 &  6.442561e-01 &      0.0 & -9.169920e-04 &  1.037583e-03 &  1.934506e-02 &  4.404086e-03 \\
470 &  7.197319e-02 &  3.093721e-02 & -1.158759e+00 &      0.0 & -2.986810e-04 &  4.339747e-04 &  1.383615e-02 & -3.853174e-03 \\
471 &  4.202402e-02 &  3.778506e-02 &  2.131868e-02 &      0.0 &  3.502005e-03 & -1.758937e-05 & -4.170361e-03 & -2.627862e-03 \\
472 &  1.222199e-02 &  1.866686e-02 &  5.448777e-01 &      0.0 & -1.502453e-03 &  2.072321e-03 &  3.560788e-03 & -1.596782e-03 \\
473 &  1.698400e-04 &  1.736450e-03 &  1.767086e-01 &      0.0 &  4.990044e-04 &  5.017016e-02 &  2.759641e-03 & -2.727822e-03 \\
474 & -1.679294e-05 &  1.507177e-05 &  3.125280e+00 &      0.0 &  5.176633e-04 & -2.385132e-03 &  5.479370e-05 & -4.985999e-05 \\
475 &  0.000000e+00 & -0.000000e+00 &  1.607502e-16 &      0.0 &  2.596068e-15 &  3.594347e-15 & -2.922401e-07 & -1.866987e-06 \\
476 &  0.000000e+00 & -0.000000e+00 &  5.224668e-17 &      0.0 &  2.940790e-15 &  5.551115e-16 &  8.334037e-08 &  6.179590e-07 \\
477 &  0.000000e+00 & -0.000000e+00 &  2.009991e-16 &      0.0 & -5.313106e-15 &  5.551115e-17 & -2.039120e-08 & -4.944325e-07 \\
478 & -4.733328e-05 & -4.117859e-06 & -4.788098e+00 &      0.0 &  3.821563e-04 & -1.167173e-03 &  3.790430e-05 & -1.763619e-04 \\
479 &  3.655494e-05 &  1.668981e-04 &  1.246717e+02 &      0.0 &  5.911663e-04 & -1.232225e-03 &  1.251496e-04 &  4.753609e-04 \\
480 &  1.570415e-02 & -1.010330e-03 &  2.050901e+00 &      0.0 &  1.628386e-03 & -7.352694e-04 & -4.649155e-03 &  6.618841e-03 \\
481 &  6.387308e-02 &  5.977152e-03 &  4.155447e-01 &      0.0 &  2.315333e-03 & -2.760068e-03 & -2.318723e-02 &  3.359355e-03 \\
482 &  9.978635e-02 &  2.889504e-03 & -7.394718e-01 &      0.0 &  4.311686e-03 & -6.881288e-04 & -3.474360e-02 & -5.038518e-03 \\
483 &  1.055375e-01 & -2.755672e-02 & -1.863616e-01 &      0.0 & -7.002536e-05 &  1.040764e-03 & -3.527107e-02 & -1.559856e-02 \\
484 &  6.654498e-02 & -6.731432e-02 &  1.240266e-02 &      0.0 &  8.719087e-04 & -3.308632e-03 & -2.475164e-02 &  4.438881e-03 \\
485 &  3.715792e-03 & -8.228019e-02 & -6.378713e-01 &      0.0 & -9.730253e-04 & -2.469982e-03 & -2.590652e-02 &  5.209062e-02 \\
486 & -4.482330e-02 & -5.763650e-02 &  2.185610e-01 &      0.0 & -1.617515e-04 &  3.507599e-03 & -2.240669e-03 &  6.587695e-02 \\
487 & -5.595698e-02 & -3.172330e-02 &  2.007924e-01 &      0.0 & -6.041759e-04 & -5.724546e-04 &  4.477163e-02 &  8.955811e-02 \\
488 & -5.290929e-02 & -2.567268e-02 & -1.180208e-01 &      0.0 &  3.792917e-04 & -9.360762e-04 &  9.209653e-02 &  8.230676e-02 \\
489 & -5.363413e-02 & -2.541234e-02 &  2.991662e-02 &      0.0 &  3.765390e-05 & -1.871644e-04 &  1.313860e-01 &  2.813489e-02 \\
490 & -6.292798e-02 & -1.650320e-02 & -7.023763e-03 &      0.0 &  5.594425e-04 &  1.365171e-04 &  1.092970e-01 & -6.033584e-02 \\
491 & -6.985920e-02 &  2.394321e-04 & -9.546124e-01 &      0.0 &  4.657724e-03 & -1.461815e-03 &  7.731901e-02 & -5.212602e-02 \\
492 & -6.315657e-02 & -3.499783e-03 & -5.564560e-01 &      0.0 & -2.629017e-03 & -1.347953e-03 &  2.522253e-02 &  6.258864e-02 \\
493 & -3.610494e-02 & -4.286478e-02 &  6.218094e-02 &      0.0 &  7.438028e-05 &  1.481621e-03 & -1.554492e-02 &  1.396789e-01 \\
494 &  8.405211e-03 & -8.886582e-02 &  1.969267e-01 &      0.0 &  2.705404e-03 & -2.354368e-03 & -2.651515e-02 &  1.164798e-01 \\
495 &  4.663673e-02 & -9.983922e-02 & -3.930430e-01 &      0.0 & -1.354154e-03 &  8.881547e-04 & -7.406495e-03 &  4.249934e-02 \\
496 &  7.408325e-02 & -5.546932e-02 & -1.369299e+00 &      0.0 &  9.789323e-04 & -1.427635e-03 &  1.366924e-02 & -2.520476e-03 \\
497 &  7.496817e-02 &  8.368046e-03 & -1.609829e-02 &      0.0 &  8.345918e-04 & -2.396345e-04 &  8.248893e-03 &  4.275905e-03 \\
498 &  5.926795e-02 &  4.044215e-02 &  2.648733e-01 &      0.0 &  6.218130e-05 & -2.003489e-03 &  6.100625e-03 & -1.010398e-02 \\
499 &  3.018331e-02 &  3.296366e-02 & -2.790550e-01 &      0.0 & -1.248869e-03 &  1.643801e-03 &  4.273384e-03 &  1.841376e-03 \\
500 &  8.919220e-03 &  1.463303e-02 & -2.095281e+00 &      0.0 &  3.457112e-03 & -1.482336e-02 &  5.719496e-03 &  9.328324e-04 \\
501 & -6.875462e-05 &  9.420436e-04 & -3.557696e+00 &      0.0 &  1.851976e-03 &  1.668053e-01 &  1.507758e-03 & -5.516039e-04 \\
502 & -8.994523e-05 & -2.192261e-04 &  1.830159e+00 &      0.0 &  2.878012e-04 & -1.013412e-03 &  3.730369e-04 &  2.187720e-04 \\
503 &  0.000000e+00 & -0.000000e+00 & -3.778672e-17 &      0.0 &  1.140488e-17 & -1.703498e-15 &  5.152992e-08 & -6.114381e-08 \\
504 &  0.000000e+00 & -0.000000e+00 &  1.279092e-16 &      0.0 & -4.452475e-18 &  1.734723e-17 & -7.427130e-08 & -3.395744e-07 \\
505 &  0.000000e+00 & -0.000000e+00 & -1.203028e-16 &      0.0 & -3.227672e-18 & -1.077263e-15 & -1.452950e-07 & -1.173685e-06 \\
506 & -1.092968e-04 & -9.508511e-06 & -2.073586e+00 &      0.0 &  3.821723e-04 & -1.167217e-03 &  8.782846e-05 & -4.052199e-04 \\
507 &  1.167069e-04 &  2.542457e-04 & -7.099195e+01 &      0.0 &  3.769310e-04 & -3.841156e-04 & -1.501147e-03 & -7.386814e-04 \\
508 &  1.664089e-02 & -5.159330e-03 & -9.014129e-02 &      0.0 &  1.075477e-03 & -4.520919e-04 & -5.140378e-03 &  2.619066e-03 \\
509 &  6.089805e-02 & -4.493567e-03 & -2.830315e-01 &      0.0 & -5.373320e-03 &  5.007039e-04 & -2.040538e-02 &  1.736854e-02 \\
510 &  9.862495e-02 & -1.063296e-02 &  5.775886e-01 &      0.0 & -7.980557e-04 &  1.399916e-03 & -2.625634e-02 &  9.668426e-03 \\
511 &  1.067131e-01 & -3.594150e-02 &  5.245588e-01 &      0.0 & -1.301948e-03 & -1.699238e-03 & -4.456636e-02 & -7.339651e-03 \\
512 &  7.437911e-02 & -6.654548e-02 & -3.072831e-01 &      0.0 & -3.804326e-04 &  2.144322e-03 & -3.908025e-02 & -1.197675e-02 \\
513 &  1.850121e-02 & -8.262182e-02 &  4.104523e-01 &      0.0 &  3.210795e-04 &  9.583763e-04 & -4.925987e-02 &  1.537712e-03 \\
514 & -2.599462e-02 & -7.138438e-02 & -1.368784e-01 &      0.0 &  8.502654e-04 & -2.658723e-03 & -3.988097e-02 &  1.263899e-02 \\
515 & -4.285949e-02 & -5.735454e-02 &  4.160490e-02 &      0.0 & -2.393164e-04 & -5.508754e-04 &  1.380128e-02 &  1.891620e-02 \\
516 & -4.314758e-02 & -5.065375e-02 &  3.361043e-01 &      0.0 &  1.156516e-03 &  5.671604e-04 &  5.057849e-02 &  8.008013e-03 \\
517 & -4.559122e-02 & -4.500943e-02 & -2.210695e-01 &      0.0 & -1.350221e-03 &  3.009991e-04 &  7.958903e-02 & -7.032367e-02 \\
518 & -5.560814e-02 & -3.327658e-02 & -5.904868e-01 &      0.0 & -1.710049e-03 &  2.115096e-03 &  6.554463e-02 & -1.389787e-01 \\
519 & -5.465414e-02 & -2.717694e-02 &  3.592736e-01 &      0.0 &  1.381755e-03 &  4.550644e-04 &  2.936111e-02 & -8.436830e-02 \\
520 & -3.873710e-02 & -4.211559e-02 &  1.203334e-01 &      0.0 &  7.477672e-04 & -2.116296e-03 &  8.782195e-03 &  4.668917e-02 \\
521 & -4.467340e-03 & -7.719329e-02 & -5.406752e-01 &      0.0 & -2.286714e-03 &  9.229425e-04 & -1.503950e-02 &  1.140429e-01 \\
522 &  3.210299e-02 & -9.052170e-02 &  5.470135e-01 &      0.0 & -2.322935e-03 &  1.712680e-03 & -4.261593e-03 &  9.428612e-02 \\
523 &  6.222136e-02 & -6.353748e-02 &  4.964774e-01 &      0.0 &  1.961316e-03 & -1.493485e-03 &  7.368419e-03 &  2.646233e-02 \\
524 &  7.369980e-02 & -8.788011e-03 &  2.585981e-01 &      0.0 & -3.527079e-03 &  3.549405e-03 &  3.191109e-03 &  2.312181e-03 \\
525 &  6.453579e-02 &  3.327574e-02 &  1.674817e-01 &      0.0 &  1.389495e-03 &  1.102241e-04 &  1.167607e-03 &  1.553431e-03 \\
526 &  4.184823e-02 &  3.873306e-02 & -5.229972e-01 &      0.0 &  1.580926e-03 & -1.179459e-03 &  9.086071e-03 &  3.226286e-03 \\
527 &  1.833588e-02 &  2.475373e-02 & -1.597526e+00 &      0.0 & -6.360094e-04 & -5.522450e-03 &  8.642558e-03 & -2.415418e-05 \\
528 &  4.689209e-03 &  8.677920e-03 &  3.143135e+00 &      0.0 & -1.762278e-03 &  1.431052e-02 &  2.669350e-03 & -5.169635e-03 \\
529 &  4.731360e-05 &  5.472003e-04 & -2.311694e+00 &      0.0 &  1.356520e-03 &  8.789641e-02 &  4.430009e-05 & -1.051850e-03 \\
530 & -2.969890e-05 & -7.238597e-05 &  5.542767e+00 &      0.0 &  2.878026e-04 & -1.013728e-03 &  1.231132e-04 &  7.226422e-05 \\
531 &  0.000000e+00 & -0.000000e+00 &  1.318916e-16 &      0.0 &  0.000000e+00 &  2.802597e-45 &  8.238667e-08 &  6.071568e-07 \\
532 &  0.000000e+00 & -0.000000e+00 &  1.112839e-16 &      0.0 &  0.000000e+00 & -2.802597e-45 &  1.577008e-07 &  1.095519e-06 \\
533 &  0.000000e+00 & -0.000000e+00 &  6.956042e-17 &      0.0 &  0.000000e+00 & -1.401298e-45 & -6.767225e-08 & -9.059859e-07 \\
534 &  0.000000e+00 & -0.000000e+00 &  9.245454e-17 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.337979e-07 & -2.546577e-07 \\
535 &  3.015029e-04 & -3.913438e-05 &  6.796172e+00 &      0.0 & -3.792841e-04 & -2.147494e-04 & -1.013179e-03 & -7.633375e-04 \\
536 &  1.513378e-02 & -7.389839e-03 & -1.235424e+00 &      0.0 & -1.170938e-03 &  1.493678e-03 & -1.802924e-03 &  2.545586e-03 \\
537 &  5.354056e-02 & -1.195370e-02 & -3.850352e-01 &      0.0 &  2.111004e-03 & -1.773393e-04 & -1.798711e-02 &  2.030949e-02 \\
538 &  9.206271e-02 & -1.825214e-02 &  5.571724e-01 &      0.0 & -2.461146e-03 &  7.797713e-04 & -1.857551e-02 &  2.903186e-02 \\
539 &  1.069718e-01 & -3.536910e-02 &  6.422343e-01 &      0.0 & -1.332844e-03 &  3.182423e-03 & -5.376804e-02 &  6.270621e-03 \\
540 &  8.663077e-02 & -5.651400e-02 &  6.111804e-01 &      0.0 &  7.517337e-04 & -1.541406e-03 & -6.134788e-02 & -1.480226e-03 \\
541 &  4.459374e-02 & -7.724974e-02 & -2.051975e-01 &      0.0 & -1.848963e-03 & -2.794492e-05 & -7.089839e-02 & -2.779363e-03 \\
542 &  1.743516e-05 & -8.755507e-02 &  9.835419e-02 &      0.0 & -3.402084e-04 &  1.340803e-03 & -6.988386e-02 & -8.711724e-03 \\
543 & -2.625140e-02 & -8.673331e-02 & -3.505020e-01 &      0.0 &  3.758317e-03 & -7.340623e-04 & -2.455168e-02 & -1.348050e-02 \\
544 & -3.549173e-02 & -8.053967e-02 &  6.207505e-01 &      0.0 & -4.014035e-03 & -7.284177e-05 &  1.137242e-02 & -5.157973e-02 \\
545 & -3.936584e-02 & -7.175882e-02 & -7.575861e-01 &      0.0 &  1.087721e-03 & -4.488376e-04 &  5.414383e-02 & -1.117643e-01 \\
546 & -4.216276e-02 & -6.271974e-02 &  7.246063e-01 &      0.0 & -8.057453e-04 & -1.586996e-03 &  5.481736e-02 & -1.233932e-01 \\
547 & -3.111870e-02 & -6.684347e-02 & -2.728561e-01 &      0.0 &  2.369415e-03 &  3.507957e-03 &  3.701853e-02 & -4.707800e-02 \\
548 & -6.009239e-03 & -8.061605e-02 &  7.223978e-01 &      0.0 & -1.234991e-03 &  7.863627e-04 &  2.139669e-02 &  5.081036e-02 \\
549 &  2.207684e-02 & -8.137574e-02 & -4.074972e-01 &      0.0 &  1.726303e-03 & -3.599152e-03 &  1.613686e-02 &  9.947454e-02 \\
550 &  5.226185e-02 & -5.653499e-02 & -7.093022e-01 &      0.0 &  1.416340e-03 & -2.074750e-03 &  2.853094e-02 &  7.029269e-02 \\
551 &  6.770914e-02 & -5.122454e-03 & -8.503429e-02 &      0.0 &  1.757754e-03 & -7.145692e-04 &  1.580309e-02 &  3.353491e-02 \\
552 &  6.351522e-02 &  2.960469e-02 & -4.937613e-01 &      0.0 &  1.870087e-03 & -2.028304e-06 &  1.504683e-02 &  1.420279e-02 \\
553 &  4.881008e-02 &  4.113525e-02 &  9.761380e-01 &      0.0 & -6.250195e-04 &  1.571972e-03 &  5.272713e-03 &  1.068236e-02 \\
554 &  2.484706e-02 &  3.031299e-02 &  1.237744e+00 &      0.0 &  9.434856e-04 &  4.051698e-03 &  1.512917e-02 &  8.665472e-03 \\
555 &  9.057751e-03 &  1.631279e-02 & -3.946293e-01 &      0.0 & -2.366512e-04 &  5.369901e-03 &  7.001058e-03 & -1.395681e-03 \\
556 &  1.692447e-03 &  3.996991e-03 &  1.721535e-01 &      0.0 &  1.058079e-03 &  6.988393e-03 &  4.360652e-04 & -4.554439e-03 \\
557 &  9.884899e-06 &  2.415830e-04 &  1.374951e+01 &      0.0 &  3.066746e-04 & -4.189415e-02 &  7.851131e-06 &  1.008061e-04 \\
558 &  0.000000e+00 & -0.000000e+00 & -2.871058e-17 &      0.0 &  0.000000e+00 & -0.000000e+00 &  4.024079e-09 &  2.396836e-07 \\
559 &  0.000000e+00 & -0.000000e+00 & -9.827127e-17 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.861283e-07 & -1.340040e-06 \\
560 &  0.000000e+00 & -0.000000e+00 & -4.101789e-17 &      0.0 &  0.000000e+00 & -0.000000e+00 & -3.031730e-07 & -1.864833e-06 \\
561 &  0.000000e+00 & -0.000000e+00 & -6.162170e-17 &      0.0 &  0.000000e+00 & -0.000000e+00 & -6.980414e-08 & -3.985736e-07 \\
562 &  0.000000e+00 & -0.000000e+00 &  1.071649e-16 &      0.0 &  0.000000e+00 & -0.000000e+00 & -8.352599e-10 &  4.913519e-08 \\
563 &  2.429149e-04 &  9.168953e-05 & -7.781624e+00 &      0.0 &  1.073085e-04 & -2.495466e-04 & -3.213437e-03 & -2.398934e-03 \\
564 &  1.111912e-02 & -6.530904e-03 &  3.596310e-01 &      0.0 &  1.329734e-03 &  1.765625e-05 & -4.161147e-03 & -4.507097e-03 \\
565 &  3.802970e-02 & -1.631012e-02 &  7.037769e-01 &      0.0 & -8.874123e-04 & -2.573819e-04 & -1.705342e-02 &  3.248611e-03 \\
566 &  7.792551e-02 & -2.318908e-02 &  2.028375e-01 &      0.0 & -1.049686e-03 & -8.009258e-06 & -1.439199e-02 &  3.445847e-02 \\
567 &  1.023534e-01 & -3.292897e-02 & -6.388816e-01 &      0.0 &  3.201089e-03 & -5.385852e-03 & -2.991529e-02 &  2.195907e-02 \\
568 &  1.007139e-01 & -4.649304e-02 &  1.490635e-01 &      0.0 & -4.826927e-04 &  1.443185e-03 & -5.646401e-02 &  1.487690e-02 \\
569 &  7.821464e-02 & -6.977330e-02 & -7.538368e-02 &      0.0 &  1.260943e-03 &  6.673170e-04 & -8.456904e-02 &  7.532582e-03 \\
570 &  4.158062e-02 & -9.426948e-02 &  9.297707e-01 &      0.0 & -1.937611e-03 & -8.037576e-05 & -9.667866e-02 &  2.024893e-02 \\
571 &  1.225991e-02 & -1.069838e-01 &  2.182313e-02 &      0.0 &  3.682945e-04 & -7.768826e-04 & -6.238688e-02 & -2.246821e-02 \\
572 & -7.334650e-03 & -1.047991e-01 & -2.716540e-01 &      0.0 & -2.806774e-03 &  4.908323e-04 &  7.448601e-04 & -6.682504e-02 \\
573 & -1.449466e-02 & -9.684847e-02 &  5.992178e-01 &      0.0 & -1.659917e-04 &  2.948347e-03 &  4.290166e-02 & -1.044717e-01 \\
574 & -1.111428e-02 & -9.035069e-02 & -8.880922e-01 &      0.0 & -4.268601e-04 & -1.279428e-03 &  6.341254e-02 & -1.006912e-01 \\
575 &  4.958594e-03 & -8.463858e-02 & -1.613192e-01 &      0.0 &  1.297600e-03 & -9.752343e-04 &  5.337030e-02 & -3.603197e-03 \\
576 &  2.637485e-02 & -6.911179e-02 & -4.812718e-01 &      0.0 &  2.790097e-04 &  1.392522e-03 &  3.414822e-02 &  7.126108e-02 \\
577 &  4.932604e-02 & -3.418569e-02 &  5.084936e-01 &      0.0 & -2.540660e-03 &  1.820103e-03 &  2.976548e-02 &  9.313524e-02 \\
578 &  6.338564e-02 &  9.694169e-03 &  2.046697e-01 &      0.0 & -3.644945e-03 &  5.379051e-03 &  3.570932e-02 &  7.239511e-02 \\
579 &  6.006904e-02 &  4.423508e-02 &  1.140782e-01 &      0.0 & -1.522917e-03 &  5.880949e-04 &  3.491846e-02 &  6.913956e-02 \\
580 &  4.786930e-02 &  4.703957e-02 &  5.099606e-01 &      0.0 & -7.199313e-04 &  4.311919e-03 &  1.849971e-02 &  3.373900e-02 \\
581 &  2.944711e-02 &  3.505369e-02 &  4.406561e-01 &      0.0 &  4.692244e-04 &  2.300350e-03 &  1.225583e-02 &  1.764287e-02 \\
582 &  1.238627e-02 &  2.027627e-02 & -2.869647e+00 &      0.0 & -3.120510e-03 &  6.532167e-03 &  9.120912e-03 &  8.232542e-03 \\
583 &  3.625255e-03 &  8.087917e-03 &  3.987030e+00 &      0.0 & -2.059745e-04 & -4.324569e-03 &  3.510562e-04 & -7.891839e-03 \\
584 &  3.534136e-04 &  1.723241e-03 & -2.023992e+01 &      0.0 & -2.084024e-03 & -1.666497e-02 & -1.081825e-03 & -3.783496e-03 \\
585 &  3.216547e-05 & -4.045509e-05 &  3.490891e+01 &      0.0 &  2.699661e-04 &  7.868290e-03 & -5.272680e-04 & -1.428933e-04 \\
586 &  5.901058e-05 & -1.561953e-04 & -2.213941e+00 &      0.0 & -4.849267e-05 &  4.231611e-03 & -1.183114e-03 & -6.626111e-04 \\
587 &  0.000000e+00 & -0.000000e+00 & -1.457286e-31 &      0.0 &  0.000000e+00 & -0.000000e+00 & -7.775692e-08 &  1.691464e-07 \\
588 &  0.000000e+00 & -0.000000e+00 & -5.169935e-32 &      0.0 &  0.000000e+00 & -0.000000e+00 &  7.558982e-08 & -1.211465e-08 \\
589 &  0.000000e+00 & -0.000000e+00 &  1.412998e-32 &      0.0 &  0.000000e+00 & -0.000000e+00 & -9.511643e-08 & -4.628999e-07 \\
590 &  0.000000e+00 & -0.000000e+00 &  1.383603e-31 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.101763e-07 &  5.643005e-07 \\
591 &  1.276555e-04 &  4.204517e-05 &  1.522571e+01 &      0.0 &  3.637722e-04 & -3.588747e-04 & -3.667674e-03 & -2.939415e-03 \\
592 &  6.372182e-03 & -4.323670e-03 & -4.971582e-01 &      0.0 & -4.671818e-04 & -1.661435e-03 & -4.326562e-03 &  4.747543e-03 \\
593 &  2.507423e-02 & -1.627059e-02 & -7.676248e-01 &      0.0 & -1.077033e-03 &  3.373921e-03 & -2.037685e-02 & -1.721845e-03 \\
594 &  5.439854e-02 & -2.488212e-02 & -4.427056e-01 &      0.0 &  6.907541e-04 &  9.332220e-04 & -2.076191e-02 &  2.679081e-02 \\
595 &  8.859094e-02 & -3.348172e-02 & -4.318043e-02 &      0.0 &  1.540087e-04 &  2.779735e-03 & -1.852560e-02 &  3.400380e-02 \\
596 &  1.050620e-01 & -3.868529e-02 &  4.747022e-01 &      0.0 & -1.691291e-03 &  7.690844e-04 & -3.775569e-02 &  2.667910e-02 \\
597 &  1.039182e-01 & -5.644295e-02 & -2.190148e-01 &      0.0 & -5.025968e-04 & -8.306441e-04 & -7.974893e-02 &  5.711449e-03 \\
598 &  8.618146e-02 & -8.023461e-02 & -8.967350e-02 &      0.0 &  1.956389e-03 & -4.550548e-04 & -1.023770e-01 & -5.950548e-03 \\
599 &  6.125428e-02 & -9.533456e-02 & -1.138328e-01 &      0.0 &  1.097497e-03 & -1.954060e-03 & -8.461495e-02 & -5.344821e-02 \\
600 &  3.792580e-02 & -9.987855e-02 &  6.103369e-02 &      0.0 & -5.903750e-04 &  3.515719e-05 & -2.948776e-02 & -1.034461e-01 \\
601 &  2.707399e-02 & -9.054901e-02 & -2.958891e-01 &      0.0 & -2.294029e-03 &  1.091562e-03 &  1.490421e-02 & -1.101282e-01 \\
602 &  2.870875e-02 & -7.112201e-02 &  2.532253e-01 &      0.0 &  4.298768e-03 & -3.043547e-03 &  2.111821e-02 & -5.484254e-02 \\
603 &  4.084742e-02 & -4.547398e-02 & -4.205169e-04 &      0.0 & -2.093314e-03 &  3.931113e-03 &  7.783915e-03 &  3.091899e-02 \\
604 &  5.424670e-02 & -6.992187e-03 &  5.080549e-01 &      0.0 & -4.437275e-04 & -1.983115e-03 &  4.735842e-03 &  5.676776e-02 \\
605 &  6.037220e-02 &  3.381457e-02 & -4.486665e-01 &      0.0 &  3.527609e-03 & -3.503054e-03 &  2.854422e-02 &  8.388750e-02 \\
606 &  5.478670e-02 &  5.531071e-02 & -5.291836e-01 &      0.0 & -1.918909e-03 & -3.045071e-03 &  2.310345e-02 &  6.418813e-02 \\
607 &  4.122003e-02 &  5.860693e-02 & -7.816564e-02 &      0.0 &  7.740329e-04 & -4.858990e-03 &  1.099240e-02 &  5.149637e-02 \\
608 &  2.596459e-02 &  4.131406e-02 & -1.418624e+00 &      0.0 &  8.464827e-05 & -3.083760e-03 &  3.842340e-03 &  2.842615e-02 \\
609 &  1.217398e-02 &  2.233534e-02 &  1.782438e+00 &      0.0 &  2.247428e-03 & -4.499941e-03 &  3.863584e-03 &  1.157643e-02 \\
610 &  4.212561e-03 &  9.264889e-03 &  1.103378e+00 &      0.0 &  2.138684e-03 & -7.601440e-04 & -1.829861e-03 & -6.170865e-03 \\
611 &  8.417400e-04 &  2.421735e-03 & -7.530690e-01 &      0.0 & -5.100264e-05 & -1.475279e-02 & -1.921327e-03 & -6.084595e-03 \\
612 &  1.510842e-04 &  8.917162e-04 &  2.776518e+01 &      0.0 & -6.839969e-04 & -3.156442e-02 & -1.427509e-03 & -3.433072e-03 \\
613 &  4.466773e-05 & -1.182311e-04 & -2.924839e+00 &      0.0 & -4.873530e-05 &  4.238613e-03 & -8.956656e-04 & -5.028600e-04 \\
614 &  1.028587e-04 & -2.722570e-04 & -1.270149e+00 &      0.0 & -4.885215e-05 &  4.276739e-03 & -2.062146e-03 & -1.154758e-03 \\
615 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.792108e-08 &  5.611592e-07 \\
616 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.635180e-07 & -7.424249e-07 \\
617 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.720362e-07 & -1.144387e-06 \\
618 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -7.469114e-08 & -1.480439e-06 \\
619 &  1.230253e-04 &  2.582007e-05 &  2.162452e+01 &      0.0 & -1.939634e-04 &  6.921972e-04 & -3.676874e-03 & -2.982143e-03 \\
620 &  2.658394e-03 & -2.263635e-03 &  1.652219e+00 &      0.0 & -1.692542e-03 &  2.043281e-03 & -7.133268e-03 & -1.388190e-03 \\
621 &  1.221136e-02 & -1.060760e-02 &  1.104361e+00 &      0.0 &  2.008374e-03 & -1.215382e-03 & -1.948223e-02 &  1.002908e-02 \\
622 &  3.075766e-02 & -2.044074e-02 &  3.076929e+00 &      0.0 &  5.059090e-04 & -3.108585e-03 & -2.546807e-02 &  1.927472e-02 \\
623 &  5.775459e-02 & -3.040093e-02 & -8.984034e-01 &      0.0 &  2.530837e-03 & -7.946021e-04 & -3.380982e-03 &  2.464195e-02 \\
624 &  8.156596e-02 & -3.536700e-02 & -1.302520e-01 &      0.0 & -3.906437e-03 & -5.689979e-04 & -9.541770e-03 &  2.184264e-02 \\
625 &  9.709215e-02 & -3.461159e-02 &  4.059596e-01 &      0.0 &  1.749079e-03 &  8.827187e-04 & -3.546476e-02 &  6.662224e-03 \\
626 &  9.786162e-02 & -3.750783e-02 & -8.311737e-02 &      0.0 &  8.799255e-04 & -8.964743e-04 & -7.004376e-02 & -2.773782e-02 \\
627 &  8.692649e-02 & -3.627469e-02 &  6.855840e-01 &      0.0 & -1.213746e-03 &  2.571889e-03 & -8.673649e-02 & -8.637463e-02 \\
628 &  7.272435e-02 & -3.220523e-02 &  1.175682e-01 &      0.0 & -2.642968e-03 &  4.359278e-04 & -8.633328e-02 & -1.349819e-01 \\
629 &  6.540714e-02 & -1.941404e-02 & -1.412976e-01 &      0.0 &  3.955272e-03 & -1.046725e-03 & -6.996925e-02 & -1.108975e-01 \\
630 &  6.183351e-02 &  1.198576e-03 & -2.514241e-01 &      0.0 & -1.946169e-03 & -1.299323e-03 & -7.055431e-02 & -5.973793e-02 \\
631 &  5.890587e-02 &  2.771604e-02 & -1.721675e-01 &      0.0 &  6.983911e-04 &  3.993406e-03 & -4.789696e-02 & -4.632540e-03 \\
632 &  5.185140e-02 &  5.343956e-02 & -5.520082e-01 &      0.0 &  2.017964e-04 & -8.064960e-04 & -1.115869e-02 &  4.358714e-02 \\
633 &  4.069575e-02 &  6.399126e-02 &  1.435097e-01 &      0.0 &  3.343243e-04 &  1.736092e-03 &  2.766651e-03 &  6.494310e-02 \\
634 &  2.832176e-02 &  5.928237e-02 & -3.489483e-01 &      0.0 &  1.225039e-03 &  1.567753e-03 &  3.989237e-03 &  5.519409e-02 \\
635 &  1.683285e-02 &  4.717894e-02 & -2.055072e-01 &      0.0 & -2.244276e-03 & -1.183912e-03 &  7.016033e-04 &  5.212507e-02 \\
636 &  8.309360e-03 &  2.743942e-02 &  6.796507e-01 &      0.0 & -2.620565e-03 & -2.551326e-03 & -2.198130e-03 &  2.241656e-02 \\
637 &  2.690998e-03 &  1.175391e-02 & -1.324759e+00 &      0.0 &  2.836800e-05 &  3.440898e-03 & -3.534516e-03 &  1.851977e-03 \\
638 &  9.310233e-04 &  3.647569e-03 &  4.994702e-01 &      0.0 & -1.026480e-03 & -1.307797e-04 & -1.189654e-03 & -3.216312e-03 \\
639 &  3.192033e-04 &  1.164713e-03 & -1.052488e+01 &      0.0 & -3.849785e-04 &  1.040071e-02 & -9.550507e-04 & -1.620447e-03 \\
640 & -7.677448e-06 &  3.484056e-04 & -7.000172e+00 &      0.0 & -6.645045e-04 & -2.399386e-02 & -1.639497e-04 & -2.603870e-04 \\
641 &  2.540733e-05 & -6.725074e-05 & -5.142056e+00 &      0.0 & -4.762684e-05 &  4.272141e-03 & -5.097839e-04 & -2.881957e-04 \\
642 &  5.819099e-05 & -1.540259e-04 & -2.245123e+00 &      0.0 & -4.807901e-05 &  4.223644e-03 & -1.166887e-03 & -6.553217e-04 \\
643 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -3.722669e-08 &  6.406791e-08 \\
644 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.259418e-07 & -1.105236e-06 \\
645 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.619933e-07 & -1.552991e-06 \\
646 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.541201e-08 & -4.794611e-07 \\
647 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.471139e-07 &  1.396762e-06 \\
648 &  2.291542e-04 & -3.020885e-04 & -3.029849e+00 &      0.0 &  1.123414e-03 &  1.313229e-03 & -2.774953e-03 & -1.773625e-03 \\
649 &  2.408616e-03 & -3.279392e-03 &  6.619567e-01 &      0.0 & -1.670524e-03 & -1.004012e-03 & -9.955099e-03 &  8.921924e-03 \\
650 &  8.526450e-03 & -8.032156e-03 & -1.086803e+00 &      0.0 & -7.951548e-05 &  4.500682e-04 & -1.501219e-02 &  6.419297e-03 \\
651 &  1.951367e-02 & -1.451156e-02 & -5.414252e-01 &      0.0 & -6.499246e-04 &  3.328614e-04 & -8.342698e-03 &  1.513591e-02 \\
652 &  3.855296e-02 & -2.310321e-02 &  2.135828e-01 &      0.0 &  1.102603e-04 &  2.455033e-03 &  2.794757e-03 &  1.478462e-02 \\
653 &  5.365519e-02 & -2.357877e-02 & -4.631131e-01 &      0.0 & -9.278198e-04 & -1.173370e-03 &  5.936655e-03 &  2.650070e-03 \\
654 &  6.145365e-02 & -1.742477e-02 & -1.717122e-01 &      0.0 &  1.302409e-03 & -1.094883e-03 & -5.775494e-03 & -3.566725e-02 \\
655 &  6.127720e-02 & -3.034289e-03 &  3.726750e-01 &      0.0 & -9.489240e-04 & -1.529546e-03 & -1.459946e-02 & -8.359256e-02 \\
656 &  5.645513e-02 &  1.528913e-02 &  1.322458e+00 &      0.0 & -3.893249e-03 &  2.093064e-03 & -4.802566e-02 & -1.087729e-01 \\
657 &  4.896479e-02 &  3.153396e-02 &  3.910037e-01 &      0.0 &  3.340570e-03 & -1.645126e-03 & -6.220286e-02 & -9.886104e-02 \\
658 &  3.973411e-02 &  4.833957e-02 &  2.388484e-01 &      0.0 &  5.239055e-04 & -7.074072e-04 & -5.005109e-02 & -5.525398e-02 \\
659 &  3.034684e-02 &  5.767275e-02 & -1.374326e-01 &      0.0 &  1.109734e-03 & -7.215829e-05 & -2.087268e-02 & -8.619746e-03 \\
660 &  1.752414e-02 &  6.063380e-02 &  9.622139e-02 &      0.0 & -5.063970e-04 &  1.083473e-03 &  1.257490e-03 &  3.834325e-02 \\
661 &  7.440882e-03 &  5.320687e-02 &  2.978281e-02 &      0.0 & -1.534009e-03 & -1.437789e-03 &  3.126735e-03 &  6.134275e-02 \\
662 &  2.638266e-03 &  4.213233e-02 & -3.764325e-04 &      0.0 &  1.411888e-04 &  4.676921e-03 &  4.593394e-03 &  6.967365e-02 \\
663 & -2.865324e-04 &  2.941350e-02 &  3.634049e-01 &      0.0 &  2.010003e-03 &  3.967871e-04 &  8.283797e-03 &  5.660677e-02 \\
664 & -1.090386e-03 &  1.694903e-02 & -3.636378e+00 &      0.0 & -2.790807e-04 & -2.663077e-03 &  7.566819e-03 &  3.078790e-02 \\
665 & -7.282638e-04 &  7.911557e-03 &  3.391390e+00 &      0.0 & -1.997747e-03 & -2.109175e-03 &  5.473784e-03 &  1.448241e-02 \\
666 & -8.854803e-05 &  3.342778e-03 & -2.419589e+00 &      0.0 &  3.259605e-04 &  6.964695e-03 &  1.037929e-03 &  3.205795e-03 \\
667 &  1.950719e-05 &  9.590925e-04 &  2.717894e+01 &      0.0 &  2.039971e-04 &  1.668076e-02 &  1.278431e-04 &  1.684250e-03 \\
668 &  1.131031e-05 &  2.181070e-04 & -1.985276e+01 &      0.0 &  7.356443e-04 &  1.684992e-03 &  6.463825e-05 &  5.880402e-04 \\
669 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.204195e-08 &  3.085839e-07 \\
670 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  6.907414e-08 &  1.131521e-07 \\
671 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -3.749352e-08 &  3.479745e-07 \\
672 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -2.705568e-07 & -2.259312e-06 \\
673 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -6.623757e-08 & -9.314802e-08 \\
674 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.072645e-07 &  8.745819e-07 \\
675 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -4.374929e-08 & -7.841749e-07 \\
676 &  5.752142e-05 & -1.241136e-05 &  2.281104e+00 &      0.0 &  2.979243e-04 & -1.749378e-03 & -7.884768e-04 & -1.377416e-03 \\
677 & -3.026679e-04 & -1.016695e-04 &  1.865537e+00 &      0.0 & -2.542523e-04 &  1.113277e-03 & -2.190754e-03 & -3.630204e-03 \\
678 & -5.263870e-04 & -2.437909e-04 & -2.619580e+00 &      0.0 & -1.518919e-03 &  7.894478e-04 & -1.806232e-03 & -6.683709e-03 \\
679 & -9.710172e-04 & -4.902726e-04 &  2.979591e-01 &      0.0 &  1.867188e-03 & -1.108736e-03 & -1.211825e-03 & -1.282012e-02 \\
680 & -1.539147e-03 &  7.842714e-04 & -9.733467e-01 &      0.0 & -2.536817e-05 & -2.970775e-04 &  2.393654e-03 & -1.890033e-02 \\
681 & -3.141457e-04 &  4.779202e-03 & -4.738006e-02 &      0.0 & -6.301547e-04 &  2.453712e-03 &  8.372378e-03 & -3.047895e-02 \\
682 & -2.076722e-03 &  1.210362e-02 &  4.385573e-01 &      0.0 &  1.697556e-03 & -1.673684e-03 &  1.685189e-02 & -5.897928e-02 \\
683 & -3.029087e-03 &  1.990606e-02 & -5.547854e-01 &      0.0 & -1.533078e-03 &  1.341376e-04 &  1.634333e-02 & -8.553485e-02 \\
684 & -2.437848e-03 &  2.802250e-02 & -6.050742e-01 &      0.0 &  3.812373e-03 & -1.371769e-03 &  2.343853e-03 & -8.746773e-02 \\
685 & -2.227851e-03 &  3.498499e-02 &  1.976017e-01 &      0.0 & -8.959979e-04 & -1.060860e-03 &  1.120302e-05 & -6.233511e-02 \\
686 & -4.497360e-03 &  3.873037e-02 &  3.369470e-01 &      0.0 & -1.274695e-04 &  1.874716e-03 &  8.732947e-04 & -3.173944e-02 \\
687 & -7.155401e-03 &  4.032267e-02 &  4.959205e-01 &      0.0 & -8.596012e-04 & -1.220093e-03 &  1.055695e-02 &  2.213586e-02 \\
688 & -9.749078e-03 &  4.098684e-02 & -9.617590e-01 &      0.0 &  2.403407e-03 &  1.419855e-03 &  2.494254e-02 &  6.802007e-02 \\
689 & -9.896483e-03 &  3.560769e-02 &  4.519485e-02 &      0.0 & -8.529057e-04 & -1.482973e-03 &  3.169825e-02 &  8.958181e-02 \\
690 & -8.035330e-03 &  2.877714e-02 &  4.022890e-01 &      0.0 & -7.105966e-04 &  3.497114e-04 &  2.782071e-02 &  8.678942e-02 \\
691 & -4.470357e-03 &  1.997129e-02 &  3.004569e-01 &      0.0 & -1.797304e-04 & -3.500160e-03 &  2.009690e-02 &  6.079634e-02 \\
692 & -2.639554e-03 &  1.379105e-02 &  9.301863e-01 &      0.0 &  2.369316e-03 &  8.204823e-03 &  1.271705e-02 &  3.918083e-02 \\
693 & -1.611075e-03 &  7.851651e-03 &  1.398335e+00 &      0.0 &  1.465724e-03 &  1.276916e-02 &  7.277467e-03 &  2.193125e-02 \\
694 & -6.684896e-04 &  3.760737e-03 &  5.415254e+00 &      0.0 &  1.206061e-03 &  1.379977e-02 &  3.415461e-03 &  1.006029e-02 \\
695 & -1.581033e-04 &  1.284376e-03 & -2.507438e+01 &      0.0 &  1.362796e-03 &  3.716244e-03 &  8.680553e-04 &  3.081955e-03 \\
696 &  1.569320e-05 &  1.844352e-04 & -3.231585e+01 &      0.0 &  7.211482e-04 &  3.666438e-03 &  6.750437e-05 &  5.865476e-04 \\
697 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -3.728324e-09 & -2.396008e-07 \\
698 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  7.041142e-08 &  9.216299e-07 \\
699 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.229953e-07 &  9.198030e-07 \\
700 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -2.600752e-08 & -4.941495e-07 \\
701 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -7.789870e-08 & -1.071397e-06 \\
702 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.281193e-08 & -3.693650e-07 \\
703 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  5.968228e-08 &  6.608798e-07 \\
704 & -5.656005e-05 &  7.435766e-06 &  5.319538e+01 &      0.0 &  4.801383e-04 & -3.018557e-03 &  5.966431e-05 & -2.246943e-04 \\
705 & -5.820547e-04 &  3.144414e-05 & -4.545644e+00 &      0.0 &  7.624410e-04 & -4.150980e-03 &  6.537492e-04 & -3.021233e-03 \\
706 & -1.403600e-03 &  8.507066e-05 &  3.345453e+00 &      0.0 &  1.257621e-03 & -5.703846e-03 &  1.684397e-03 & -6.819222e-03 \\
707 & -3.259427e-03 &  2.521225e-04 & -9.037955e-01 &      0.0 &  1.923377e-03 & -7.267389e-03 &  3.855714e-03 & -1.689189e-02 \\
708 & -6.386035e-03 &  1.775354e-03 & -3.557002e-03 &      0.0 & -2.589965e-04 &  6.545213e-04 &  8.585917e-03 & -3.616561e-02 \\
709 & -1.047250e-02 &  5.648504e-03 & -3.907660e-01 &      0.0 &  8.791606e-05 & -7.834184e-04 &  1.477371e-02 & -5.986629e-02 \\
710 & -1.477581e-02 &  1.069580e-02 & -6.360919e-01 &      0.0 & -3.189530e-04 & -1.029635e-03 &  1.916153e-02 & -8.321219e-02 \\
711 & -1.667399e-02 &  1.454275e-02 & -1.165163e+00 &      0.0 & -4.720623e-05 & -2.117163e-03 &  1.940722e-02 & -8.584347e-02 \\
712 & -1.667474e-02 &  1.831108e-02 &  2.614845e-01 &      0.0 & -4.390325e-04 &  1.126803e-03 &  1.803492e-02 & -6.445247e-02 \\
713 & -1.540295e-02 &  1.979781e-02 & -1.357805e+00 &      0.0 & -8.065292e-04 &  2.799086e-03 &  1.827271e-02 & -2.640612e-02 \\
714 & -1.375604e-02 &  2.066811e-02 & -2.625102e-01 &      0.0 & -1.823079e-04 & -3.435751e-04 &  2.281172e-02 &  7.647501e-03 \\
715 & -1.295598e-02 &  2.302606e-02 & -5.946117e-01 &      0.0 &  1.408122e-04 & -1.496174e-03 &  2.704860e-02 &  4.051363e-02 \\
716 & -1.224512e-02 &  2.513088e-02 &  3.408945e-01 &      0.0 &  4.389574e-03 & -1.563694e-02 &  3.193883e-02 &  6.780026e-02 \\
717 & -1.025611e-02 &  2.440068e-02 &  1.521726e-01 &      0.0 &  4.201773e-03 & -1.677160e-02 &  3.012652e-02 &  7.744319e-02 \\
718 & -7.095916e-03 &  1.922932e-02 & -5.157978e-01 &      0.0 &  3.932051e-03 & -1.672007e-02 &  2.236834e-02 &  6.401290e-02 \\
719 & -3.501526e-03 &  1.275257e-02 &  7.205732e-03 &      0.0 &  3.247515e-03 & -1.238979e-02 &  1.303173e-02 &  4.218208e-02 \\
720 & -2.074388e-03 &  9.981586e-03 & -8.651963e-01 &      0.0 &  3.168770e-03 & -1.004380e-02 &  9.015038e-03 &  3.185675e-02 \\
721 & -1.199328e-03 &  5.825877e-03 & -2.221341e+00 &      0.0 &  2.577584e-03 & -5.364812e-03 &  5.507347e-03 &  1.864539e-02 \\
722 & -4.827425e-04 &  2.289409e-03 & -7.240986e+00 &      0.0 &  2.013705e-03 & -1.976114e-03 &  2.112922e-03 &  7.013789e-03 \\
723 & -7.144246e-05 &  8.653296e-04 &  2.738386e+01 &      0.0 &  1.338511e-03 &  1.032021e-03 &  5.114464e-04 &  2.275834e-03 \\
724 &  1.799549e-05 &  1.147735e-04 & -3.397953e+00 &      0.0 &  7.134833e-04 &  1.805383e-03 &  3.638362e-05 &  3.861966e-04 \\
725 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -4.190207e-08 &  2.328689e-07 \\
726 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.306750e-07 & -1.424870e-06 \\
727 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -4.398063e-10 & -1.264876e-07 \\
728 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.884309e-07 &  1.124663e-06 \\
729 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.711148e-07 &  1.349753e-06 \\
730 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -5.313396e-08 & -6.039921e-07 \\
731 & -2.539976e-05 &  3.776508e-06 & -1.102688e+02 &      0.0 &  4.075603e-04 & -2.682511e-03 &  2.570099e-05 & -7.448078e-05 \\
732 & -2.294575e-04 &  4.397752e-05 &  5.987496e+00 &      0.0 &  5.070693e-04 & -3.210839e-03 &  2.273402e-04 & -7.652246e-04 \\
733 & -2.738462e-04 &  7.203454e-05 & -3.953761e+00 &      0.0 &  6.234298e-04 & -3.415640e-03 &  2.474373e-04 & -1.060198e-03 \\
734 & -6.135806e-04 &  2.877787e-04 & -1.717996e+00 &      0.0 &  1.039610e-03 & -3.942357e-03 &  5.589388e-04 & -2.555238e-03 \\
735 & -1.152899e-03 &  2.874451e-04 &  4.047560e-01 &      0.0 &  1.309093e-03 & -4.957458e-03 &  1.241243e-03 & -5.535967e-03 \\
736 & -2.504250e-03 &  1.231505e-03 & -8.673062e-01 &      0.0 &  1.452820e-03 & -5.796370e-03 &  3.391797e-03 & -1.287028e-02 \\
737 & -3.500268e-03 &  2.205906e-03 & -2.598129e-01 &      0.0 &  1.821299e-03 & -7.194959e-03 &  5.261684e-03 & -1.857650e-02 \\
738 & -4.122172e-03 &  3.315884e-03 & -4.441546e-01 &      0.0 &  2.020664e-03 & -7.528529e-03 &  6.033610e-03 & -2.169075e-02 \\
739 & -4.730412e-03 &  4.723344e-03 & -9.949365e-02 &      0.0 &  2.284612e-03 & -7.711842e-03 &  6.074879e-03 & -2.521749e-02 \\
740 & -4.602826e-03 &  5.233969e-03 & -6.330188e-01 &      0.0 &  2.596169e-03 & -7.639656e-03 &  5.927498e-03 & -1.790067e-02 \\
741 & -4.687762e-03 &  5.631349e-03 &  1.291550e+00 &      0.0 &  2.589763e-03 & -7.380886e-03 &  7.094035e-03 & -8.514172e-03 \\
742 & -4.594130e-03 &  6.861087e-03 & -1.683821e+00 &      0.0 &  2.653358e-03 & -7.986959e-03 &  7.791921e-03 &  2.790446e-03 \\
743 & -3.194886e-03 &  5.962465e-03 &  1.082502e+00 &      0.0 &  2.506563e-03 & -8.312009e-03 &  6.431393e-03 &  1.000250e-02 \\
744 & -3.138126e-03 &  5.993810e-03 & -1.503194e+00 &      0.0 &  2.759348e-03 & -1.021936e-02 &  6.510421e-03 &  1.208243e-02 \\
745 & -3.120424e-03 &  5.910728e-03 &  1.358648e+00 &      0.0 &  2.790179e-03 & -1.150426e-02 &  7.627292e-03 &  1.689616e-02 \\
746 & -1.902058e-03 &  4.865051e-03 & -1.094915e+00 &      0.0 &  2.662167e-03 & -1.154675e-02 &  5.552636e-03 &  1.587248e-02 \\
747 & -7.870360e-04 &  3.124731e-03 & -4.288916e-01 &      0.0 &  2.322850e-03 & -9.592799e-03 &  2.823232e-03 &  9.738898e-03 \\
748 & -5.203996e-04 &  2.650715e-03 & -2.055665e+00 &      0.0 &  2.270236e-03 & -8.774401e-03 &  2.109933e-03 &  7.718832e-03 \\
749 & -3.035289e-04 &  1.405775e-03 &  4.753428e+00 &      0.0 &  1.755095e-03 & -7.045795e-03 &  1.223565e-03 &  4.229259e-03 \\
750 & -1.336764e-04 &  6.661385e-04 & -3.432319e+00 &      0.0 &  1.338670e-03 & -5.880489e-03 &  6.285150e-04 &  1.967355e-03 \\
751 & -6.115193e-05 &  1.684902e-04 & -9.518437e+00 &      0.0 &  8.708382e-04 & -6.086616e-03 &  1.915568e-04 &  6.989065e-04 \\
752 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.014745e-07 & -1.778624e-07 \\
753 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -5.643109e-08 & -3.344708e-07 \\
754 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -9.806280e-08 & -1.009002e-06 \\
755 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.336854e-07 & -8.389283e-07 \\
756 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.367782e-07 &  1.319870e-08 \\
757 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  4.413217e-09 &  1.590588e-07 \\
758 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.615125e-07 &  7.672923e-07 \\
759 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.320162e-07 & -6.571403e-07 \\
760 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.269850e-07 &  1.511644e-06 \\
761 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  1.460426e-07 &  8.283582e-07 \\
762 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.999891e-07 & -2.203385e-06 \\
763 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  7.727143e-08 &  4.255096e-08 \\
764 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  6.994222e-08 &  8.889251e-07 \\
765 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -3.851499e-08 &  4.730342e-07 \\
766 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  7.632283e-08 & -6.124176e-09 \\
767 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -1.628061e-07 & -1.073616e-06 \\
768 & -1.143231e-04 &  1.686250e-04 &  2.151678e+00 &      0.0 &  8.932923e-04 & -2.657314e-03 &  1.993987e-04 & -4.379605e-04 \\
769 & -1.526303e-04 &  2.251276e-04 &  1.611649e+00 &      0.0 &  8.932279e-04 & -2.657234e-03 &  2.664358e-04 & -5.829223e-04 \\
770 & -2.166498e-04 &  2.988405e-04 & -1.618115e+00 &      0.0 &  9.664795e-04 & -2.926651e-03 &  3.373058e-04 & -3.061332e-04 \\
771 & -9.736587e-05 &  1.977600e-04 & -7.895789e-01 &      0.0 &  5.543896e-04 & -1.764739e-03 &  6.914643e-05 &  3.300455e-04 \\
772 & -2.781882e-05 &  5.650284e-05 & -2.763526e+00 &      0.0 &  5.544265e-04 & -1.764233e-03 &  1.992400e-05 &  9.574934e-05 \\
773 & -6.131117e-06 &  1.867468e-05 & -1.746288e+01 &      0.0 &  7.252392e-04 & -3.394297e-03 &  1.210975e-05 &  5.968858e-05 \\
774 & -9.765993e-05 &  2.974610e-04 & -1.096325e+00 &      0.0 &  7.252445e-04 & -3.394531e-03 &  1.951335e-04 &  9.732997e-04 \\
775 & -1.312188e-04 &  3.809570e-04 & -2.195891e-01 &      0.0 &  1.156035e-03 & -5.660519e-03 &  3.406247e-04 &  1.112978e-03 \\
776 & -7.612529e-05 &  2.147084e-04 &  8.472045e-01 &      0.0 &  9.028760e-04 & -4.529890e-03 &  2.240243e-04 &  5.799613e-04 \\
777 & -1.064689e-06 &  3.002915e-06 &  6.057512e+01 &      0.0 &  9.027813e-04 & -4.529981e-03 &  3.223115e-06 &  8.787394e-06 \\
778 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -5.168960e-08 & -8.730578e-07 \\
779 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  4.035262e-08 &  6.541917e-07 \\
780 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.965180e-07 &  2.597290e-06 \\
781 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -5.173480e-08 & -2.495303e-08 \\
782 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 &  2.666126e-07 &  1.383249e-06 \\
783 &  0.000000e+00 & -0.000000e+00 &  0.000000e+00 &      0.0 &  0.000000e+00 & -0.000000e+00 & -6.421842e-08 & -5.347574e-07 \\
\bottomrule
\end{tabular}

